Adaptive Classification of Interval-Valued Time Series

In recent years, the modeling and analysis of interval-valued time series have garnered significant attention in the fields of econometrics and statistics. However, the existing literature primarily focuses on regression tasks while neglecting classification aspects. In this paper, we propose an adaptive approach for interval-valued time series classification. Specifically, we represent interval-valued time series using convex combinations of upper and lower bounds of intervals and transform these representations into images based on point-valued time series imaging methods. We utilize a fine-grained image classification neural network to classify these images, to achieve the goal of classifying the original interval-valued time series. This proposed method is applicable to both univariate and multivariate interval-valued time series. On the optimization front, we treat the convex combination coefficients as learnable parameters similar to the parameters of the neural network and provide an efficient estimation method based on the alternating direction method of multipliers (ADMM). On the theoretical front, under specific conditions, we establish a margin-based multiclass generalization bound for generic CNNs composed of basic blocks involving convolution, pooling, and fully connected layers. Through simulation studies and real data applications, we validate the effectiveness of the proposed method and compare its performance against a wide range of point-valued time series classification methods.

==> Annotation.tex <==
\section{Simulation Studies} \label{sec5}
The purpose of this section is to compare, via simulation experiments, the impact of point-valued time series imaging methods and interval-value time series imaging methods on the discrimination of different data generation processes (DGPs). In this section and the real data studies in Section \ref{sec6}, we choose representative ResNet \cite{He2016} with different layers as discriminant models which have promising performance on many computer vision tasks. Specifically, we choose ResNet18, 34, 50, 101, 152 as the base models for discrimination and assess the effect of network depth on simulation results. In all the examples below, we first generate the center and range  time series, which are then transformed into upper and lower bound time series for discriminations. Each randomly generated interval-valued time series has a length of \(T=100\), and the number of samples per class is 300. In addition, the threshold values in both the point-value and interval-value time series imaging methods are set to \(\pi/18\). The effectiveness of different models and levels of approximation, as well as different kernel functions for the discrimination of different DGPs is evaluated based on the following metrics: 
\[
\begin{aligned}
	\text{miP} & = P(A, \widehat{A}), \ \text{maP}  = \frac{1}{|L|}\sum_{l \in L} P(A_l, \widehat{A}_l), \ \text{weiP} = \frac{1}{\sum_{l=L}|A_l|}\sum_{l \in L} |A_l|P(A_l, \widehat{A}_l),\\
	\text{miR} &= R(A, \widehat{A}), \ \text{maR} = \frac{1}{|L|}\sum_{l \in L} R(A_l, \widehat{A}_l), \ \text{weiR} = \frac{1}{\sum_{l=L}|A_l|}\sum_{l \in L} |A_l|R(A_l, \widehat{A}_l),\\
	\text{miF}_1 &= F_1(A, \widehat{A}),\ \text{maF}_1 = \frac{1}{|L|}\sum_{l \in L} F_1(A_l, \widehat{A}_l), \ \text{weiF}_1 = \frac{1}{\sum_{l=L}|A_l|}\sum_{l \in L} |A_l|F_1(A_l, \widehat{A}_l), \\
\end{aligned}
\]
where \(A\) is the set of true labels, \(\widehat{A}\) is the set of predicted labels, \(L\) is the  set of labels, \(A_l\) is the subset of \(A\) with label \(l\), \(\widehat{A}_l\) is the subset of \(\widehat{A}\) with label \(l\), \(|A|\) is the cardinality of set \(A\), mi,ma,wei are abbreviations of micro, macro, weighted, respectively. \(P(A, \widehat{A}), R(A, \widehat{A})\) and \(F_1(A, \widehat{A})\) are are generally referred to as precision, recall and \(F_1\) score, which are defined as
\[
P(A, \widehat{A}) = \frac{|A  \cap \widehat{A}|}{|\widehat{A}|},\  R(A, \widehat{A}) = \frac{|A  \cap \widehat{A}|}{|A|}, \ F_1(A, \widehat{A}) = \frac{2 P(A, \widehat{A}) \times R(A, \widehat{A})}{P(A, \widehat{A}) + R(A, \widehat{A})}.
\]
%\[r
%\begin{aligned}
%\text{miP} & = P(A, \widehat{A}), \ \text{miR} = R(A, \widehat{A}), \ \ \text{miF}_1 = F_1(A, \widehat{A})\\
%\text{maP} & = \frac{1}{|L|}\sum_{l \in L} P(A_l, \widehat{A}_l), \ \text{maR} = \frac{1}{|L|}\sum_{l \in L} R(A_l, \widehat{A}_l), \ \ \text{maF}_1 = \frac{1}{|L|}\sum_{l \in L} F_1(A_l, \widehat{A}_l)\\
%\text{weiP} & = \frac{1}{\sum_{l=L}|A_l|}\sum_{l \in L} |A_l|P(A_l, \widehat{A}_l), \ \text{weiR} = \frac{1}{\sum_{l=L}|A_l|}\sum_{l \in L} |A_l|R(A_l, \widehat{A}_l), \ \ \text{weiF}_1 = \frac{1}{\sum_{l=L}|A_l|}\sum_{l \in L} |A_l|F_1(A_l, \widehat{A}_l)\\
%\end{aligned}
%\]



\subsection{Univariate interval-valued time series discriminant}\label{ss1}
\subsubsection{Simulation design}
In the following example, \(\epsilon_t = \left(\begin{array}{c}
	\epsilon^c_t\\
	\epsilon^r_t\\
\end{array}\right)  \overset{i.i.d}{\sim} \mathcal{N}(0, \Sigma)\), where \(\Sigma = \left(\begin{array}{cc}
	1 & \rho/2\\
	\rho/ 2 & 1/4
\end{array}\right)\), \(\rho\) is the correlation coefficient between the center and the range interval-valued residuals. We choose \(\rho=0, 0.3, 0.7, 0.9\) such that the interval-valued time series generated by different \(\rho\) are of different classes. Following are the three DGPs considered in the simulation studies.

%\(\rho=0, \pm 0.3, \pm 0.5, \pm 0.7, \pm 0.9\) /
\emph{DGP1:bivariate regression}: 
\[
x_t = \left(\begin{array}{c}
	x^c_t\\
	x^r_t\\
\end{array}\right)= \sum_{l=1}^{\infty} \pi_l \Phi z_{t,l} + \epsilon_{t},
\]
where \(z_{t,1}= \left(\begin{array}{c}
	1\\
	1\\
\end{array}\right)\), \(z_{t, l} \overset{i.i.d}{\sim} \mathcal{N}(0, \Sigma), l\geq 2\), and \(\Phi = \left(\begin{array}{cc}
	0.2 & -0.1\\
	0.1 & 0.2
\end{array}\right)\), \(\pi_l = l^{-2} / \sqrt{3}\).


\emph{DGP2:bivariate regression}: 
\[
x_t = \left(\begin{array}{c}
	x^c_t\\
	x^r_t\\
\end{array}\right)=\Phi  x_{t-1} + \epsilon_{t} - \theta \epsilon_{t-1}, 
\]
where \(\Phi\) is the same as in DGP1, and \(\theta=\left(\begin{array}{cc}
	-0.6 & 0.3\\
	0.3 & 0.6
\end{array}\right)\).

\emph{DGP3:bivariate regression}: 
\[
x_t = \left(\begin{array}{c}
	x^c_t\\
	x^r_t\\
\end{array}\right)=\epsilon_t - \theta \epsilon_{t-1},
\]
where \(\theta\) is the same as in DGP2. 

According to the DGPs 1-3, we yield a total of three interval-valued time series classification data sets, each containing 2700 samples in nine classes. We randomly select 80 percent of the data as the training set and the remaining as the test set. In light of Figure \ref{app}, it can be found that \((1 + \tanh(\nu(\epsilon_i - \lVert \vec{x}^{\text{cov}}_{i,j} -\vec{x}^{\text{cov}}_{i, k} \rVert_2))) / 2\) shows a superior approximation to the function \(H(\epsilon_i - \lVert \vec{x}^{\text{cov}}_{i,j} -\vec{x}^{\text{cov}}_{i, k} \rVert_2)\) for \(\nu=20\). To evaluate the effect of different levels of approximation, i.e., different values of \(\nu\), on the discriminant results, we chose \(\nu = 1, 5, 10, 15, 20\) for the simulation studies. In detail, the RP-based interval-valued time series discriminant results on the validation set are shown in the following three tables.

\subsubsection{Discriminant results based on RP}

% table 1
%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Univariate interval-valued time series (DGP1) discriminant results based on RP}
%\setlength{\tabcolsep}{2mm}{
	%\begin{tabular}{clccccccccc}
	%\toprule
	%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 1\)}} &ResNet18 & 0.6428 & 0.6604 & 0.6674 & 0.6961 & 0.6898 & 0.6966 & 0.6134 & 0.663 & 0.6681 \\ 
	%&ResNet34& 0.7124 & 0.6759 & 0.6815 & 0.7381 & 0.6846 & 0.7285 & 0.6645 & 0.6663 & 0.665 \\ 
	%&ResNet50& 0.8272 & 0.8042 & 0.8033 & 0.8002 & 0.8181 & 0.8115 & 0.8137 & 0.8181 & 0.8357 \\ 
	%&ResNet101& 0.8481 & 0.8446 & 0.8692 & 0.8591 & 0.8441 & 0.8564 & 0.8868 & 0.8733 & 0.8605 \\ 
	%&ResNet152& 0.9526 & 0.9457 & 0.9436 & 0.9254 & 0.93 & 0.9663 & 0.9017 & 0.9139 & 0.9249 \\ 
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 5\)}} &ResNet18 & 0.603 & 0.631 & 0.6784 & 0.6649 & 0.6142 & 0.6489 & 0.6922 & 0.6244 & 0.6393 \\ 
	%&ResNet34 & 0.6785 & 0.6575 & 0.6832 & 0.7435 & 0.7498 & 0.6958 & 0.7255 & 0.6761 & 0.7428 \\ 
	%&ResNet50& 0.811 & 0.8044 & 0.8429 & 0.8252 & 0.8212 & 0.8365 & 0.8363 & 0.8498 & 0.8267 \\ 
	%&ResNet101& 0.855 & 0.8541 & 0.8471 & 0.8465 & 0.8447 & 0.8685 & 0.8406 & 0.8897 & 0.8719 \\ 
	%&ResNet152& 0.94 & 0.9174 & 0.9524 & 0.9195 & 0.9607 & 0.9128 & 0.9069 & 0.9674 & 0.9383 \\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 10\)}} &ResNet18 & 0.6548 & 0.6085 & 0.6964 & 0.6335 & 0.692 & 0.6255 & 0.6309 & 0.6487 & 0.6 \\ 
	%&ResNet34 & 0.6763 & 0.7051 & 0.6824 & 0.706 & 0.7101 & 0.6766 & 0.716 & 0.6534 & 0.6768 \\ 
	%&ResNet50& 0.8071 & 0.8001 & 0.8265 & 0.826 & 0.832 & 0.8285 & 0.8494 & 0.8248 & 0.8312 \\ 
	%&ResNet101& 0.8482 & 0.8868 & 0.8699 & 0.8686 & 0.8513 & 0.8722 & 0.8648 & 0.8662 & 0.8869 \\ 
	%&ResNet152& 0.9619 & 0.9353 & 0.9006 & 0.93 & 0.909 & 0.9188 & 0.9649 & 0.9105 & 0.9141 \\ 
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 15\)}} &ResNet18 & 0.6061 & 0.6808 & 0.6333 & 0.6339 & 0.6139 & 0.6245 & 0.6084 & 0.6858 & 0.6396 \\ 
	%&ResNet34 & 0.6692 & 0.714 & 0.6519 & 0.7222 & 0.6612 & 0.7199 & 0.7142 & 0.7036 & 0.7273 \\ 
	%&ResNet50& 0.8088 & 0.8368 & 0.8211 & 0.823 & 0.8477 & 0.8435 & 0.8072 & 0.8071 & 0.8422 \\ 
	%&ResNet101& 0.8781 & 0.8678 & 0.8704 & 0.8703 & 0.8511 & 0.8751 & 0.8888 & 0.8701 & 0.8717 \\ 
	%&ResNet152& 0.9276 & 0.9518 & 0.9404 & 0.9636 & 0.9553 & 0.9216 & 0.9516 & 0.9695 & 0.9266 \\ 
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 20\)}} &ResNet18 & 0.6399 & 0.6562 & 0.6901 & 0.6737 & 0.6331 & 0.6042 & 0.6211 & 0.6442 & 0.6122 \\ 
	%&ResNet34 & 0.6706 & 0.6947 & 0.6902 & 0.7168 & 0.7074 & 0.7353 & 0.682 & 0.7132 & 0.7269 \\ 
	%&ResNet50& 0.8171 & 0.8489 & 0.8497 & 0.8361 & 0.817 & 0.8261 & 0.8399 & 0.8427 & 0.8323 \\ 
	%&ResNet101& 0.8642 & 0.8543 & 0.8882 & 0.8816 & 0.8845 & 0.8458 & 0.8613 & 0.8752 & 0.8404 \\ 
	%&ResNet152& 0.9376 & 0.9423 & 0.9143 & 0.909 & 0.9631 & 0.9301 & 0.9397 & 0.9047 & 0.9195 \\ 
	%\bottomrule
	%\end{tabular}
	%}
%\end{table}

\begin{table}[H]
	\footnotesize
	\setlength{\abovecaptionskip}{0pt}%
	\setlength{\belowcaptionskip}{3pt}%
	\centering
	\caption{Univariate interval-valued time series discriminant results based on RP}
	\setlength{\tabcolsep}{2mm}{
		\begin{tabular}{ccccccccccc}
			\toprule
			DGP& \(\nu\) & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
			\midrule
			\multirow{5}{*}{\tabincell{c}{DGP1}} &\(\nu = 1\) & 0.6428 & 0.6604 & 0.6674 & 0.6961 & 0.6898 & 0.6966 & 0.6134 & 0.663 & 0.6681 \\ 
			&\(\nu = 5\)& 0.7124 & 0.6759 & 0.6815 & 0.7381 & 0.6846 & 0.7285 & 0.6645 & 0.6663 & 0.665 \\ 
			&\(\nu = 10\)& 0.8272 & 0.8042 & 0.8033 & 0.8002 & 0.8181 & 0.8115 & 0.8137 & 0.8181 & 0.8357 \\ 
			&\(\nu = 15\)& 0.8481 & 0.8446 & 0.8692 & 0.8591 & 0.8441 & 0.8564 & 0.8868 & 0.8733 & 0.8605 \\ 
			&\(\nu = 20\)& 0.9526 & 0.9457 & 0.9436 & 0.9254 & 0.93 & 0.9663 & 0.9017 & 0.9139 & 0.9249 \\ 
			\midrule
			\multirow{5}{*}{\tabincell{c}{DGP2}} &\(\nu = 1\) & 0.603 & 0.631 & 0.6784 & 0.6649 & 0.6142 & 0.6489 & 0.6922 & 0.6244 & 0.6393 \\ 
			&\(\nu = 5\) & 0.6785 & 0.6575 & 0.6832 & 0.7435 & 0.7498 & 0.6958 & 0.7255 & 0.6761 & 0.7428 \\ 
			&\(\nu = 10\)& 0.811 & 0.8044 & 0.8429 & 0.8252 & 0.8212 & 0.8365 & 0.8363 & 0.8498 & 0.8267 \\ 
			&\(\nu = 15\)& 0.855 & 0.8541 & 0.8471 & 0.8465 & 0.8447 & 0.8685 & 0.8406 & 0.8897 & 0.8719 \\ 
			&\(\nu = 20\)& 0.94 & 0.9174 & 0.9524 & 0.9195 & 0.9607 & 0.9128 & 0.9069 & 0.9674 & 0.9383 \\
			\midrule
			\multirow{5}{*}{\tabincell{c}{DGP2}} &\(\nu = 1\) & 0.6548 & 0.6085 & 0.6964 & 0.6335 & 0.692 & 0.6255 & 0.6309 & 0.6487 & 0.6 \\ 
			&\(\nu = 5\) & 0.6763 & 0.7051 & 0.6824 & 0.706 & 0.7101 & 0.6766 & 0.716 & 0.6534 & 0.6768 \\ 
			&\(\nu = 10\)& 0.8071 & 0.8001 & 0.8265 & 0.826 & 0.832 & 0.8285 & 0.8494 & 0.8248 & 0.8312 \\ 
			&\(\nu = 15\)& 0.8482 & 0.8868 & 0.8699 & 0.8686 & 0.8513 & 0.8722 & 0.8648 & 0.8662 & 0.8869 \\ 
			&\(\nu = 20\)& 0.9619 & 0.9353 & 0.9006 & 0.93 & 0.909 & 0.9188 & 0.9649 & 0.9105 & 0.9141 \\
			\bottomrule
		\end{tabular}
	}
\end{table}


%%\begin{table}[H]
%%\footnotesize
%%\setlength{\abovecaptionskip}{0pt}%
%%\setlength{\belowcaptionskip}{3pt}%
%%\centering
%%\caption{Univariate interval-valued time series (DGP2) discriminant results based on RP}
%%\setlength{\tabcolsep}{2mm}{  
	%%\begin{tabular}{clccccccccc}
	%%\toprule
	%%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%%\midrule
	%%\multirow{5}{*}{\tabincell{c}{\(\nu = 1\)}} &ResNet18 & 0.694 & 0.678 & 0.6578 & 0.6821 & 0.6976 & 0.6896 & 0.6773 & 0.6893 & 0.6712 \\ 
	%%&ResNet34 & 0.7073 & 0.721 & 0.7255 & 0.7237 & 0.7128 & 0.7494 & 0.7326 & 0.7332 & 0.7419 \\ 
	%%&ResNet50& 0.8147 & 0.8436 & 0.803 & 0.8109 & 0.7972 & 0.8053 & 0.8287 & 0.8174 & 0.8043 \\ 
	%%&ResNet101& 0.8721 & 0.8872 & 0.8025 & 0.8287 & 0.8023 & 0.8873 & 0.8232 & 0.8723 & 0.828 \\ 
	%%&ResNet152& 0.9569 & 0.9617 & 0.9669 & 0.9442 & 0.9374 & 0.9328 & 0.9319 & 0.9503 & 0.9395 \\
	%%\midrule
	%%\multirow{5}{*}{\tabincell{c}{\(\nu = 5\)}} &ResNet18 & 0.6556 & 0.6646 & 0.6548 & 0.6976 & 0.6663 & 0.6575 & 0.6874 & 0.6914 & 0.6513 \\ 
	%%&ResNet34 & 0.7283 & 0.7245 & 0.7103 & 0.6913 & 0.6896 & 0.6889 & 0.7053 & 0.7258 & 0.6935 \\ 
	%%&ResNet50& 0.8115 & 0.8436 & 0.8412 & 0.8416 & 0.8447 & 0.829 & 0.791 & 0.8275 & 0.8411 \\ 
	%%&ResNet101& 0.8674 & 0.8027 & 0.8181 & 0.8327 & 0.8446 & 0.8571 & 0.8638 & 0.8628 & 0.8014 \\ 
	%%&ResNet152& 0.9214 & 0.939 & 0.9677 & 0.92 & 0.9623 & 0.9695 & 0.9397 & 0.9694 & 0.936 \\ 
	%%\midrule
	%%\multirow{5}{*}{\tabincell{c}{\(\nu = 10\)}} &ResNet18 & 0.6992 & 0.658 & 0.6822 & 0.6932 & 0.69 & 0.674 & 0.693 & 0.6952 & 0.6879 \\ 
	%%&ResNet34 & 0.7444 & 0.7307 & 0.6884 & 0.7037 & 0.7028 & 0.7074 & 0.6954 & 0.6852 & 0.7394 \\ 
	%%&ResNet50& 0.8303 & 0.8129 & 0.8217 & 0.8251 & 0.8497 & 0.8492 & 0.8296 & 0.7966 & 0.8381 \\ 
	%%&ResNet101& 0.8578 & 0.8854 & 0.8493 & 0.8387 & 0.8531 & 0.874 & 0.8368 & 0.8529 & 0.8443 \\ 
	%%&ResNet152& 0.9373 & 0.9675 & 0.9544 & 0.9319 & 0.9551 & 0.9685 & 0.9684 & 0.9633 & 0.9695 \\ 
	%%\midrule
	%%\multirow{5}{*}{\tabincell{c}{\(\nu = 15\)}}&ResNet18 & 0.6852 & 0.6709 & 0.6678 & 0.6617 & 0.6987 & 0.6942 & 0.6785 & 0.6825 & 0.6513 \\ 
	%%&ResNet34 & 0.7486 & 0.7346 & 0.6904 & 0.6812 & 0.7363 & 0.684 & 0.7198 & 0.7223 & 0.6929 \\ 
	%%&ResNet50& 0.8389 & 0.8202 & 0.8205 & 0.8022 & 0.7948 & 0.8372 & 0.8473 & 0.796 & 0.8331 \\ 
	%%&ResNet101& 0.8612 & 0.8508 & 0.8434 & 0.8859 & 0.8401 & 0.8837 & 0.8327 & 0.8134 & 0.8224 \\ 
	%%&ResNet152& 0.9647 & 0.9442 & 0.9317 & 0.9268 & 0.9392 & 0.9263 & 0.9368 & 0.9425 & 0.9437 \\ 
	%%\midrule
	%%\multirow{5}{*}{\tabincell{c}{\(\nu = 20\)}} &ResNet18 & 0.6805 & 0.654 & 0.6524 & 0.697 & 0.6758 & 0.6721 & 0.6643 & 0.6643 & 0.6875 \\ 
	%%&ResNet34 & 0.6903 & 0.6828 & 0.7162 & 0.6972 & 0.728 & 0.6835 & 0.7203 & 0.7318 & 0.7324 \\ 
	%%&ResNet50& 0.8265 & 0.8278 & 0.8331 & 0.8065 & 0.84 & 0.8002 & 0.8399 & 0.8435 & 0.7975 \\ 
	%%&ResNet101& 0.8537 & 0.8707 & 0.8214 & 0.8301 & 0.8543 & 0.8124 & 0.8153 & 0.823 & 0.8097 \\ 
	%%&ResNet152& 0.9575 & 0.9327 & 0.9202 & 0.9363 & 0.9302 & 0.9587 & 0.9537 & 0.93 & 0.9469 \\ 
	%%\bottomrule
	%%\end{tabular}
	%%}
%%\end{table}
%%
%%
%%\begin{table}[H]
%%\footnotesize
%%\setlength{\abovecaptionskip}{0pt}%
%%\setlength{\belowcaptionskip}{3pt}%
%%\centering
%%\caption{Univariate interval-valued time series (DGP3) discriminant results based on RP}
%%\setlength{\tabcolsep}{2mm}{  
	%%\begin{tabular}{clccccccccc}
	%%\toprule
	%%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%%\midrule
	%%\multirow{5}{*}{\tabincell{c}{\(\nu = 1\)}} &ResNet18 & 0.58 & 0.5582 & 0.6513 & 0.695 & 0.6944 & 0.6502 & 0.6958 & 0.5839 & 0.6776 \\ 
	%%&ResNet34 & 0.7123 & 0.713 & 0.6358 & 0.6462 & 0.6314 & 0.741 & 0.7139 & 0.74 & 0.6926 \\ 
	%%&ResNet50& 0.8344 & 0.7529 & 0.8357 & 0.7444 & 0.8393 & 0.7435 & 0.8417 & 0.8425 & 0.7859 \\ 
	%%&ResNet101& 0.8348 & 0.8191 & 0.8436 & 0.8201 & 0.8731 & 0.7948 & 0.8105 & 0.8585 & 0.8099 \\ 
	%%&ResNet152& 0.9263 & 0.9386 & 0.9192 & 0.9513 & 0.9491 & 0.9195 & 0.917 & 0.9252 & 0.9509 \\ 
	%%\midrule
	%%\multirow{5}{*}{\tabincell{c}{\(\nu = 5\)}} &ResNet18 & 0.6626 & 0.6702 & 0.5827 & 0.6771 & 0.652 & 0.6717 & 0.5666 & 0.6421 & 0.658 \\ 
	%%&ResNet34 & 0.6185 & 0.7198 & 0.6092 & 0.6874 & 0.6845 & 0.6244 & 0.684 & 0.6922 & 0.732 \\ 
	%%&ResNet50& 0.8482 & 0.8478 & 0.838 & 0.8021 & 0.8232 & 0.7774 & 0.7895 & 0.8427 & 0.7273 \\ 
	%%&ResNet101& 0.8848 & 0.8327 & 0.7999 & 0.8116 & 0.8308 & 0.8702 & 0.8209 & 0.8619 & 0.8686 \\ 
	%%&ResNet152& 0.9138 & 0.9018 & 0.93 & 0.9404 & 0.8967 & 0.9611 & 0.9383 & 0.9398 & 0.9674 \\ 
	%%\midrule
	%%\multirow{5}{*}{\tabincell{c}{\(\nu = 10\)}} &ResNet18 & 0.589 & 0.6309 & 0.6042 & 0.5906 & 0.5789 & 0.6877 & 0.6668 & 0.6177 & 0.6394 \\ 
	%%&ResNet34 & 0.6453 & 0.6706 & 0.6594 & 0.6964 & 0.7092 & 0.656 & 0.6252 & 0.7334 & 0.6432 \\ 
	%%&ResNet50& 0.7515 & 0.8467 & 0.8171 & 0.8244 & 0.7262 & 0.8221 & 0.7303 & 0.8349 & 0.8324 \\ 
	%%&ResNet101& 0.8541 & 0.8471 & 0.7916 & 0.8095 & 0.8376 & 0.8767 & 0.8387 & 0.8852 & 0.8191 \\ 
	%%&ResNet152& 0.9466 & 0.9298 & 0.9085 & 0.9422 & 0.8999 & 0.955 & 0.8973 & 0.9356 & 0.9632 \\ 
	%%\midrule
	%%\multirow{5}{*}{\tabincell{c}{\(\nu = 15\)}} &ResNet18 & 0.6287 & 0.65 & 0.6764 & 0.5649 & 0.6416 & 0.6561 & 0.6171 & 0.5872 & 0.6241 \\ 
	%%&ResNet34 & 0.6858 & 0.6441 & 0.6002 & 0.7455 & 0.6458 & 0.7373 & 0.6514 & 0.6688 & 0.6818 \\ 
	%%&ResNet50& 0.7905 & 0.7265 & 0.8174 & 0.7917 & 0.8329 & 0.8185 & 0.747 & 0.7973 & 0.7426 \\ 
	%%&ResNet101& 0.8759 & 0.8617 & 0.818 & 0.831 & 0.8311 & 0.8758 & 0.851 & 0.8211 & 0.7953 \\ 
	%%&ResNet152& 0.9489 & 0.9297 & 0.9536 & 0.9675 & 0.9317 & 0.8969 & 0.8969 & 0.9448 & 0.9355 \\ 
	%%\midrule
	%%\multirow{5}{*}{\tabincell{c}{\(\nu = 20\)}}&ResNet18 & 0.6728 & 0.6643 & 0.5564 & 0.6117 & 0.6955 & 0.6514 & 0.6436 & 0.5611 & 0.615 \\ 
	%%&ResNet34 & 0.6211 & 0.6503 & 0.7333 & 0.7185 & 0.6632 & 0.6658 & 0.6169 & 0.6492 & 0.6212 \\ 
	%%&ResNet50& 0.7214 & 0.7926 & 0.8427 & 0.771 & 0.7949 & 0.7847 & 0.8286 & 0.7893 & 0.7573 \\ 
	%%&ResNet101& 0.8592 & 0.8896 & 0.8518 & 0.8587 & 0.8268 & 0.8226 & 0.8835 & 0.8445 & 0.7973 \\ 
	%%&ResNet152& 0.9007 & 0.9484 & 0.9175 & 0.909 & 0.9379 & 0.9238 & 0.9538 & 0.9459 & 0.9425 \\ 
	%%\bottomrule
	%%\end{tabular}
	%%}
%%\end{table} 


\subsubsection{Discriminant results based on IRP}
A prerequisite for discriminating interval-valued time series based on IRP is to determine the kernel function \(K(u, v)\) in the \(D_k\)-distance. We now explore some special choices of kernel \(K(u, v)\) and discuss their implication on capturing the information contained in intervals. For notational convenience, we denote a generic choice of a symmetric kernel 
\[
K = \left[
\begin{array}{cc}
	K(1,1) & K(1,-1)\\
	K(-1,1) & K(-1, -1)
\end{array}
\right]
\]
as \(K(1; 1) = a, K(1; -1) = K(-1; 1) = b, K(-1; -1) = c\), where \(a, b\) and \(c\) satisfy the positive definite condition in Section \ref{sec3}. Following \citet{han2012autoregressive}, we choose the following three kernel functions for IRP-based interval vector-valued time series discriminations,
\[
K_1 = \left[
\begin{array}{cc}
	1/4 & -1/4\\
	-1/4 & 1/4
\end{array}
\right], \ K_2 = \left[
\begin{array}{cc}
	1 & 1\\
	1 & 1
\end{array}
\right], \ K_3 = \left[
\begin{array}{cc}
	1/2 & 1/4\\
	1/4 & 1/2
\end{array}
\right].
\]

The following three tables show the discriminant results of IRP-based interval-valued time series based on different kernel functions and network depths.

\begin{table}[H]
	\footnotesize
	\setlength{\abovecaptionskip}{0pt}%
	\setlength{\belowcaptionskip}{3pt}%
	\centering
	\caption{Univariate interval-valued time series discriminant results based on IRP}
	\setlength{\tabcolsep}{2mm}{
		\begin{tabular}{ccccccccccc}
			\toprule
			DGP& kernel & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
			\midrule
			\multirow{3}{*}{\tabincell{c}{DGP1}} &\(K_1\) & 0.6428 & 0.6604 & 0.6674 & 0.6961 & 0.6898 & 0.6966 & 0.6134 & 0.663 & 0.6681 \\ 
			&\(K_2\)& 0.7124 & 0.6759 & 0.6815 & 0.7381 & 0.6846 & 0.7285 & 0.6645 & 0.6663 & 0.665 \\ 
			&\(K_3\)& 0.8272 & 0.8042 & 0.8033 & 0.8002 & 0.8181 & 0.8115 & 0.8137 & 0.8181 & 0.8357 \\ 
			\midrule
			\multirow{3}{*}{\tabincell{c}{DGP2}} &\(K_1\) & 0.603 & 0.631 & 0.6784 & 0.6649 & 0.6142 & 0.6489 & 0.6922 & 0.6244 & 0.6393 \\ 
			&\(K_2\) & 0.6785 & 0.6575 & 0.6832 & 0.7435 & 0.7498 & 0.6958 & 0.7255 & 0.6761 & 0.7428 \\ 
			&\(K_3\)& 0.811 & 0.8044 & 0.8429 & 0.8252 & 0.8212 & 0.8365 & 0.8363 & 0.8498 & 0.8267 \\
			\midrule
			\multirow{3}{*}{\tabincell{c}{DGP3}} &\(K_1\) & 0.6548 & 0.6085 & 0.6964 & 0.6335 & 0.692 & 0.6255 & 0.6309 & 0.6487 & 0.6 \\ 
			&\(K_2\) & 0.6763 & 0.7051 & 0.6824 & 0.706 & 0.7101 & 0.6766 & 0.716 & 0.6534 & 0.6768 \\ 
			&\(K_3\)& 0.8071 & 0.8001 & 0.8265 & 0.826 & 0.832 & 0.8285 & 0.8494 & 0.8248 & 0.8312 \\
			\bottomrule
		\end{tabular}
	}
\end{table}


%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Univariate interval-valued time series (DGP1) discriminant results based on IRP}
%\setlength{\tabcolsep}{2mm}{  
	%\begin{tabular}{clccccccccc}
	%\toprule
	%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_1\)}}  &ResNet18 & 0.6918 & 0.6858 & 0.6735 & 0.6665 & 0.6636 & 0.6881 & 0.6794 & 0.6836 & 0.67 \\ 
	%&ResNet34 & 0.7322 & 0.7329 & 0.7409 & 0.7484 & 0.7441 & 0.7406 & 0.7477 & 0.7496 & 0.735 \\ 
	%&ResNet50& 0.8305 & 0.8115 & 0.831 & 0.8173 & 0.8411 & 0.8015 & 0.8195 & 0.8128 & 0.8186 \\ 
	%&ResNet101& 0.8585 & 0.8639 & 0.8782 & 0.8865 & 0.8521 & 0.8374 & 0.8628 & 0.8707 & 0.8566 \\ 
	%&ResNet152& 0.9568 & 0.9616 & 0.9667 & 0.9529 & 0.938 & 0.9336 & 0.9309 & 0.9353 & 0.9408 \\ 
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_1\)}} &ResNet18 & 0.6933 & 0.6791 & 0.6609 & 0.6901 & 0.6781 & 0.6735 & 0.6642 & 0.6605 & 0.6757 \\ 
	%&ResNet34 & 0.7374 & 0.7316 & 0.7338 & 0.7349 & 0.7465 & 0.7487 & 0.7348 & 0.7434 & 0.7456 \\ 
	%&ResNet50& 0.8483 & 0.8333 & 0.8006 & 0.8236 & 0.8267 & 0.8452 & 0.8237 & 0.8121 & 0.8077 \\ 
	%&ResNet101& 0.8499 & 0.8798 & 0.8709 & 0.8468 & 0.8894 & 0.8504 & 0.8511 & 0.8486 & 0.8543 \\ 
	%&ResNet152& 0.952 & 0.9418 & 0.9604 & 0.9675 & 0.94 & 0.9492 & 0.9588 & 0.9698 & 0.9668 \\ 
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_3\)}}&ResNet18 & 0.6866 & 0.6898 & 0.6974 & 0.6714 & 0.669 & 0.6609 & 0.6782 & 0.6834 & 0.6618 \\ 
	%&ResNet34 & 0.7388 & 0.7465 & 0.7454 & 0.7397 & 0.7408 & 0.7319 & 0.7373 & 0.7438 & 0.7397 \\ 
	%&ResNet50& 0.8179 & 0.8145 & 0.8187 & 0.8192 & 0.8462 & 0.8279 & 0.8048 & 0.8282 & 0.8385 \\ 
	%&ResNet101& 0.8386 & 0.8689 & 0.8704 & 0.864 & 0.857 & 0.8403 & 0.836 & 0.8859 & 0.8341 \\ 
	%&ResNet152& 0.9412 & 0.9505 & 0.9528 & 0.9411 & 0.954 & 0.9691 & 0.945 & 0.9423 & 0.9564 \\
	%\bottomrule
	%\end{tabular}
	%}
%\end{table}
%
%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Univariate interval-valued time series (DGP2) discriminant results based on IRP}
%\setlength{\tabcolsep}{2mm}{  
	%\begin{tabular}{clccccccccc}
	%\toprule
	%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_1\)}} &ResNet18 & 0.6782 & 0.6636 & 0.6739 & 0.6787 & 0.6655 & 0.6815 & 0.6959 & 0.6856 & 0.6876 \\ 
	%&ResNet34 & 0.7495 & 0.7444 & 0.7478 & 0.7376 & 0.7313 & 0.7428 & 0.7369 & 0.7311 & 0.7334 \\ 
	%&ResNet50& 0.8205 & 0.816 & 0.8028 & 0.8489 & 0.8205 & 0.8293 & 0.8046 & 0.8321 & 0.8315 \\ 
	%&ResNet101& 0.8437 & 0.8578 & 0.8622 & 0.8806 & 0.842 & 0.8895 & 0.8361 & 0.8837 & 0.8446 \\ 
	%&ResNet152& 0.9444 & 0.9544 & 0.9345 & 0.937 & 0.9507 & 0.9484 & 0.933 & 0.9662 & 0.9662 \\ 
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_1\)}} &ResNet18 & 0.6809 & 0.6977 & 0.6779 & 0.6912 & 0.6936 & 0.6664 & 0.6878 & 0.6906 & 0.6691 \\ 
	%&ResNet34 & 0.7405 & 0.7388 & 0.7448 & 0.7467 & 0.7312 & 0.7438 & 0.7456 & 0.7434 & 0.7313 \\ 
	%&ResNet50& 0.8083 & 0.8105 & 0.8062 & 0.8265 & 0.8481 & 0.808 & 0.835 & 0.8156 & 0.8084 \\ 
	%&ResNet101& 0.8763 & 0.8521 & 0.876 & 0.8339 & 0.8735 & 0.8816 & 0.8384 & 0.8738 & 0.8472 \\ 
	%&ResNet152& 0.9627 & 0.9677 & 0.9394 & 0.947 & 0.953 & 0.9418 & 0.9539 & 0.9698 & 0.9514 \\ 
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_3\)}} &ResNet18 & 0.683 & 0.6896 & 0.6864 & 0.6761 & 0.6861 & 0.6688 & 0.665 & 0.6718 & 0.6869 \\ 
	%&ResNet34 & 0.7336 & 0.7445 & 0.7429 & 0.7458 & 0.7305 & 0.7359 & 0.7446 & 0.7447 & 0.7387 \\ 
	%&ResNet50& 0.8471 & 0.8268 & 0.8401 & 0.8119 & 0.834 & 0.8099 & 0.8219 & 0.8265 & 0.8265 \\ 
	%&ResNet101& 0.8341 & 0.8317 & 0.8616 & 0.8587 & 0.8758 & 0.8508 & 0.8431 & 0.8644 & 0.8548 \\ 
	%&ResNet152& 0.9679 & 0.9401 & 0.9395 & 0.9406 & 0.9502 & 0.9664 & 0.958 & 0.9317 & 0.9479 \\ 
	%\bottomrule
	%\end{tabular}
	%}
%\end{table}
%
%
%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Univariate interval-valued time series (DGP3) discriminant results based on IRP}
%\setlength{\tabcolsep}{2mm}{  
	%\begin{tabular}{clccccccccc}
	%\toprule
	%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_1\)}} &ResNet18 & 0.6806 & 0.6803 & 0.6671 & 0.6765 & 0.6691 & 0.674 & 0.6695 & 0.6901 & 0.6643 \\ 
	%&ResNet34 & 0.7404 & 0.7443 & 0.7451 & 0.7466 & 0.7359 & 0.7336 & 0.7482 & 0.7421 & 0.7484 \\ 
	%&ResNet50& 0.8155 & 0.8399 & 0.8285 & 0.8174 & 0.8421 & 0.836 & 0.8426 & 0.8366 & 0.8159 \\ 
	%&ResNet101& 0.8865 & 0.8452 & 0.8401 & 0.8468 & 0.8787 & 0.8331 & 0.8334 & 0.863 & 0.8823 \\ 
	%&ResNet152& 0.933 & 0.9606 & 0.9684 & 0.9676 & 0.9349 & 0.9613 & 0.9621 & 0.9572 & 0.9603 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_1\)}} &ResNet18 & 0.6769 & 0.6818 & 0.6908 & 0.6848 & 0.6982 & 0.6745 & 0.6921 & 0.6793 & 0.6971 \\ 
	%&ResNet34 & 0.7468 & 0.7312 & 0.7373 & 0.7388 & 0.732 & 0.7412 & 0.7475 & 0.7399 & 0.7309 \\ 
	%&ResNet50& 0.8098 & 0.8427 & 0.8038 & 0.8361 & 0.8112 & 0.8364 & 0.813 & 0.8374 & 0.8073 \\ 
	%&ResNet101& 0.8859 & 0.8831 & 0.8623 & 0.8749 & 0.8707 & 0.8396 & 0.8663 & 0.8564 & 0.8576 \\ 
	%&ResNet152& 0.9658 & 0.9454 & 0.9673 & 0.9518 & 0.9626 & 0.9547 & 0.9606 & 0.9312 & 0.9554 \\ 
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_3\)}} &ResNet18 & 0.6843 & 0.6903 & 0.6705 & 0.6626 & 0.6683 & 0.6964 & 0.6684 & 0.6725 & 0.6952 \\ 
	%&ResNet34 & 0.7418 & 0.7468 & 0.7496 & 0.7372 & 0.74 & 0.7338 & 0.7497 & 0.7327 & 0.7326 \\ 
	%&ResNet50& 0.8026 & 0.8492 & 0.8297 & 0.8237 & 0.8327 & 0.8095 & 0.8215 & 0.8295 & 0.8104 \\ 
	%&ResNet101& 0.8329 & 0.8872 & 0.8766 & 0.8732 & 0.8387 & 0.8622 & 0.8564 & 0.8584 & 0.8328 \\ 
	%&ResNet152& 0.9455 & 0.9629 & 0.9505 & 0.963 & 0.937 & 0.9376 & 0.9471 & 0.942 & 0.9635 \\ 
	%\bottomrule
	%\end{tabular}
	%}
%\end{table}






\subsection{Interval vector-valued time series discriminant}
% 注意:对此处进行修改, 与实验一致.
By using the DGPs of univariate interval-valued time series in Subsection \ref{ss1}, we construct the following two interval vector-valued time series generation processes. Specifically, in the first case (case 1), we repeatedly generate DGP1 three times as three dimensions of the interval vector-valued time series, respectively, and different correlation coefficients \(\rho\) denote different classes. In the second case (case 2), we generate DGP1, DGP2 and DGP3 as three dimensions of the interval vector-valued time series, respectively, and again, different correlation coefficients \(\rho\) denote different classes. As with the univariate interval-valued time series, the interval vector-valued time series in both cases above also contain nine classes. We choose the same kernel functions as in Subsection \ref{ss1} for interval vector-valued time series imaging and discrimination. The following four tables show the discriminant results of interval vector-valued time series based on JRP and IJRP for the two cases, respectively.


\begin{table}[H]
	\footnotesize
	\setlength{\abovecaptionskip}{0pt}%
	\setlength{\belowcaptionskip}{3pt}%
	\centering
	\caption{Interval vector-valued time series discriminant results based on JRP}
	\setlength{\tabcolsep}{2mm}{
		\begin{tabular}{ccccccccccc}
			\toprule
			DGP& \(\nu\) & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
			\midrule
			\multirow{5}{*}{\tabincell{c}{C1}} &\(\nu = 1\) & 0.6428 & 0.6604 & 0.6674 & 0.6961 & 0.6898 & 0.6966 & 0.6134 & 0.663 & 0.6681 \\ 
			&\(\nu = 5\)& 0.7124 & 0.6759 & 0.6815 & 0.7381 & 0.6846 & 0.7285 & 0.6645 & 0.6663 & 0.665 \\ 
			&\(\nu = 10\)& 0.8272 & 0.8042 & 0.8033 & 0.8002 & 0.8181 & 0.8115 & 0.8137 & 0.8181 & 0.8357 \\ 
			&\(\nu = 15\)& 0.8481 & 0.8446 & 0.8692 & 0.8591 & 0.8441 & 0.8564 & 0.8868 & 0.8733 & 0.8605 \\ 
			&\(\nu = 20\)& 0.9526 & 0.9457 & 0.9436 & 0.9254 & 0.93 & 0.9663 & 0.9017 & 0.9139 & 0.9249 \\ 
			\midrule
			\multirow{5}{*}{\tabincell{c}{C2}} &\(\nu = 1\) & 0.603 & 0.631 & 0.6784 & 0.6649 & 0.6142 & 0.6489 & 0.6922 & 0.6244 & 0.6393 \\ 
			&\(\nu = 5\) & 0.6785 & 0.6575 & 0.6832 & 0.7435 & 0.7498 & 0.6958 & 0.7255 & 0.6761 & 0.7428 \\ 
			&\(\nu = 10\)& 0.811 & 0.8044 & 0.8429 & 0.8252 & 0.8212 & 0.8365 & 0.8363 & 0.8498 & 0.8267 \\ 
			&\(\nu = 15\)& 0.855 & 0.8541 & 0.8471 & 0.8465 & 0.8447 & 0.8685 & 0.8406 & 0.8897 & 0.8719 \\ 
			&\(\nu = 20\)& 0.94 & 0.9174 & 0.9524 & 0.9195 & 0.9607 & 0.9128 & 0.9069 & 0.9674 & 0.9383 \\
			\bottomrule
		\end{tabular}
	}
\end{table}


\begin{table}[H]
	\footnotesize
	\setlength{\abovecaptionskip}{0pt}%
	\setlength{\belowcaptionskip}{3pt}%
	\centering
	\caption{Interval vector-valued time series discriminant results based on IJRP}
	\setlength{\tabcolsep}{2mm}{
		\begin{tabular}{ccccccccccc}
			\toprule
			DGP& kernel & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
			\midrule
			\multirow{3}{*}{\tabincell{c}{C1}} &\(K_1\) & 0.6428 & 0.6604 & 0.6674 & 0.6961 & 0.6898 & 0.6966 & 0.6134 & 0.663 & 0.6681 \\ 
			&\(K_2\)& 0.7124 & 0.6759 & 0.6815 & 0.7381 & 0.6846 & 0.7285 & 0.6645 & 0.6663 & 0.665 \\ 
			&\(K_3\)& 0.8272 & 0.8042 & 0.8033 & 0.8002 & 0.8181 & 0.8115 & 0.8137 & 0.8181 & 0.8357 \\ 
			\midrule
			\multirow{3}{*}{\tabincell{c}{C1}} &\(K_1\) & 0.603 & 0.631 & 0.6784 & 0.6649 & 0.6142 & 0.6489 & 0.6922 & 0.6244 & 0.6393 \\ 
			&\(K_2\) & 0.6785 & 0.6575 & 0.6832 & 0.7435 & 0.7498 & 0.6958 & 0.7255 & 0.6761 & 0.7428 \\ 
			&\(K_3\)& 0.811 & 0.8044 & 0.8429 & 0.8252 & 0.8212 & 0.8365 & 0.8363 & 0.8498 & 0.8267 \\
			\bottomrule
		\end{tabular}
	}
\end{table}



%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Interval vector-valued time series (case 1) discriminant results based on JRP}
%\setlength{\tabcolsep}{2mm}{  
	%\begin{tabular}{clccccccccc}
	%\toprule
	%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 1\)}} &ResNet18 & 0.6781 & 0.6647 & 0.6843 & 0.6903 & 0.6785 & 0.6695 & 0.6955 & 0.697 & 0.6749 \\ 
	%&ResNet34 & 0.7372 & 0.7406 & 0.7417 & 0.7367 & 0.7402 & 0.7466 & 0.7429 & 0.7456 & 0.7356 \\ 
	%&ResNet50& 0.8045 & 0.8228 & 0.8152 & 0.8078 & 0.8131 & 0.8435 & 0.8148 & 0.8042 & 0.8403 \\ 
	%&ResNet101& 0.8382 & 0.8505 & 0.8327 & 0.8532 & 0.8808 & 0.8824 & 0.8869 & 0.8535 & 0.8806 \\ 
	%&ResNet152& 0.9429 & 0.9579 & 0.9542 & 0.9421 & 0.9415 & 0.956 & 0.9426 & 0.9304 & 0.945 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 5\)}} &ResNet18 & 0.6916 & 0.6794 & 0.6962 & 0.6929 & 0.687 & 0.6928 & 0.6658 & 0.6736 & 0.6822 \\ 
	%&ResNet34 & 0.7471 & 0.7433 & 0.7379 & 0.7369 & 0.7337 & 0.7303 & 0.74 & 0.733 & 0.7457 \\ 
	%&ResNet50& 0.8249 & 0.8317 & 0.8144 & 0.814 & 0.8423 & 0.8254 & 0.8165 & 0.822 & 0.8377 \\ 
	%&ResNet101& 0.8894 & 0.8841 & 0.8884 & 0.8823 & 0.8325 & 0.8345 & 0.8415 & 0.879 & 0.8864 \\ 
	%&ResNet152& 0.9567 & 0.9542 & 0.9327 & 0.9375 & 0.9364 & 0.9522 & 0.9345 & 0.9304 & 0.9327 \\ 
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 10\)}} &ResNet18 & 0.6957 & 0.6688 & 0.6741 & 0.6686 & 0.6672 & 0.663 & 0.6633 & 0.6908 & 0.6638 \\ 
	%&ResNet34 & 0.7352 & 0.73 & 0.741 & 0.7492 & 0.7308 & 0.7341 & 0.7307 & 0.74 & 0.7403 \\ 
	%&ResNet50& 0.8176 & 0.8432 & 0.8289 & 0.8117 & 0.8031 & 0.8444 & 0.8132 & 0.8191 & 0.838 \\ 
	%&ResNet101& 0.8629 & 0.8434 & 0.8698 & 0.853 & 0.855 & 0.8461 & 0.8708 & 0.8353 & 0.8574 \\ 
	%&ResNet152& 0.9602 & 0.9625 & 0.9476 & 0.9307 & 0.9589 & 0.952 & 0.9393 & 0.9698 & 0.9394 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 15\)}} &ResNet18 & 0.6694 & 0.6792 & 0.6886 & 0.6854 & 0.6607 & 0.6727 & 0.6822 & 0.6871 & 0.6846 \\ 
	%&ResNet34 & 0.7395 & 0.7432 & 0.7384 & 0.7314 & 0.7329 & 0.7355 & 0.7305 & 0.7324 & 0.7374 \\ 
	%&ResNet50& 0.8299 & 0.8445 & 0.8255 & 0.8361 & 0.8487 & 0.8296 & 0.8251 & 0.8053 & 0.8107 \\ 
	%&ResNet101& 0.859 & 0.8553 & 0.8582 & 0.8887 & 0.8321 & 0.8716 & 0.8753 & 0.8711 & 0.8462 \\ 
	%&ResNet152& 0.967 & 0.9671 & 0.9454 & 0.9497 & 0.9686 & 0.9423 & 0.9688 & 0.9626 & 0.9651 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 20\)}} &ResNet18 & 0.6922 & 0.6808 & 0.6985 & 0.675 & 0.6636 & 0.6753 & 0.6736 & 0.6697 & 0.6841 \\ 
	%&ResNet34 & 0.7324 & 0.7449 & 0.7311 & 0.738 & 0.7399 & 0.7457 & 0.7339 & 0.7306 & 0.7446 \\ 
	%&ResNet50& 0.8415 & 0.8066 & 0.8103 & 0.8095 & 0.8025 & 0.8275 & 0.8194 & 0.8123 & 0.8285 \\ 
	%&ResNet101& 0.8752 & 0.8819 & 0.8857 & 0.887 & 0.8838 & 0.8435 & 0.8611 & 0.8807 & 0.8593 \\ 
	%&ResNet152& 0.945 & 0.9562 & 0.961 & 0.9484 & 0.9532 & 0.9579 & 0.9512 & 0.9354 & 0.9488 \\ 
	%\bottomrule
	%\end{tabular}
	%}
%\end{table}


%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Interval vector-valued time series (case 2) discriminant results based on JRP}
%\setlength{\tabcolsep}{2mm}{  
	%\begin{tabular}{clccccccccc}
	%\toprule
	%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 1\)}}  &ResNet18 & 0.6314 & 0.6318 & 0.6201 & 0.642 & 0.6372 & 0.6052 & 0.6349 & 0.6047 & 0.6008 \\ 
	%&ResNet34 & 0.7077 & 0.7399 & 0.7072 & 0.7214 & 0.7125 & 0.7308 & 0.7204 & 0.7256 & 0.7259 \\ 
	%&ResNet50& 0.8158 & 0.76 & 0.8249 & 0.8282 & 0.756 & 0.7783 & 0.8084 & 0.7956 & 0.7802 \\ 
	%&ResNet101& 0.8538 & 0.8455 & 0.8551 & 0.8575 & 0.8574 & 0.842 & 0.859 & 0.845 & 0.8556 \\ 
	%&ResNet152& 0.9041 & 0.9099 & 0.9172 & 0.9182 & 0.9062 & 0.9051 & 0.9164 & 0.9046 & 0.9163 \\ 
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 5\)}} &ResNet18 & 0.645 & 0.6177 & 0.6335 & 0.6323 & 0.639 & 0.6471 & 0.6026 & 0.6369 & 0.6058 \\ 
	%&ResNet34 & 0.7286 & 0.7278 & 0.7118 & 0.7331 & 0.7295 & 0.7193 & 0.7141 & 0.7329 & 0.7369 \\ 
	%&ResNet50& 0.7975 & 0.7671 & 0.7909 & 0.778 & 0.8036 & 0.7583 & 0.8041 & 0.7631 & 0.7537 \\ 
	%&ResNet101& 0.8536 & 0.8567 & 0.8401 & 0.8556 & 0.8536 & 0.8404 & 0.8424 & 0.8562 & 0.8413 \\ 
	%&ResNet152& 0.9149 & 0.9033 & 0.9113 & 0.9028 & 0.9155 & 0.9009 & 0.9164 & 0.9191 & 0.9065 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 10\)}} &ResNet18 & 0.609 & 0.6056 & 0.6118 & 0.6361 & 0.6181 & 0.6365 & 0.6199 & 0.6138 & 0.6472 \\ 
	%&ResNet34 & 0.712 & 0.7034 & 0.7308 & 0.726 & 0.7157 & 0.7193 & 0.7061 & 0.7355 & 0.7324 \\ 
	%&ResNet50& 0.8277 & 0.7829 & 0.7992 & 0.8102 & 0.801 & 0.7925 & 0.7918 & 0.8223 & 0.8178 \\ 
	%&ResNet101& 0.8578 & 0.8565 & 0.8546 & 0.8519 & 0.8437 & 0.8531 & 0.8449 & 0.8571 & 0.8588 \\ 
	%&ResNet152& 0.9104 & 0.9175 & 0.9087 & 0.9107 & 0.9 & 0.9134 & 0.9093 & 0.9155 & 0.9188 \\ 
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 15\)}} &ResNet18 & 0.6143 & 0.644 & 0.6239 & 0.6473 & 0.6068 & 0.6484 & 0.6475 & 0.605 & 0.641 \\ 
	%&ResNet34 & 0.7109 & 0.7129 & 0.7183 & 0.7092 & 0.7325 & 0.7253 & 0.7115 & 0.7271 & 0.7389 \\ 
	%&ResNet50& 0.7737 & 0.8245 & 0.7542 & 0.7521 & 0.8105 & 0.7774 & 0.7907 & 0.8099 & 0.7596 \\ 
	%&ResNet101& 0.8598 & 0.845 & 0.8518 & 0.8592 & 0.8573 & 0.8455 & 0.8491 & 0.8538 & 0.8482 \\ 
	%&ResNet152& 0.9053 & 0.9179 & 0.9169 & 0.9135 & 0.9113 & 0.9158 & 0.9016 & 0.9052 & 0.9055 \\ 
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 20\)}} &ResNet18 & 0.6143 & 0.644 & 0.6239 & 0.6473 & 0.6068 & 0.6484 & 0.6475 & 0.605 & 0.641 \\ 
	%&ResNet34 & 0.7109 & 0.7129 & 0.7183 & 0.7092 & 0.7325 & 0.7253 & 0.7115 & 0.7271 & 0.7389 \\ 
	%&ResNet50& 0.7737 & 0.8245 & 0.7542 & 0.7521 & 0.8105 & 0.7774 & 0.7907 & 0.8099 & 0.7596 \\ 
	%&ResNet101& 0.8598 & 0.845 & 0.8518 & 0.8592 & 0.8573 & 0.8455 & 0.8491 & 0.8538 & 0.8482 \\ 
	%&ResNet152& 0.9053 & 0.9179 & 0.9169 & 0.9135 & 0.9113 & 0.9158 & 0.9016 & 0.9052 & 0.9055 \\ 
	%\bottomrule
	%\end{tabular}
	%}
%\end{table}
%
%
%
%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Interval vector-valued time series (case 1) discriminant results based on IJRP}
%\setlength{\tabcolsep}{2mm}{  
	%\begin{tabular}{clccccccccc}
	%\toprule
	%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_1\)}}&ResNet18 & 0.6286 & 0.615 & 0.6302 & 0.6422 & 0.6338 & 0.6318 & 0.6051 & 0.6351 & 0.6186 \\ 
	%&ResNet34 & 0.7304 & 0.7226 & 0.7082 & 0.7292 & 0.7273 & 0.7152 & 0.733 & 0.7378 & 0.7084 \\ 
	%&ResNet50& 0.8068 & 0.8256 & 0.8298 & 0.817 & 0.8273 & 0.8105 & 0.8246 & 0.7768 & 0.7667 \\ 
	%&ResNet101& 0.8514 & 0.8563 & 0.8464 & 0.8442 & 0.8512 & 0.8426 & 0.8488 & 0.8497 & 0.86 \\ 
	%&ResNet152& 0.9053 & 0.9018 & 0.9125 & 0.9146 & 0.9077 & 0.9071 & 0.9041 & 0.919 & 0.9097 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_2\)}}&ResNet18 & 0.603 & 0.6431 & 0.6092 & 0.6055 & 0.6482 & 0.6237 & 0.6452 & 0.6201 & 0.6132 \\ 
	%&ResNet34 & 0.7203 & 0.7279 & 0.7104 & 0.7263 & 0.7181 & 0.7252 & 0.7082 & 0.7067 & 0.7317 \\ 
	%&ResNet50& 0.7548 & 0.8246 & 0.8294 & 0.7543 & 0.7612 & 0.7781 & 0.7998 & 0.8234 & 0.8272 \\ 
	%&ResNet101& 0.8542 & 0.855 & 0.8527 & 0.8492 & 0.8455 & 0.841 & 0.8537 & 0.8441 & 0.8402 \\ 
	%&ResNet152& 0.9011 & 0.92 & 0.9047 & 0.9093 & 0.9071 & 0.9111 & 0.9036 & 0.902 & 0.9066 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_3\)}}&ResNet18 & 0.6279 & 0.6333 & 0.6365 & 0.6044 & 0.6385 & 0.6361 & 0.6407 & 0.6358 & 0.6245 \\ 
	%&ResNet34 & 0.722 & 0.7223 & 0.7396 & 0.7051 & 0.7314 & 0.725 & 0.7015 & 0.7062 & 0.7233 \\ 
	%&ResNet50& 0.8224 & 0.7684 & 0.8045 & 0.7707 & 0.782 & 0.7803 & 0.7674 & 0.769 & 0.8144 \\ 
	%&ResNet101& 0.8484 & 0.8452 & 0.8543 & 0.8541 & 0.8588 & 0.8452 & 0.8585 & 0.8494 & 0.844 \\ 
	%&ResNet152& 0.9163 & 0.9173 & 0.9 & 0.9156 & 0.9118 & 0.9135 & 0.9036 & 0.901 & 0.9095 \\ 
	%\bottomrule
	%\end{tabular}
	%}
%\end{table}
%
%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Interval vector-valued time series (case 2) discriminant results based on IJRP}
%\setlength{\tabcolsep}{2mm}{  
	%\begin{tabular}{clccccccccc}
	%\toprule
	%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_1\)}}&ResNet18 & 0.6068 & 0.6241 & 0.6189 & 0.6157 & 0.6474 & 0.6135 & 0.6323 & 0.6393 & 0.634 \\ 
	%&ResNet34 & 0.7329 & 0.7186 & 0.7222 & 0.7319 & 0.7011 & 0.7162 & 0.701 & 0.7343 & 0.7117 \\ 
	%&ResNet50& 0.7556 & 0.7748 & 0.7701 & 0.7921 & 0.8065 & 0.8129 & 0.7678 & 0.7948 & 0.8106 \\ 
	%&ResNet101& 0.8564 & 0.8444 & 0.8472 & 0.8584 & 0.8495 & 0.8524 & 0.8487 & 0.8517 & 0.8464 \\ 
	%&ResNet152& 0.9012 & 0.9072 & 0.9084 & 0.9143 & 0.9122 & 0.9024 & 0.9093 & 0.9011 & 0.9171 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_2\)}}&ResNet18 & 0.6112 & 0.6211 & 0.6427 & 0.6192 & 0.6158 & 0.611 & 0.6437 & 0.6374 & 0.6031 \\ 
	%&ResNet34 & 0.7364 & 0.7072 & 0.707 & 0.7213 & 0.7167 & 0.7254 & 0.7207 & 0.7066 & 0.7031 \\ 
	%&ResNet50& 0.7508 & 0.8042 & 0.812 & 0.8275 & 0.754 & 0.798 & 0.7698 & 0.821 & 0.8038 \\ 
	%&ResNet101& 0.8414 & 0.8515 & 0.8479 & 0.8538 & 0.8557 & 0.8577 & 0.854 & 0.8563 & 0.8586 \\ 
	%&ResNet152& 0.9177 & 0.9004 & 0.9107 & 0.9047 & 0.909 & 0.9198 & 0.9154 & 0.912 & 0.9086 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_3\)}}&ResNet18 & 0.6138 & 0.6303 & 0.638 & 0.6232 & 0.6383 & 0.6416 & 0.6254 & 0.6196 & 0.617 \\ 
	%&ResNet34 & 0.7306 & 0.7385 & 0.715 & 0.7374 & 0.7352 & 0.7256 & 0.7027 & 0.7364 & 0.7331 \\ 
	%&ResNet50& 0.7865 & 0.7578 & 0.8113 & 0.7507 & 0.7554 & 0.8289 & 0.7817 & 0.7837 & 0.764 \\ 
	%&ResNet101& 0.8518 & 0.8539 & 0.8414 & 0.8597 & 0.8454 & 0.8583 & 0.8473 & 0.8484 & 0.8551 \\ 
	%&ResNet152& 0.9154 & 0.9128 & 0.9031 & 0.9168 & 0.9177 & 0.9073 & 0.9091 & 0.9168 & 0.9023 \\ 
	%
	%\midrule
	%\bottomrule
	%\end{tabular}
	%}
%\end{table}



\section{Real Data Examples}\label{sec6}
Some existing methods \cite{Utkin2016, Wang2017} for interval-valued time series discrimination in the context of real data studies employ an approach that fuzzes the real point-valued time series to construct the desired interval-valued time series. The weakness of these methods is the inclusion of some artificial design and random ingredients in the interval construction, hence the merit of the proposed methods in real data could not be verified. In the following we verify the effectiveness of the proposed method in terms of natural interval-valued time series.

The real data we use from the website \url{https://rp5.ru/}. The website contains all weather data for 241 countries and regions worldwide since the beginning of records. In addition, the site provides weather forecasts and information for the coming seven days, with the latest data added to the site database at three-hour increments, i.e.,at an intensity of eight times daily. The website records a total of 28 weather indicators, six of which we selected for subsequent discriminant analysis. These six indicators are: atmospheric temperature above two meters above the ground (in degrees Celsius), atmospheric pressure at the level of the weather station (mmHg), atmospheric pressure at mean sea level (mmHg), relative humidity at two meters above the ground (\%), average wind speed at 10-12 meters above the ground during the ten minutes before the observation (m/s), and dew point temperature (in degrees Celsius) at two meters above the ground. 

% https://rp5.ru/ 从该网站选取最近十年的数据, 以天为单位来压缩数据, 构建区间数据来判别
% 三个月的数据为一个观测
% 选取哈尔滨, 三亚, 太原和北京四座城市的数据
% 哈尔滨-三亚,  三亚-太原-北京, 哈尔滨-三亚-太原-北京, 三种场景

% 将要的建模的变量, 共选取六个个指标, 按照顺序: 
% T at 2 metre height above the earth's surface
% P0 atmospheric pressure at weather station level (millimeters of mercury)
% P atmospheric pressure reduced to mean sea level (millimeters of mercury)
% relative humidity (%) at a height of 2 metres above the earth's surface
%
% T Po P U Ff Td
%地面两米以上大气温度（摄氏度）、气象站水平的大气压（毫米汞柱）、平均海平面的大气压（毫米汞柱）、地面高度两米处的相对湿度、观察前十分钟内地面高度10-12米处的平均风速、地面高度两米处的露点温度
\subsection{Univariate interval-valued time series discriminant} \label{sec61}
We compress the point-valued time series into interval-valued time series in units of days, and take the maximum and minimum values of the observed indicators of a day as the upper and lower bounds of the interval. After obtaining the interval-valued time series, we treat the 30-day observations as a trajectory for discriminating. We select Harbin (H) and Beijing (B) in northern China, Taiyuan (T) in central China, and Sanya (S) in southern China as four classes, respectively. There are three combinations specifically considered for discrimination, H-S, S-T-B, and H-S-T-B. We construct the discriminant models for the above three combinations using the first weather indicator selected, temperature. 
% 在单变量区间值时间序列中我们将选取温度T来作为区间值变量用于判别

\subsubsection{Discriminant results based on RP} 
The selection of the smooth parameter \(\nu\) and the discriminant model structure as in the Section \ref{sec5}, and the discrimination results corresponding to the three combinations are shown in the following three tables.

%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Univariate interval-valued time series (H-S) discriminant results based on RP}
%\setlength{\tabcolsep}{2mm}{  
	%\begin{tabular}{clccccccccc}
	%\toprule
	%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 1\)}}&ResNet18 & 0.7699 & 0.7874 & 0.7768 & 0.7613 & 0.7969 & 0.7733 & 0.7831 & 0.7694 & 0.7773 \\ 
	%&ResNet34 & 0.8176 & 0.8301 & 0.7926 & 0.8073 & 0.8032 & 0.7931 & 0.841 & 0.8166 & 0.844 \\ 
	%&ResNet50& 0.8574 & 0.8249 & 0.8859 & 0.8712 & 0.8629 & 0.8718 & 0.8761 & 0.8397 & 0.8077 \\ 
	%&ResNet101& 0.9297 & 0.9294 & 0.9272 & 0.9454 & 0.9224 & 0.9454 & 0.9395 & 0.9297 & 0.9385 \\ 
	%&ResNet152& 0.9543 & 0.9593 & 0.9542 & 0.9633 & 0.9563 & 0.9512 & 0.9515 & 0.9529 & 0.9573 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 5\)}}&ResNet18 & 0.7791 & 0.7835 & 0.7771 & 0.7864 & 0.7817 & 0.7713 & 0.787 & 0.7661 & 0.7625 \\ 
	%&ResNet34 & 0.8366 & 0.836 & 0.8534 & 0.805 & 0.8402 & 0.7986 & 0.8108 & 0.808 & 0.7903 \\ 
	%&ResNet50& 0.8105 & 0.8286 & 0.8112 & 0.8899 & 0.8489 & 0.894 & 0.8998 & 0.8757 & 0.888 \\ 
	%&ResNet101& 0.9244 & 0.9338 & 0.9308 & 0.9426 & 0.9323 & 0.9284 & 0.941 & 0.9428 & 0.9357 \\ 
	%&ResNet152& 0.9683 & 0.9632 & 0.9504 & 0.9699 & 0.9537 & 0.9555 & 0.9673 & 0.9576 & 0.9645 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 10\)}}&ResNet18 & 0.7522 & 0.7732 & 0.7729 & 0.7772 & 0.7517 & 0.756 & 0.7628 & 0.7619 & 0.7808 \\ 
	%&ResNet34 & 0.8169 & 0.8423 & 0.8167 & 0.8582 & 0.8012 & 0.8068 & 0.8212 & 0.8403 & 0.8281 \\ 
	%&ResNet50& 0.8415 & 0.8559 & 0.8447 & 0.8551 & 0.8011 & 0.8524 & 0.8712 & 0.8888 & 0.8136 \\ 
	%&ResNet101& 0.9276 & 0.9423 & 0.9475 & 0.9358 & 0.9322 & 0.9447 & 0.9486 & 0.9418 & 0.9477 \\ 
	%&ResNet152& 0.968 & 0.9602 & 0.9573 & 0.9508 & 0.9532 & 0.9517 & 0.9581 & 0.9564 & 0.968 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 15\)}}&ResNet18 & 0.7992 & 0.7595 & 0.7541 & 0.7799 & 0.7861 & 0.7662 & 0.7941 & 0.7987 & 0.7619 \\ 
	%&ResNet34 & 0.8365 & 0.8381 & 0.8298 & 0.8154 & 0.829 & 0.8247 & 0.8467 & 0.836 & 0.7904 \\ 
	%&ResNet50& 0.8313 & 0.8725 & 0.817 & 0.8918 & 0.8944 & 0.8126 & 0.8962 & 0.8691 & 0.8837 \\ 
	%&ResNet101& 0.9343 & 0.947 & 0.9202 & 0.9441 & 0.9296 & 0.9467 & 0.9336 & 0.9267 & 0.9462 \\ 
	%&ResNet152& 0.9597 & 0.9667 & 0.9603 & 0.9655 & 0.9617 & 0.9639 & 0.9631 & 0.9533 & 0.9526 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 20\)}}&ResNet18 & 0.7557 & 0.7621 & 0.7724 & 0.7552 & 0.7969 & 0.7557 & 0.7898 & 0.7765 & 0.7856 \\ 
	%&ResNet34 & 0.8041 & 0.816 & 0.8315 & 0.8024 & 0.8236 & 0.8457 & 0.8455 & 0.8135 & 0.8024 \\ 
	%&ResNet50& 0.8629 & 0.8637 & 0.8256 & 0.8948 & 0.8906 & 0.8948 & 0.8186 & 0.8213 & 0.8895 \\ 
	%&ResNet101& 0.9354 & 0.9349 & 0.9379 & 0.9201 & 0.936 & 0.9378 & 0.9421 & 0.9457 & 0.9315 \\ 
	%&ResNet152& 0.9554 & 0.9528 & 0.9518 & 0.9523 & 0.9696 & 0.9503 & 0.9691 & 0.964 & 0.9645 \\ 
	%	\bottomrule
	%\end{tabular}
	%}
%\end{table}
%
%
%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Univariate interval-valued time series (S-T-B) discriminant results based on RP}
%\setlength{\tabcolsep}{2mm}{  
	%\begin{tabular}{clccccccccc}
	%\toprule
	%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 1\)}}&ResNet18 & 0.7657 & 0.778 & 0.7988 & 0.7861 & 0.7804 & 0.7677 & 0.7712 & 0.7801 & 0.7669 \\ 
	%&ResNet34 & 0.8285 & 0.802 & 0.8452 & 0.8567 & 0.8079 & 0.833 & 0.7976 & 0.8176 & 0.8172 \\ 
	%&ResNet50& 0.8421 & 0.8644 & 0.8396 & 0.8144 & 0.8317 & 0.867 & 0.8236 & 0.8947 & 0.8617 \\ 
	%&ResNet101& 0.9237 & 0.9374 & 0.9492 & 0.9207 & 0.9235 & 0.9214 & 0.9233 & 0.9209 & 0.9496 \\ 
	%&ResNet152& 0.9683 & 0.9527 & 0.9657 & 0.9601 & 0.9661 & 0.9681 & 0.9535 & 0.961 & 0.9509 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 5\)}}&ResNet18 & 0.7643 & 0.7634 & 0.796 & 0.7912 & 0.7539 & 0.7534 & 0.7794 & 0.7895 & 0.7586 \\ 
	%&ResNet34 & 0.8593 & 0.817 & 0.86 & 0.8393 & 0.7917 & 0.8249 & 0.8145 & 0.8447 & 0.8124 \\ 
	%&ResNet50& 0.8215 & 0.8371 & 0.859 & 0.8156 & 0.8888 & 0.8585 & 0.8731 & 0.8524 & 0.8631 \\ 
	%&ResNet101& 0.9287 & 0.9275 & 0.9393 & 0.9246 & 0.9456 & 0.9202 & 0.9469 & 0.9227 & 0.9263 \\ 
	%&ResNet152& 0.9638 & 0.9659 & 0.9506 & 0.9586 & 0.9517 & 0.9607 & 0.9603 & 0.9581 & 0.9629 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 10\)}}&ResNet18 & 0.7978 & 0.7759 & 0.7513 & 0.7688 & 0.761 & 0.7506 & 0.7854 & 0.7742 & 0.765 \\ 
	%&ResNet34 & 0.823 & 0.7938 & 0.7923 & 0.8196 & 0.8421 & 0.8386 & 0.8108 & 0.8331 & 0.7907 \\ 
	%&ResNet50& 0.8547 & 0.8292 & 0.813 & 0.8753 & 0.863 & 0.8945 & 0.8692 & 0.8334 & 0.8384 \\ 
	%&ResNet101& 0.921 & 0.9465 & 0.9406 & 0.9343 & 0.9279 & 0.9408 & 0.9372 & 0.9388 & 0.9403 \\ 
	%&ResNet152& 0.9688 & 0.9681 & 0.9656 & 0.962 & 0.954 & 0.9649 & 0.9536 & 0.9592 & 0.9568 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 15\)}}&ResNet18 & 0.7673 & 0.772 & 0.7953 & 0.7903 & 0.7981 & 0.7838 & 0.7715 & 0.7731 & 0.7555 \\ 
	%&ResNet34 & 0.8325 & 0.8318 & 0.8276 & 0.8477 & 0.7912 & 0.8156 & 0.7958 & 0.829 & 0.8399 \\ 
	%&ResNet50& 0.835 & 0.8648 & 0.8608 & 0.8758 & 0.8928 & 0.8412 & 0.8417 & 0.8308 & 0.8375 \\ 
	%&ResNet101& 0.923 & 0.9223 & 0.9386 & 0.9321 & 0.9444 & 0.9266 & 0.9298 & 0.9353 & 0.9293 \\ 
	%&ResNet152& 0.9572 & 0.9538 & 0.9646 & 0.9568 & 0.9683 & 0.9602 & 0.9614 & 0.95 & 0.9648 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 20\)}}&ResNet18 & 0.7965 & 0.7665 & 0.756 & 0.7598 & 0.7504 & 0.7528 & 0.7515 & 0.7741 & 0.7638 \\ 
	%&ResNet34 & 0.8271 & 0.8194 & 0.8377 & 0.8436 & 0.8511 & 0.832 & 0.83 & 0.82 & 0.8239 \\ 
	%&ResNet50& 0.86 & 0.8049 & 0.8013 & 0.8654 & 0.8143 & 0.8283 & 0.8648 & 0.8004 & 0.8893 \\ 
	%&ResNet101& 0.9491 & 0.9497 & 0.9451 & 0.9335 & 0.9376 & 0.9215 & 0.9336 & 0.9465 & 0.9404 \\ 
	%&ResNet152& 0.9679 & 0.9536 & 0.9607 & 0.9674 & 0.9629 & 0.9653 & 0.9666 & 0.9511 & 0.9586 \\ 
	%\bottomrule
	%\end{tabular}
	%}
%\end{table}
%
%
%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Univariate interval-valued time series (H-S-T-B) discriminant results based on RP}
%\setlength{\tabcolsep}{2mm}{  
	%\begin{tabular}{clccccccccc}
	%\toprule
	%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 1\)}}&ResNet18 & 0.7664 & 0.7854 & 0.768 & 0.7586 & 0.7686 & 0.7823 & 0.7754 & 0.797 & 0.7883 \\ 
	%&ResNet34 & 0.8584 & 0.8572 & 0.7995 & 0.8199 & 0.8587 & 0.8084 & 0.8517 & 0.8102 & 0.8016 \\ 
	%&ResNet50& 0.8023 & 0.8505 & 0.8465 & 0.8627 & 0.8195 & 0.8387 & 0.8163 & 0.868 & 0.8906 \\ 
	%&ResNet101& 0.9271 & 0.9438 & 0.9298 & 0.9328 & 0.9473 & 0.9312 & 0.9205 & 0.9296 & 0.9214 \\ 
	%&ResNet152& 0.9658 & 0.9592 & 0.9598 & 0.9561 & 0.9699 & 0.9652 & 0.9694 & 0.9673 & 0.9699 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 5\)}}&ResNet18 & 0.7887 & 0.775 & 0.7796 & 0.7807 & 0.7872 & 0.7607 & 0.7871 & 0.783 & 0.7505 \\ 
	%&ResNet34 & 0.85 & 0.8219 & 0.8524 & 0.7971 & 0.8549 & 0.8242 & 0.8197 & 0.8562 & 0.7977 \\ 
	%&ResNet50& 0.8612 & 0.8316 & 0.8518 & 0.8833 & 0.8459 & 0.8114 & 0.8841 & 0.8291 & 0.8457 \\ 
	%&ResNet101& 0.9393 & 0.9276 & 0.9403 & 0.9305 & 0.9291 & 0.9499 & 0.9339 & 0.9234 & 0.9466 \\ 
	%&ResNet152& 0.9549 & 0.9656 & 0.9538 & 0.9631 & 0.96 & 0.9503 & 0.9664 & 0.9578 & 0.951 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 10\)}}&ResNet18 & 0.7511 & 0.783 & 0.7502 & 0.7933 & 0.7731 & 0.7661 & 0.7752 & 0.7509 & 0.7775 \\ 
	%&ResNet34 & 0.825 & 0.8348 & 0.8077 & 0.7927 & 0.8538 & 0.8078 & 0.8532 & 0.7921 & 0.834 \\ 
	%&ResNet50& 0.8647 & 0.8058 & 0.811 & 0.8858 & 0.8703 & 0.8882 & 0.866 & 0.8705 & 0.8942 \\ 
	%&ResNet101& 0.9209 & 0.9419 & 0.9427 & 0.9383 & 0.9416 & 0.9291 & 0.932 & 0.9445 & 0.9223 \\ 
	%&ResNet152& 0.9611 & 0.9574 & 0.9519 & 0.9584 & 0.9668 & 0.9544 & 0.9584 & 0.9507 & 0.9572 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 15\)}}&ResNet18 & 0.7803 & 0.7836 & 0.7725 & 0.7741 & 0.7511 & 0.7973 & 0.7513 & 0.7765 & 0.7747 \\ 
	%&ResNet34 & 0.8285 & 0.8001 & 0.7978 & 0.8372 & 0.837 & 0.8555 & 0.7974 & 0.8558 & 0.7958 \\ 
	%&ResNet50& 0.8169 & 0.8962 & 0.8986 & 0.8675 & 0.8134 & 0.8845 & 0.8831 & 0.8914 & 0.82 \\ 
	%&ResNet101& 0.9273 & 0.9229 & 0.9226 & 0.9266 & 0.9465 & 0.9451 & 0.931 & 0.9452 & 0.9442 \\ 
	%&ResNet152& 0.9518 & 0.9603 & 0.9679 & 0.9678 & 0.9515 & 0.9555 & 0.9582 & 0.9588 & 0.9616 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 20\)}}&ResNet18 & 0.7833 & 0.763 & 0.7575 & 0.7513 & 0.7879 & 0.7853 & 0.7783 & 0.7835 & 0.7974 \\ 
	%&ResNet34 & 0.8466 & 0.8116 & 0.8493 & 0.8156 & 0.8112 & 0.8061 & 0.7947 & 0.7973 & 0.7914 \\ 
	%&ResNet50& 0.8065 & 0.8043 & 0.8459 & 0.8844 & 0.8136 & 0.8951 & 0.8667 & 0.8562 & 0.8263 \\ 
	%&ResNet101& 0.942 & 0.9258 & 0.9327 & 0.9232 & 0.9421 & 0.9381 & 0.9476 & 0.9263 & 0.9366 \\ 
	%&ResNet152& 0.9525 & 0.9501 & 0.9645 & 0.9606 & 0.957 & 0.9648 & 0.9622 & 0.9558 & 0.9585 \\ 
	%\bottomrule
	%\end{tabular}
	%}
%\end{table}

\begin{table}[H]
	\footnotesize
	\setlength{\abovecaptionskip}{0pt}%
	\setlength{\belowcaptionskip}{3pt}%
	\centering
	\caption{Univariate interval-valued time series discriminant results based on RP}
	\setlength{\tabcolsep}{2mm}{
		\begin{tabular}{ccccccccccc}
			\toprule
			DGP& \(\nu\) & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
			\midrule
			\multirow{5}{*}{\tabincell{c}{H-S}} &\(\nu = 1\) & 0.6428 & 0.6604 & 0.6674 & 0.6961 & 0.6898 & 0.6966 & 0.6134 & 0.663 & 0.6681 \\ 
			&\(\nu = 5\)& 0.7124 & 0.6759 & 0.6815 & 0.7381 & 0.6846 & 0.7285 & 0.6645 & 0.6663 & 0.665 \\ 
			&\(\nu = 10\)& 0.8272 & 0.8042 & 0.8033 & 0.8002 & 0.8181 & 0.8115 & 0.8137 & 0.8181 & 0.8357 \\ 
			&\(\nu = 15\)& 0.8481 & 0.8446 & 0.8692 & 0.8591 & 0.8441 & 0.8564 & 0.8868 & 0.8733 & 0.8605 \\ 
			&\(\nu = 20\)& 0.9526 & 0.9457 & 0.9436 & 0.9254 & 0.93 & 0.9663 & 0.9017 & 0.9139 & 0.9249 \\ 
			\midrule
			\multirow{5}{*}{\tabincell{c}{S-T-B}} &\(\nu = 1\) & 0.603 & 0.631 & 0.6784 & 0.6649 & 0.6142 & 0.6489 & 0.6922 & 0.6244 & 0.6393 \\ 
			&\(\nu = 5\) & 0.6785 & 0.6575 & 0.6832 & 0.7435 & 0.7498 & 0.6958 & 0.7255 & 0.6761 & 0.7428 \\ 
			&\(\nu = 10\)& 0.811 & 0.8044 & 0.8429 & 0.8252 & 0.8212 & 0.8365 & 0.8363 & 0.8498 & 0.8267 \\ 
			&\(\nu = 15\)& 0.855 & 0.8541 & 0.8471 & 0.8465 & 0.8447 & 0.8685 & 0.8406 & 0.8897 & 0.8719 \\ 
			&\(\nu = 20\)& 0.94 & 0.9174 & 0.9524 & 0.9195 & 0.9607 & 0.9128 & 0.9069 & 0.9674 & 0.9383 \\
			\midrule
			\multirow{5}{*}{\tabincell{c}{H-S-T-B}} &\(\nu = 1\) & 0.6548 & 0.6085 & 0.6964 & 0.6335 & 0.692 & 0.6255 & 0.6309 & 0.6487 & 0.6 \\ 
			&\(\nu = 5\) & 0.6763 & 0.7051 & 0.6824 & 0.706 & 0.7101 & 0.6766 & 0.716 & 0.6534 & 0.6768 \\ 
			&\(\nu = 10\)& 0.8071 & 0.8001 & 0.8265 & 0.826 & 0.832 & 0.8285 & 0.8494 & 0.8248 & 0.8312 \\ 
			&\(\nu = 15\)& 0.8482 & 0.8868 & 0.8699 & 0.8686 & 0.8513 & 0.8722 & 0.8648 & 0.8662 & 0.8869 \\ 
			&\(\nu = 20\)& 0.9619 & 0.9353 & 0.9006 & 0.93 & 0.909 & 0.9188 & 0.9649 & 0.9105 & 0.9141 \\
			\bottomrule
		\end{tabular}
	} 
\end{table}

\subsubsection{Discriminant results based on IRP}

We choose the same kernel functions \(K(u, v)\) as in the simulation studies in Section \ref{sec5}, and the discrimination results corresponding to the three combinations are shown in the following three tables.

%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Univariate interval-valued time series (H-S) discriminant results based on IRP}
%\setlength{\tabcolsep}{2mm}{  
	%\begin{tabular}{clccccccccc}
	%\toprule
	%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_1\)}}&ResNet18 & 0.627 & 0.6081 & 0.6313 & 0.6178 & 0.6037 & 0.6175 & 0.6401 & 0.6252 & 0.6383 \\ 
	%&ResNet34 & 0.7331 & 0.7009 & 0.7336 & 0.7154 & 0.7393 & 0.7109 & 0.7334 & 0.7258 & 0.7054 \\ 
	%&ResNet50& 0.7886 & 0.7694 & 0.7922 & 0.7788 & 0.7702 & 0.8231 & 0.7894 & 0.7688 & 0.7888 \\ 
	%&ResNet101& 0.8465 & 0.8509 & 0.8594 & 0.8495 & 0.8472 & 0.8499 & 0.842 & 0.854 & 0.8495 \\ 
	%&ResNet152& 0.9115 & 0.9182 & 0.9181 & 0.9168 & 0.9121 & 0.9026 & 0.9044 & 0.9063 & 0.9 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_2\)}}&ResNet18 & 0.6256 & 0.6213 & 0.6244 & 0.6291 & 0.6296 & 0.6013 & 0.6489 & 0.6497 & 0.6333 \\ 
	%&ResNet34 & 0.7099 & 0.7127 & 0.7296 & 0.7024 & 0.7382 & 0.7229 & 0.7208 & 0.7273 & 0.7255 \\ 
	%&ResNet50& 0.7814 & 0.8171 & 0.7903 & 0.7791 & 0.8008 & 0.7504 & 0.7593 & 0.7823 & 0.823 \\ 
	%&ResNet101& 0.8571 & 0.8582 & 0.8505 & 0.8508 & 0.8571 & 0.844 & 0.8519 & 0.8427 & 0.8439 \\ 
	%&ResNet152& 0.913 & 0.9139 & 0.918 & 0.913 & 0.9083 & 0.9139 & 0.9096 & 0.9057 & 0.9006 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_3\)}}&ResNet18 & 0.6327 & 0.6192 & 0.6461 & 0.645 & 0.6474 & 0.649 & 0.6137 & 0.6483 & 0.6038 \\ 
	%&ResNet34 & 0.7256 & 0.7303 & 0.7283 & 0.7207 & 0.7398 & 0.74 & 0.7294 & 0.7366 & 0.7206 \\ 
	%&ResNet50& 0.7622 & 0.8192 & 0.7926 & 0.7523 & 0.7933 & 0.7725 & 0.78 & 0.8296 & 0.7809 \\ 
	%&ResNet101& 0.8548 & 0.8563 & 0.8462 & 0.849 & 0.85 & 0.8561 & 0.8496 & 0.8439 & 0.8576 \\ 
	%&ResNet152& 0.9099 & 0.9173 & 0.9168 & 0.9055 & 0.906 & 0.9169 & 0.9136 & 0.9159 & 0.9181 \\ 
	%\bottomrule
	%\end{tabular}
	%}
%\end{table}
%
%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Univariate interval-valued time series (S-T-B) discriminant results based on IRP}
%\setlength{\tabcolsep}{2mm}{  
	%\begin{tabular}{clccccccccc}
	%\toprule
	%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_1\)}}&ResNet18 & 0.6172 & 0.6304 & 0.6186 & 0.6469 & 0.6143 & 0.626 & 0.6345 & 0.6419 & 0.6164 \\ 
	%&ResNet34 & 0.7233 & 0.7243 & 0.7057 & 0.7269 & 0.7215 & 0.7277 & 0.7077 & 0.7323 & 0.7157 \\ 
	%&ResNet50& 0.8082 & 0.7823 & 0.823 & 0.8235 & 0.756 & 0.7757 & 0.7556 & 0.7796 & 0.7907 \\ 
	%&ResNet101& 0.8472 & 0.8515 & 0.859 & 0.8436 & 0.8432 & 0.8558 & 0.8433 & 0.84 & 0.8476 \\ 
	%&ResNet152& 0.9008 & 0.9071 & 0.913 & 0.9165 & 0.9149 & 0.9002 & 0.9175 & 0.9138 & 0.9184 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_2\)}}&ResNet18 & 0.6468 & 0.6117 & 0.6307 & 0.6035 & 0.6467 & 0.612 & 0.6094 & 0.6061 & 0.6486 \\ 
	%&ResNet34 & 0.7133 & 0.7031 & 0.7268 & 0.7274 & 0.7391 & 0.7072 & 0.7122 & 0.7172 & 0.7246 \\ 
	%&ResNet50& 0.7816 & 0.8169 & 0.7599 & 0.7881 & 0.754 & 0.7525 & 0.7709 & 0.8237 & 0.8289 \\ 
	%&ResNet101& 0.8464 & 0.8564 & 0.8545 & 0.8518 & 0.8443 & 0.8463 & 0.8515 & 0.854 & 0.8576 \\ 
	%&ResNet152& 0.9023 & 0.9148 & 0.9189 & 0.9181 & 0.9071 & 0.9025 & 0.903 & 0.9103 & 0.9027 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_3\)}}&ResNet18 & 0.6353 & 0.6157 & 0.6097 & 0.6222 & 0.6012 & 0.6272 & 0.637 & 0.6223 & 0.6271 \\ 
	%&ResNet34 & 0.7087 & 0.7086 & 0.7279 & 0.7129 & 0.7092 & 0.7226 & 0.7165 & 0.731 & 0.7222 \\ 
	%&ResNet50& 0.8296 & 0.7931 & 0.7688 & 0.7755 & 0.8167 & 0.7514 & 0.7801 & 0.7927 & 0.7659 \\ 
	%&ResNet101& 0.86 & 0.8592 & 0.8495 & 0.846 & 0.8455 & 0.8544 & 0.851 & 0.8593 & 0.8581 \\ 
	%&ResNet152& 0.9175 & 0.9082 & 0.9049 & 0.9056 & 0.9093 & 0.9112 & 0.9124 & 0.9006 & 0.9019 \\ 
	%\bottomrule
	%\end{tabular}
	%}
%\end{table}
%
%
%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Univariate interval-valued time series (H-S-T-B) discriminant results based on IRP}
%\setlength{\tabcolsep}{2mm}{  
	%\begin{tabular}{clccccccccc}
	%\toprule
	%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_1\)}}&ResNet18 & 0.6317 & 0.6062 & 0.6379 & 0.6082 & 0.6465 & 0.642 & 0.6445 & 0.609 & 0.61 \\ 
	%&ResNet34 & 0.7374 & 0.7334 & 0.7369 & 0.7059 & 0.7024 & 0.7079 & 0.7277 & 0.7378 & 0.7193 \\ 
	%&ResNet50& 0.8115 & 0.7584 & 0.7535 & 0.7682 & 0.7902 & 0.7636 & 0.8277 & 0.8286 & 0.7757 \\ 
	%&ResNet101& 0.8577 & 0.8559 & 0.8472 & 0.8588 & 0.859 & 0.8517 & 0.8405 & 0.8531 & 0.8451 \\ 
	%&ResNet152& 0.9093 & 0.905 & 0.9124 & 0.9042 & 0.9066 & 0.901 & 0.9125 & 0.9062 & 0.919 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_2\)}}&ResNet18 & 0.6032 & 0.6299 & 0.6111 & 0.6025 & 0.6349 & 0.6465 & 0.627 & 0.6472 & 0.614 \\ 
	%&ResNet34 & 0.7068 & 0.7208 & 0.7029 & 0.7373 & 0.7194 & 0.7118 & 0.7281 & 0.703 & 0.7384 \\ 
	%&ResNet50& 0.8211 & 0.8275 & 0.7926 & 0.8262 & 0.7983 & 0.8084 & 0.7864 & 0.794 & 0.8288 \\ 
	%&ResNet101& 0.8485 & 0.8537 & 0.8438 & 0.8551 & 0.8471 & 0.8502 & 0.8441 & 0.8548 & 0.8599 \\ 
	%&ResNet152& 0.9131 & 0.9067 & 0.9185 & 0.9052 & 0.9099 & 0.9058 & 0.9133 & 0.9163 & 0.9103 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_3\)}}&ResNet18 & 0.6391 & 0.6157 & 0.6025 & 0.6337 & 0.6402 & 0.617 & 0.6389 & 0.6216 & 0.6123 \\ 
	%&ResNet34 & 0.7381 & 0.7304 & 0.7292 & 0.7064 & 0.7389 & 0.723 & 0.734 & 0.7384 & 0.7316 \\ 
	%&ResNet50& 0.8221 & 0.7857 & 0.7991 & 0.8247 & 0.7525 & 0.7511 & 0.7527 & 0.8034 & 0.7897 \\ 
	%&ResNet101& 0.8413 & 0.8579 & 0.8537 & 0.8596 & 0.8475 & 0.859 & 0.8415 & 0.8538 & 0.8594 \\ 
	%&ResNet152& 0.9034 & 0.9178 & 0.9168 & 0.9007 & 0.9022 & 0.9135 & 0.9019 & 0.9006 & 0.9047 \\ 
	%\bottomrule
	%\end{tabular}
	%}
%\end{table}

\begin{table}[H]
	\footnotesize
	\setlength{\abovecaptionskip}{0pt}%
	\setlength{\belowcaptionskip}{3pt}%
	\centering
	\caption{Univariate interval-valued time series discriminant results based on IRP}
	\setlength{\tabcolsep}{2mm}{
		\begin{tabular}{ccccccccccc}
			\toprule
			DGP& kernel & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
			\midrule
			\multirow{3}{*}{\tabincell{c}{H-S}} &\(K_1\) & 0.6428 & 0.6604 & 0.6674 & 0.6961 & 0.6898 & 0.6966 & 0.6134 & 0.663 & 0.6681 \\ 
			&\(K_2\)& 0.7124 & 0.6759 & 0.6815 & 0.7381 & 0.6846 & 0.7285 & 0.6645 & 0.6663 & 0.665 \\ 
			&\(K_3\)& 0.8272 & 0.8042 & 0.8033 & 0.8002 & 0.8181 & 0.8115 & 0.8137 & 0.8181 & 0.8357 \\ 
			\midrule
			\multirow{3}{*}{\tabincell{c}{S-T-B}} &\(K_1\) & 0.603 & 0.631 & 0.6784 & 0.6649 & 0.6142 & 0.6489 & 0.6922 & 0.6244 & 0.6393 \\ 
			&\(K_2\) & 0.6785 & 0.6575 & 0.6832 & 0.7435 & 0.7498 & 0.6958 & 0.7255 & 0.6761 & 0.7428 \\ 
			&\(K_3\)& 0.811 & 0.8044 & 0.8429 & 0.8252 & 0.8212 & 0.8365 & 0.8363 & 0.8498 & 0.8267 \\
			\midrule
			\multirow{3}{*}{\tabincell{c}{H-S-T-B}} &\(K_1\) & 0.6548 & 0.6085 & 0.6964 & 0.6335 & 0.692 & 0.6255 & 0.6309 & 0.6487 & 0.6 \\ 
			&\(K_2\) & 0.6763 & 0.7051 & 0.6824 & 0.706 & 0.7101 & 0.6766 & 0.716 & 0.6534 & 0.6768 \\ 
			&\(K_3\)& 0.8071 & 0.8001 & 0.8265 & 0.826 & 0.832 & 0.8285 & 0.8494 & 0.8248 & 0.8312 \\
			\bottomrule
		\end{tabular}
	}
\end{table}


\subsection{Interval vector-valued time series discriminant}
In this subsection, all of the modeling settings are the same as in Subsection \ref{sec61}, with the exception that the all six variables described at the beginning of Section \ref{sec6} will be selected for discriminations. The detailed discrimination results are shown below. 


% 除了上述三种场景, 还可以考虑更加细粒度的判别问题. 选取上海的虹桥和上海浦东机场两个观测点的点的数据用于分类
\subsubsection{Discriminant results based on JRP}

%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Interval vector-valued time series (H-S) discriminant results based on JRP}
%\setlength{\tabcolsep}{2mm}{  
	%\begin{tabular}{clccccccccc}
	%\toprule
	%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 1\)}}&ResNet18 & 0.7872 & 0.7963 & 0.7661 & 0.7667 & 0.7868 & 0.7583 & 0.7862 & 0.7706 & 0.7711 \\ 
	%&ResNet34 & 0.8161 & 0.8005 & 0.8423 & 0.8432 & 0.8067 & 0.8498 & 0.8214 & 0.8338 & 0.8231 \\ 
	%&ResNet50& 0.8714 & 0.8429 & 0.8874 & 0.8949 & 0.8337 & 0.8273 & 0.846 & 0.8426 & 0.8151 \\ 
	%&ResNet101& 0.9371 & 0.9409 & 0.9452 & 0.9239 & 0.9454 & 0.9294 & 0.9378 & 0.9286 & 0.9253 \\ 
	%&ResNet152& 0.9631 & 0.9523 & 0.9623 & 0.9544 & 0.9536 & 0.9504 & 0.9612 & 0.9697 & 0.9637 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 5\)}}&ResNet18 & 0.797 & 0.776 & 0.7931 & 0.7826 & 0.7632 & 0.7901 & 0.7892 & 0.7688 & 0.7524 \\ 
	%&ResNet34 & 0.8453 & 0.7903 & 0.8337 & 0.8113 & 0.8569 & 0.7988 & 0.8269 & 0.8297 & 0.8043 \\ 
	%&ResNet50& 0.8497 & 0.866 & 0.8831 & 0.8993 & 0.8791 & 0.8737 & 0.8002 & 0.8957 & 0.8825 \\ 
	%&ResNet101& 0.9381 & 0.9249 & 0.9357 & 0.9246 & 0.9267 & 0.9231 & 0.9416 & 0.9428 & 0.9493 \\ 
	%&ResNet152& 0.9502 & 0.9695 & 0.9673 & 0.9633 & 0.9676 & 0.9559 & 0.9694 & 0.9535 & 0.9649 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 10\)}}&ResNet18 & 0.7835 & 0.7954 & 0.7854 & 0.7681 & 0.7617 & 0.7812 & 0.7673 & 0.7759 & 0.7593 \\ 
	%&ResNet34 & 0.8437 & 0.8167 & 0.8287 & 0.7945 & 0.8273 & 0.8453 & 0.8348 & 0.8588 & 0.8289 \\ 
	%&ResNet50& 0.8771 & 0.8062 & 0.8548 & 0.8255 & 0.8434 & 0.872 & 0.8065 & 0.83 & 0.8016 \\ 
	%&ResNet101& 0.9205 & 0.9462 & 0.9416 & 0.9308 & 0.9323 & 0.9264 & 0.9313 & 0.948 & 0.9215 \\ 
	%&ResNet152& 0.9624 & 0.965 & 0.953 & 0.9677 & 0.9613 & 0.9546 & 0.9555 & 0.9544 & 0.965 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 15\)}}&ResNet18 & 0.7956 & 0.7643 & 0.7824 & 0.7973 & 0.7697 & 0.7917 & 0.7613 & 0.7627 & 0.7732 \\ 
	%&ResNet34 & 0.8284 & 0.8544 & 0.8242 & 0.8418 & 0.8568 & 0.8064 & 0.8282 & 0.8057 & 0.8176 \\ 
	%&ResNet50& 0.8336 & 0.8191 & 0.8801 & 0.8241 & 0.8894 & 0.8746 & 0.8781 & 0.8005 & 0.8675 \\ 
	%&ResNet101& 0.9465 & 0.9466 & 0.9492 & 0.9435 & 0.9352 & 0.9311 & 0.9344 & 0.9321 & 0.937 \\ 
	%&ResNet152& 0.9647 & 0.9535 & 0.9688 & 0.9648 & 0.9572 & 0.9516 & 0.9577 & 0.9606 & 0.9538 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 20\)}}&ResNet18 & 0.7542 & 0.7733 & 0.7982 & 0.7945 & 0.7556 & 0.7565 & 0.7518 & 0.7962 & 0.7964 \\ 
	%&ResNet34 & 0.7972 & 0.8177 & 0.8423 & 0.7978 & 0.8286 & 0.8088 & 0.8212 & 0.8098 & 0.8125 \\ 
	%&ResNet50& 0.8836 & 0.8002 & 0.868 & 0.8951 & 0.8607 & 0.8952 & 0.8818 & 0.8821 & 0.8214 \\ 
	%&ResNet101& 0.9389 & 0.9228 & 0.9274 & 0.9488 & 0.9386 & 0.9414 & 0.9437 & 0.9399 & 0.924 \\ 
	%&ResNet152& 0.9616 & 0.9518 & 0.9569 & 0.9631 & 0.9504 & 0.9686 & 0.9663 & 0.9651 & 0.9604 \\ 
	%\bottomrule
	%\end{tabular}
	%}
%\end{table}
%
%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Interval vector-valued time series (S-T-B) discriminant results based on JRP}
%\setlength{\tabcolsep}{2mm}{  
	%\begin{tabular}{clccccccccc}
	%\toprule
	%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 1\)}}&ResNet18 & 0.7506 & 0.7795 & 0.7734 & 0.7666 & 0.7814 & 0.7794 & 0.7994 & 0.7949 & 0.7509 \\ 
	%&ResNet34 & 0.8384 & 0.8365 & 0.8185 & 0.8134 & 0.8594 & 0.8563 & 0.8311 & 0.824 & 0.8387 \\ 
	%&ResNet50& 0.8288 & 0.8614 & 0.8133 & 0.8735 & 0.8917 & 0.8044 & 0.8207 & 0.8021 & 0.839 \\ 
	%&ResNet101& 0.9378 & 0.9269 & 0.9224 & 0.9215 & 0.9487 & 0.9322 & 0.947 & 0.9491 & 0.9453 \\ 
	%&ResNet152& 0.9667 & 0.9697 & 0.9508 & 0.9605 & 0.9686 & 0.9649 & 0.9696 & 0.9548 & 0.9594 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 5\)}}&ResNet18 & 0.7635 & 0.7996 & 0.761 & 0.7945 & 0.7833 & 0.7561 & 0.7513 & 0.7518 & 0.7556 \\ 
	%&ResNet34 & 0.8163 & 0.8453 & 0.7926 & 0.8112 & 0.7982 & 0.8545 & 0.8184 & 0.8366 & 0.8458 \\ 
	%&ResNet50& 0.8942 & 0.8458 & 0.8374 & 0.8914 & 0.8301 & 0.8932 & 0.813 & 0.8383 & 0.8335 \\ 
	%&ResNet101& 0.9236 & 0.9357 & 0.9374 & 0.9288 & 0.9436 & 0.945 & 0.9247 & 0.928 & 0.9448 \\ 
	%&ResNet152& 0.9648 & 0.9685 & 0.9667 & 0.9514 & 0.9664 & 0.958 & 0.9594 & 0.9628 & 0.958 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 10\)}}&ResNet18 & 0.7522 & 0.7516 & 0.7748 & 0.7517 & 0.7859 & 0.799 & 0.7704 & 0.7957 & 0.7896 \\ 
	%&ResNet34 & 0.7995 & 0.7962 & 0.8316 & 0.8042 & 0.7904 & 0.8398 & 0.8327 & 0.8115 & 0.8044 \\ 
	%&ResNet50& 0.8611 & 0.8763 & 0.8349 & 0.8173 & 0.8695 & 0.8595 & 0.8846 & 0.8134 & 0.8986 \\ 
	%&ResNet101& 0.9491 & 0.9269 & 0.9357 & 0.9401 & 0.95 & 0.9482 & 0.9313 & 0.9256 & 0.9353 \\ 
	%&ResNet152& 0.9635 & 0.9554 & 0.9591 & 0.9563 & 0.9612 & 0.9642 & 0.9571 & 0.969 & 0.9664 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 15\)}}&ResNet18 & 0.7563 & 0.7624 & 0.7554 & 0.7712 & 0.7648 & 0.7862 & 0.7811 & 0.7687 & 0.7803 \\ 
	%&ResNet34 & 0.8239 & 0.8184 & 0.7972 & 0.8501 & 0.851 & 0.7959 & 0.8526 & 0.8493 & 0.8083 \\ 
	%&ResNet50& 0.8594 & 0.8176 & 0.8497 & 0.8049 & 0.8807 & 0.8733 & 0.8343 & 0.8385 & 0.8085 \\ 
	%&ResNet101& 0.9246 & 0.9201 & 0.9339 & 0.9268 & 0.9278 & 0.9486 & 0.9287 & 0.9275 & 0.9206 \\ 
	%&ResNet152& 0.9571 & 0.9617 & 0.9609 & 0.9678 & 0.9605 & 0.959 & 0.953 & 0.9571 & 0.9591 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 20\)}}&ResNet18 & 0.7909 & 0.7794 & 0.7834 & 0.7888 & 0.7589 & 0.7796 & 0.7942 & 0.7888 & 0.784 \\ 
	%&ResNet34 & 0.8493 & 0.8046 & 0.7967 & 0.849 & 0.8014 & 0.8161 & 0.8401 & 0.8094 & 0.8586 \\ 
	%&ResNet50& 0.8027 & 0.8879 & 0.8803 & 0.869 & 0.8191 & 0.8138 & 0.8871 & 0.8267 & 0.8662 \\ 
	%&ResNet101& 0.9273 & 0.9336 & 0.9238 & 0.9238 & 0.927 & 0.946 & 0.9328 & 0.9426 & 0.9472 \\ 
	%&ResNet152& 0.9581 & 0.9642 & 0.9592 & 0.9508 & 0.9581 & 0.959 & 0.9681 & 0.9648 & 0.956 \\ 
	%\bottomrule
	%\end{tabular}
	%}
%\end{table}
%
%
%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Interval vector-valued time series (H-S-T-B) discriminant results based on JRP}
%\setlength{\tabcolsep}{2mm}{  
	%\begin{tabular}{clccccccccc}
	%\toprule
	%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 1\)}}&ResNet18 & 0.7607 & 0.7612 & 0.7583 & 0.7584 & 0.78 & 0.7505 & 0.7585 & 0.7607 & 0.7681 \\ 
	%&ResNet34 & 0.8514 & 0.8412 & 0.8031 & 0.8136 & 0.8478 & 0.8298 & 0.8197 & 0.8339 & 0.8492 \\ 
	%&ResNet50& 0.8839 & 0.8935 & 0.8388 & 0.8915 & 0.8098 & 0.8395 & 0.8105 & 0.8075 & 0.8244 \\ 
	%&ResNet101& 0.9207 & 0.9359 & 0.9337 & 0.9349 & 0.937 & 0.9346 & 0.9334 & 0.9393 & 0.9419 \\ 
	%&ResNet152& 0.9534 & 0.9512 & 0.9678 & 0.9527 & 0.97 & 0.9693 & 0.9558 & 0.9656 & 0.9584 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 5\)}}&ResNet18 & 0.7958 & 0.7532 & 0.7975 & 0.7839 & 0.7718 & 0.7905 & 0.7751 & 0.7796 & 0.7569 \\ 
	%&ResNet34 & 0.8302 & 0.8067 & 0.7902 & 0.7926 & 0.8354 & 0.8272 & 0.8057 & 0.8385 & 0.8143 \\ 
	%&ResNet50& 0.8205 & 0.8102 & 0.855 & 0.8234 & 0.8775 & 0.813 & 0.8643 & 0.8902 & 0.899 \\ 
	%&ResNet101& 0.9211 & 0.9229 & 0.9279 & 0.9253 & 0.9256 & 0.95 & 0.9213 & 0.925 & 0.929 \\ 
	%&ResNet152& 0.9641 & 0.9566 & 0.9551 & 0.9603 & 0.9534 & 0.9567 & 0.9629 & 0.9643 & 0.9501 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 10\)}}&ResNet18 & 0.7836 & 0.7764 & 0.7811 & 0.7895 & 0.7549 & 0.7551 & 0.7723 & 0.7635 & 0.7967 \\ 
	%&ResNet34 & 0.8546 & 0.8422 & 0.7916 & 0.7987 & 0.8461 & 0.7963 & 0.8285 & 0.834 & 0.8267 \\ 
	%&ResNet50& 0.8811 & 0.8619 & 0.8789 & 0.8114 & 0.8822 & 0.8537 & 0.8986 & 0.816 & 0.8718 \\ 
	%&ResNet101& 0.9344 & 0.9304 & 0.9219 & 0.9243 & 0.933 & 0.9395 & 0.9315 & 0.9233 & 0.9223 \\ 
	%&ResNet152& 0.9674 & 0.9506 & 0.9516 & 0.9521 & 0.9689 & 0.9649 & 0.9699 & 0.959 & 0.9636 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 15\)}}&ResNet18 & 0.7925 & 0.766 & 0.7978 & 0.7915 & 0.7953 & 0.7933 & 0.7657 & 0.7992 & 0.7557 \\ 
	%&ResNet34 & 0.8245 & 0.8425 & 0.7931 & 0.8421 & 0.7931 & 0.8406 & 0.8218 & 0.8414 & 0.8235 \\ 
	%&ResNet50& 0.8163 & 0.8618 & 0.8214 & 0.8838 & 0.8792 & 0.8984 & 0.8041 & 0.8129 & 0.8395 \\ 
	%&ResNet101& 0.9394 & 0.9357 & 0.94 & 0.9422 & 0.9403 & 0.9299 & 0.9444 & 0.9394 & 0.9491 \\ 
	%&ResNet152& 0.9519 & 0.9524 & 0.9585 & 0.9691 & 0.9676 & 0.9621 & 0.9671 & 0.9627 & 0.9649 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(\nu = 20\)}}&ResNet18 & 0.7556 & 0.7824 & 0.781 & 0.7876 & 0.7742 & 0.7599 & 0.7908 & 0.7775 & 0.7735 \\ 
	%&ResNet34 & 0.8222 & 0.817 & 0.8548 & 0.8006 & 0.8538 & 0.8412 & 0.8461 & 0.8592 & 0.8068 \\ 
	%&ResNet50& 0.849 & 0.8891 & 0.8204 & 0.8963 & 0.8548 & 0.8916 & 0.8561 & 0.8645 & 0.8165 \\ 
	%&ResNet101& 0.9328 & 0.9363 & 0.9405 & 0.9311 & 0.9431 & 0.9406 & 0.9317 & 0.9356 & 0.9352 \\ 
	%&ResNet152& 0.955 & 0.9642 & 0.9663 & 0.954 & 0.9532 & 0.9605 & 0.9671 & 0.9531 & 0.9645 \\ 
	%\bottomrule
	%\end{tabular}
	%}
%\end{table}

\subsubsection{Discriminant results based on IJRP}


%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Interval vector-valued time series (H-S) discriminant results based on IJRP}
%\setlength{\tabcolsep}{2mm}{  
	%\begin{tabular}{clccccccccc}
	%\toprule
	%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_1\)}}&ResNet18 & 0.6465 & 0.6255 & 0.6259 & 0.6435 & 0.6144 & 0.6171 & 0.613 & 0.6005 & 0.6229 \\ 
	%&ResNet34 & 0.7195 & 0.7204 & 0.7184 & 0.7034 & 0.7373 & 0.7216 & 0.7338 & 0.7281 & 0.7384 \\ 
	%&ResNet50& 0.7739 & 0.7621 & 0.7885 & 0.8064 & 0.8011 & 0.7533 & 0.7628 & 0.7531 & 0.7932 \\ 
	%&ResNet101& 0.8484 & 0.8439 & 0.8574 & 0.855 & 0.8585 & 0.8422 & 0.8582 & 0.8423 & 0.8511 \\ 
	%&ResNet152& 0.905 & 0.9008 & 0.9072 & 0.9027 & 0.9073 & 0.9187 & 0.9166 & 0.9094 & 0.9079 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_2\)}}&ResNet18 & 0.6358 & 0.6373 & 0.6238 & 0.6146 & 0.6177 & 0.625 & 0.6499 & 0.6052 & 0.6496 \\ 
	%&ResNet34 & 0.7075 & 0.7082 & 0.7216 & 0.7318 & 0.705 & 0.7069 & 0.7011 & 0.7043 & 0.7162 \\ 
	%&ResNet50& 0.7666 & 0.7571 & 0.768 & 0.7675 & 0.7817 & 0.7904 & 0.7651 & 0.7517 & 0.7991 \\ 
	%&ResNet101& 0.8444 & 0.844 & 0.8418 & 0.8513 & 0.8475 & 0.8407 & 0.8532 & 0.8413 & 0.8488 \\ 
	%&ResNet152& 0.9108 & 0.9127 & 0.9181 & 0.9022 & 0.9101 & 0.9137 & 0.9042 & 0.9191 & 0.9156 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_3\)}}&ResNet18 & 0.6073 & 0.6029 & 0.6318 & 0.6208 & 0.6389 & 0.6313 & 0.646 & 0.6379 & 0.6386 \\ 
	%&ResNet34 & 0.7264 & 0.7072 & 0.7084 & 0.7252 & 0.7295 & 0.7008 & 0.7185 & 0.7208 & 0.725 \\ 
	%&ResNet50& 0.7785 & 0.7929 & 0.8245 & 0.7739 & 0.8283 & 0.815 & 0.7757 & 0.8187 & 0.7823 \\ 
	%&ResNet101& 0.8486 & 0.8556 & 0.8479 & 0.8583 & 0.8559 & 0.8482 & 0.8554 & 0.8557 & 0.8523 \\ 
	%&ResNet152& 0.9007 & 0.9189 & 0.9157 & 0.9014 & 0.9117 & 0.9129 & 0.9136 & 0.9046 & 0.9054 \\ 
	%\bottomrule
	%\end{tabular}
	%}
%\end{table}
%
%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Interval vector-valued time series (S-T-B) discriminant results based on IJRP}
%\setlength{\tabcolsep}{2mm}{  
	%\begin{tabular}{clccccccccc}
	%\toprule
	%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_1\)}}&ResNet18 & 0.6264 & 0.6372 & 0.6248 & 0.6295 & 0.6032 & 0.6487 & 0.6121 & 0.6036 & 0.6038 \\ 
	%&ResNet34 & 0.7241 & 0.7191 & 0.7217 & 0.7069 & 0.7027 & 0.711 & 0.7222 & 0.7269 & 0.7184 \\ 
	%&ResNet50& 0.822 & 0.8094 & 0.828 & 0.7863 & 0.803 & 0.8168 & 0.766 & 0.7983 & 0.8043 \\ 
	%&ResNet101& 0.8546 & 0.8534 & 0.8457 & 0.8591 & 0.8506 & 0.8447 & 0.8407 & 0.8495 & 0.8598 \\ 
	%&ResNet152& 0.9141 & 0.9121 & 0.9046 & 0.9189 & 0.9126 & 0.9128 & 0.9121 & 0.9041 & 0.9156 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_2\)}}&ResNet18 & 0.6279 & 0.6319 & 0.6406 & 0.6349 & 0.6407 & 0.6214 & 0.6118 & 0.6122 & 0.6268 \\ 
	%&ResNet34 & 0.7053 & 0.7168 & 0.7174 & 0.7229 & 0.724 & 0.7082 & 0.7333 & 0.713 & 0.7097 \\ 
	%&ResNet50& 0.7513 & 0.8053 & 0.8237 & 0.8111 & 0.8248 & 0.7651 & 0.8205 & 0.8152 & 0.7748 \\ 
	%&ResNet101& 0.8487 & 0.8529 & 0.8579 & 0.8584 & 0.855 & 0.8494 & 0.8585 & 0.8547 & 0.8561 \\ 
	%&ResNet152& 0.9162 & 0.9148 & 0.9189 & 0.9156 & 0.918 & 0.9093 & 0.9088 & 0.9004 & 0.9092 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_3\)}}&ResNet18 & 0.6371 & 0.6068 & 0.6116 & 0.6123 & 0.6256 & 0.6088 & 0.6237 & 0.6042 & 0.6409 \\ 
	%&ResNet34 & 0.7312 & 0.703 & 0.7181 & 0.7198 & 0.7331 & 0.7167 & 0.7013 & 0.721 & 0.715 \\ 
	%&ResNet50& 0.77 & 0.7947 & 0.8188 & 0.7713 & 0.7711 & 0.7943 & 0.7926 & 0.8077 & 0.7665 \\ 
	%&ResNet101& 0.8499 & 0.8478 & 0.8429 & 0.8531 & 0.8445 & 0.8569 & 0.8432 & 0.8436 & 0.8586 \\ 
	%&ResNet152& 0.9001 & 0.918 & 0.9078 & 0.9169 & 0.9102 & 0.9068 & 0.9197 & 0.9183 & 0.9195 \\ 
	%
	%\bottomrule
	%\end{tabular}
	%}
%\end{table}
%
%
%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Interval vector-valued time series (H-S-T-B) discriminant results based on IJRP}
%\setlength{\tabcolsep}{2mm}{  
	%\begin{tabular}{clccccccccc}
	%\toprule
	%\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_1\)}}&ResNet18 & 0.6491 & 0.6326 & 0.6135 & 0.617 & 0.6252 & 0.6254 & 0.6335 & 0.6089 & 0.619 \\ 
	%&ResNet34 & 0.7259 & 0.7276 & 0.7263 & 0.7021 & 0.725 & 0.7074 & 0.7321 & 0.7133 & 0.7167 \\ 
	%&ResNet50& 0.7787 & 0.7895 & 0.7713 & 0.7711 & 0.7632 & 0.7622 & 0.7861 & 0.7745 & 0.7503 \\ 
	%&ResNet101& 0.846 & 0.8538 & 0.8482 & 0.8576 & 0.8441 & 0.8553 & 0.8529 & 0.851 & 0.856 \\ 
	%&ResNet152& 0.9109 & 0.9053 & 0.9195 & 0.9099 & 0.9073 & 0.9172 & 0.9136 & 0.9075 & 0.9159 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_2\)}}&ResNet18 & 0.6132 & 0.6073 & 0.6309 & 0.6256 & 0.6486 & 0.6245 & 0.6305 & 0.6016 & 0.6455 \\ 
	%&ResNet34 & 0.7368 & 0.7061 & 0.7066 & 0.7228 & 0.7092 & 0.7183 & 0.724 & 0.7104 & 0.701 \\ 
	%&ResNet50& 0.807 & 0.7841 & 0.8058 & 0.7995 & 0.8017 & 0.7627 & 0.7701 & 0.8287 & 0.8017 \\ 
	%&ResNet101& 0.8541 & 0.8452 & 0.8592 & 0.842 & 0.8569 & 0.8447 & 0.8598 & 0.8479 & 0.8597 \\ 
	%&ResNet152& 0.9007 & 0.9123 & 0.9192 & 0.9045 & 0.9111 & 0.9178 & 0.9 & 0.9196 & 0.9092 \\ 
	%
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{\(K_3\)}}&ResNet18 & 0.6264 & 0.633 & 0.6438 & 0.6233 & 0.6439 & 0.6155 & 0.6131 & 0.6462 & 0.6498 \\ 
	%&ResNet34 & 0.721 & 0.7132 & 0.7033 & 0.713 & 0.7203 & 0.7312 & 0.7247 & 0.7175 & 0.7014 \\ 
	%&ResNet50& 0.7532 & 0.7647 & 0.7853 & 0.7575 & 0.805 & 0.772 & 0.8029 & 0.7998 & 0.7619 \\ 
	%&ResNet101& 0.8585 & 0.8552 & 0.8467 & 0.8458 & 0.8516 & 0.8509 & 0.8469 & 0.8547 & 0.8409 \\ 
	%&ResNet152& 0.9001 & 0.9166 & 0.9006 & 0.9148 & 0.9094 & 0.9101 & 0.9073 & 0.9134 & 0.9118 \\ 
	%\bottomrule
	%\end{tabular}
	%}
%\end{table}

\subsection{Fine-grained discrimination}
Beyond the discrimination tasks discussed above, we also consider the fine-grained discrimination of interval-valued time series in order to better assess the effectiveness of the proposed method. By fine-grained discrimination, one refers to the high similarity or correlation of the data to be discriminated.
We obtained six weather indicators from the website \url{https://rp5.ru/} from 2005-01-02 to 2023-04-11 for the Shanghai Baoan station and from 2019-07-07 to 2023-04-11  for the Shanghai Hongqiao station, and compressed in units of days into interval vector value time series. Similar to the preceding, 30 days of observations serve as a trajectory for discrimination. The data from each of the two districts are treated as a class to construct the interval vector-valued time series discriminant data. 

Since both Baoan and Hongqiao districts are located in Shanghai, the geographic location is rather close and the climate is relatively similar, causing a high correlation of the six weather indicators, which raises the difficulty of discriminating. Furthermore, the data available from the website for Hongqiao district is quite less than that for Baoan district, and such class imbalance further exacerbates the difficulty of discriminating. The following two tables show the fine-grained discriminant results based on JRP and IJRP, respectively.


\begin{table}[H]
	\footnotesize
	\setlength{\abovecaptionskip}{0pt}%
	\setlength{\belowcaptionskip}{3pt}%
	\centering
	\caption{The discriminant results of Hongqiao-Baoan and based on JRP}
	\setlength{\tabcolsep}{2mm}{  
		\begin{tabular}{clccccccccc}
			\toprule
			\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
			\midrule
			\multirow{5}{*}{\tabincell{c}{\(\nu = 1\)}}&ResNet18 & 0.7927 & 0.7545 & 0.7579 & 0.7503 & 0.7665 & 0.7668 & 0.7604 & 0.776 & 0.7653 \\ 
			&ResNet34 & 0.7976 & 0.8471 & 0.8035 & 0.8476 & 0.7907 & 0.797 & 0.7933 & 0.8106 & 0.8443 \\ 
			&ResNet50& 0.8133 & 0.8619 & 0.8627 & 0.8249 & 0.8493 & 0.8322 & 0.8608 & 0.8272 & 0.8914 \\ 
			&ResNet101& 0.9373 & 0.9229 & 0.9383 & 0.9317 & 0.9216 & 0.9399 & 0.9271 & 0.9303 & 0.9356 \\ 
			&ResNet152& 0.9526 & 0.9677 & 0.9607 & 0.9588 & 0.9562 & 0.9502 & 0.96 & 0.9606 & 0.965 \\ 
			
			\midrule
			\multirow{5}{*}{\tabincell{c}{\(\nu = 1\)}}&ResNet18 & 0.7968 & 0.7511 & 0.7587 & 0.7979 & 0.7635 & 0.7755 & 0.7501 & 0.7822 & 0.7637 \\ 
			&ResNet34 & 0.8286 & 0.8429 & 0.8402 & 0.8007 & 0.7996 & 0.8233 & 0.8138 & 0.8568 & 0.8462 \\ 
			&ResNet50& 0.8102 & 0.8369 & 0.8357 & 0.8739 & 0.8218 & 0.8114 & 0.8388 & 0.8083 & 0.8327 \\ 
			&ResNet101& 0.9347 & 0.9493 & 0.9237 & 0.9409 & 0.9301 & 0.945 & 0.9487 & 0.9312 & 0.9428 \\ 
			&ResNet152& 0.9508 & 0.9605 & 0.9604 & 0.9687 & 0.9531 & 0.9698 & 0.9516 & 0.9667 & 0.9528 \\ 
			
			\midrule
			\multirow{5}{*}{\tabincell{c}{\(\nu = 1\)}}&ResNet18 & 0.772 & 0.7686 & 0.7742 & 0.7914 & 0.7704 & 0.7823 & 0.7852 & 0.7925 & 0.7827 \\ 
			&ResNet34 & 0.8225 & 0.7932 & 0.8407 & 0.8297 & 0.819 & 0.8429 & 0.8069 & 0.8587 & 0.8052 \\ 
			&ResNet50& 0.8558 & 0.8882 & 0.8913 & 0.8713 & 0.8888 & 0.8421 & 0.8649 & 0.8625 & 0.8094 \\ 
			&ResNet101& 0.9412 & 0.9235 & 0.9448 & 0.924 & 0.944 & 0.9472 & 0.9457 & 0.9424 & 0.9456 \\ 
			&ResNet152& 0.9601 & 0.9614 & 0.951 & 0.9699 & 0.9618 & 0.9659 & 0.9653 & 0.9562 & 0.9568 \\ 
			
			\midrule
			\multirow{5}{*}{\tabincell{c}{\(\nu = 1\)}}&ResNet18 & 0.7927 & 0.7952 & 0.78 & 0.7603 & 0.7611 & 0.7717 & 0.7557 & 0.7518 & 0.7935 \\ 
			&ResNet34 & 0.8472 & 0.855 & 0.8238 & 0.8571 & 0.815 & 0.8039 & 0.8156 & 0.8343 & 0.825 \\ 
			&ResNet50& 0.8446 & 0.8312 & 0.8808 & 0.8564 & 0.8947 & 0.846 & 0.8538 & 0.8561 & 0.828 \\ 
			&ResNet101& 0.9337 & 0.9437 & 0.9341 & 0.9487 & 0.9445 & 0.9211 & 0.9456 & 0.9253 & 0.9346 \\ 
			&ResNet152& 0.9537 & 0.9656 & 0.9586 & 0.9674 & 0.9524 & 0.9631 & 0.9637 & 0.9695 & 0.957 \\ 
			
			\midrule
			\multirow{5}{*}{\tabincell{c}{\(\nu = 1\)}}&ResNet18 & 0.7545 & 0.7996 & 0.7937 & 0.7603 & 0.765 & 0.7606 & 0.7764 & 0.7923 & 0.76 \\ 
			&ResNet34 & 0.8327 & 0.7931 & 0.7933 & 0.8337 & 0.8267 & 0.8417 & 0.8136 & 0.8487 & 0.8462 \\ 
			&ResNet50& 0.824 & 0.8372 & 0.8425 & 0.8535 & 0.8953 & 0.8632 & 0.8241 & 0.8263 & 0.848 \\ 
			&ResNet101& 0.939 & 0.9463 & 0.9365 & 0.9282 & 0.9302 & 0.9455 & 0.95 & 0.9461 & 0.9244 \\ 
			&ResNet152& 0.9522 & 0.9524 & 0.9631 & 0.9554 & 0.9556 & 0.9504 & 0.956 & 0.969 & 0.9511 \\ 
			\bottomrule
		\end{tabular}
	}
\end{table}



\begin{table}[H]
	\footnotesize
	\setlength{\abovecaptionskip}{0pt}%
	\setlength{\belowcaptionskip}{3pt}%
	\centering
	\caption{The discriminant results of Hongqiao-Baoan and based on IJRP}
	\setlength{\tabcolsep}{2mm}{  
		\begin{tabular}{clccccccccc}
			\toprule
			\(\nu\) & model & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
			\midrule
			\multirow{5}{*}{\tabincell{c}{\(K_1\)}}&ResNet18 & 0.6009 & 0.64 & 0.6343 & 0.6306 & 0.6153 & 0.6431 & 0.6384 & 0.6253 & 0.6007 \\ 
			&ResNet34 & 0.7323 & 0.7166 & 0.7056 & 0.7353 & 0.7245 & 0.7176 & 0.708 & 0.7349 & 0.7266 \\ 
			&ResNet50& 0.7665 & 0.8222 & 0.7532 & 0.7588 & 0.8066 & 0.7763 & 0.7743 & 0.7675 & 0.7541 \\ 
			&ResNet101& 0.847 & 0.8514 & 0.8578 & 0.8446 & 0.8413 & 0.8488 & 0.8534 & 0.8478 & 0.8455 \\ 
			&ResNet152& 0.9197 & 0.9056 & 0.9199 & 0.9196 & 0.9154 & 0.9098 & 0.9084 & 0.9087 & 0.9115 \\ 
			
			\midrule
			\multirow{5}{*}{\tabincell{c}{\(K_1\)}}&ResNet18 & 0.6238 & 0.6403 & 0.6368 & 0.6057 & 0.6257 & 0.6434 & 0.6016 & 0.6408 & 0.6202 \\ 
			&ResNet34 & 0.7134 & 0.705 & 0.7329 & 0.7253 & 0.7325 & 0.7314 & 0.7281 & 0.7018 & 0.7315 \\ 
			&ResNet50& 0.8283 & 0.7934 & 0.7676 & 0.7799 & 0.8275 & 0.7506 & 0.8285 & 0.7712 & 0.7921 \\ 
			&ResNet101& 0.8596 & 0.8561 & 0.8424 & 0.8444 & 0.8414 & 0.8465 & 0.8587 & 0.8482 & 0.8443 \\ 
			&ResNet152& 0.9052 & 0.9133 & 0.9023 & 0.9045 & 0.9044 & 0.9065 & 0.9134 & 0.9079 & 0.9085 \\ 
			
			\midrule
			\multirow{5}{*}{\tabincell{c}{\(K_1\)}}&ResNet18 & 0.6062 & 0.6367 & 0.6225 & 0.6391 & 0.649 & 0.6326 & 0.6116 & 0.6273 & 0.6162 \\ 
			&ResNet34 & 0.7184 & 0.7036 & 0.7237 & 0.7107 & 0.7245 & 0.7308 & 0.7243 & 0.7144 & 0.7251 \\ 
			&ResNet50& 0.7637 & 0.8088 & 0.7839 & 0.7889 & 0.8229 & 0.8074 & 0.8272 & 0.7779 & 0.8269 \\ 
			&ResNet101& 0.8481 & 0.8571 & 0.8563 & 0.8443 & 0.8548 & 0.8468 & 0.8584 & 0.8444 & 0.8405 \\ 
			&ResNet152& 0.9046 & 0.9129 & 0.9153 & 0.9052 & 0.9066 & 0.9108 & 0.9142 & 0.9095 & 0.9 \\ 
			
			\midrule
			\bottomrule
		\end{tabular}
	}
\end{table}











%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Discrimination results based on imaging method RP} \label{unRP}
%\setlength{\tabcolsep}{2mm}{
	%\begin{tabular}{ccccccccccccc}
	%\toprule
	%DGP& \(\nu\) & Acc. & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule 
	%\multirow{5}{*}{\tabincell{c}{DGP1}} &\(\nu = 1\) & 0.6428 & 0.6428 & 0.6604 & 0.6674 & 0.6961 & 0.6898 & 0.6966 & 0.6134 & 0.663 & 0.6681 \\ 
	%&\(\nu = 5\)& 0.7124 & 0.6428 & 0.6759 & 0.6815 & 0.7381 & 0.6846 & 0.7285 & 0.6645 & 0.6663 & 0.665 \\ 
	%&\(\nu = 10\)& 0.8272& 0.6428  & 0.8042 & 0.8033 & 0.8002 & 0.8181 & 0.8115 & 0.8137 & 0.8181 & 0.8357 \\ 
	%&\(\nu = 15\)& 0.8481 & 0.6428 & 0.8446 & 0.8692 & 0.8591 & 0.8441 & 0.8564 & 0.8868 & 0.8733 & 0.8605 \\ 
	%&\(\nu = 20\)& 0.9526& 0.6428  & 0.9457 & 0.9436 & 0.9254 & 0.93 & 0.9663 & 0.9017 & 0.9139 & 0.9249 \\ 
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{DGP2}} &\(\nu = 1\) & 0.6428 & 0.603 & 0.631 & 0.6784 & 0.6649 & 0.6142 & 0.6489 & 0.6922 & 0.6244 & 0.6393 \\ 
	%&\(\nu = 5\) & 0.6428 & 0.6785 & 0.6575 & 0.6832 & 0.7435 & 0.7498 & 0.6958 & 0.7255 & 0.6761 & 0.7428 \\ 
	%&\(\nu = 10\)& 0.6428 & 0.811 & 0.8044 & 0.8429 & 0.8252 & 0.8212 & 0.8365 & 0.8363 & 0.8498 & 0.8267 \\ 
	%&\(\nu = 15\)& 0.6428 & 0.855 & 0.8541 & 0.8471 & 0.8465 & 0.8447 & 0.8685 & 0.8406 & 0.8897 & 0.8719 \\ 
	%&\(\nu = 20\)& 0.6428 & 0.94 & 0.9174 & 0.9524 & 0.9195 & 0.9607 & 0.9128 & 0.9069 & 0.9674 & 0.9383 \\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{DGP2}} &\(\nu = 1\) & 0.6428  & 0.6548 & 0.6085 & 0.6964 & 0.6335 & 0.692 & 0.6255 & 0.6309 & 0.6487 & 0.6 \\ 
	%&\(\nu = 5\) & 0.6428 & 0.6763 & 0.7051 & 0.6824 & 0.706 & 0.7101 & 0.6766 & 0.716 & 0.6534 & 0.6768 \\ 
	%&\(\nu = 10\) & 0.6428 & 0.8071 & 0.8001 & 0.8265 & 0.826 & 0.832 & 0.8285 & 0.8494 & 0.8248 & 0.8312 \\ 
	%&\(\nu = 15\) & 0.6428 & 0.8482 & 0.8868 & 0.8699 & 0.8686 & 0.8513 & 0.8722 & 0.8648 & 0.8662 & 0.8869 \\ 
	%&\(\nu = 20\) & 0.6428 & 0.9619 & 0.9353 & 0.9006 & 0.93 & 0.909 & 0.9188 & 0.9649 & 0.9105 & 0.9141 \\
	%\bottomrule
	%\end{tabular}
	%}
%\end{table}



%\begin{table}[H]
%	\footnotesize
%	\setlength{\abovecaptionskip}{0pt}%
%	\setlength{\belowcaptionskip}{3pt}%
%	\centering
%	\caption{Discrimination results based on imaging method IRP} \label{unIRP} 
%	\setlength{\tabcolsep}{2mm}{
	%		\begin{tabular}{ccccccccccc}
		%			\toprule
		%			DGP& kernel & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
		%			\midrule
		%			\multirow{3}{*}{\tabincell{c}{DGP1}} &\(K_1\) & 0.6428 & 0.6604 & 0.6674 & 0.6961 & 0.6898 & 0.6966 & 0.6134 & 0.663 & 0.6681 \\ 
		%			&\(K_2\)& 0.7124 & 0.6759 & 0.6815 & 0.7381 & 0.6846 & 0.7285 & 0.6645 & 0.6663 & 0.665 \\ 
		%			&\(K_3\)& 0.8272 & 0.8042 & 0.8033 & 0.8002 & 0.8181 & 0.8115 & 0.8137 & 0.8181 & 0.8357 \\ 
		%			\midrule
		%			\multirow{3}{*}{\tabincell{c}{DGP2}} &\(K_1\) & 0.603 & 0.631 & 0.6784 & 0.6649 & 0.6142 & 0.6489 & 0.6922 & 0.6244 & 0.6393 \\ 
		%			&\(K_2\) & 0.6785 & 0.6575 & 0.6832 & 0.7435 & 0.7498 & 0.6958 & 0.7255 & 0.6761 & 0.7428 \\ 
		%			&\(K_3\)& 0.811 & 0.8044 & 0.8429 & 0.8252 & 0.8212 & 0.8365 & 0.8363 & 0.8498 & 0.8267 \\
		%			\midrule
		%			\multirow{3}{*}{\tabincell{c}{DGP3}} &\(K_1\) & 0.6548 & 0.6085 & 0.6964 & 0.6335 & 0.692 & 0.6255 & 0.6309 & 0.6487 & 0.6 \\ 
		%			&\(K_2\) & 0.6763 & 0.7051 & 0.6824 & 0.706 & 0.7101 & 0.6766 & 0.716 & 0.6534 & 0.6768 \\ 
		%			&\(K_3\)& 0.8071 & 0.8001 & 0.8265 & 0.826 & 0.832 & 0.8285 & 0.8494 & 0.8248 & 0.8312 \\
		%			\bottomrule
		%		\end{tabular}
	%	}
%\end{table}

% 这里需要选择单变量时间序列判别方法.




%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Interval vector-valued time series discriminant results based on JRP}
%\setlength{\tabcolsep}{2mm}{
	%\begin{tabular}{cccccccccccc}
	%	\toprule
	%	DGP& \(\nu\) & Acc. & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%	\midrule
	%	\multirow{5}{*}{\tabincell{c}{C1}} &\(\nu = 1\) & & 0.6428 & 0.6604 & 0.6674 & 0.6961 & 0.6898 & 0.6966 & 0.6134 & 0.663 & 0.6681 \\ 
	%	&\(\nu = 5\)& &0.7124 & 0.6759 & 0.6815 & 0.7381 & 0.6846 & 0.7285 & 0.6645 & 0.6663 & 0.665 \\ 
	%	&\(\nu = 10\)& &0.8272 & 0.8042 & 0.8033 & 0.8002 & 0.8181 & 0.8115 & 0.8137 & 0.8181 & 0.8357 \\ 
	%	&\(\nu = 15\)& & 0.8481 & 0.8446 & 0.8692 & 0.8591 & 0.8441 & 0.8564 & 0.8868 & 0.8733 & 0.8605 \\ 
	%	&\(\nu = 20\)& &0.9526 & 0.9457 & 0.9436 & 0.9254 & 0.93 & 0.9663 & 0.9017 & 0.9139 & 0.9249 \\ 
	%	\midrule
	%	\multirow{5}{*}{\tabincell{c}{C2}} &\(\nu = 1\) &&  0.603 & 0.631 & 0.6784 & 0.6649 & 0.6142 & 0.6489 & 0.6922 & 0.6244 & 0.6393 \\ 
	%	&\(\nu = 5\) & &0.6785 & 0.6575 & 0.6832 & 0.7435 & 0.7498 & 0.6958 & 0.7255 & 0.6761 & 0.7428 \\ 
	%	&\(\nu = 10\)&& 0.811 & 0.8044 & 0.8429 & 0.8252 & 0.8212 & 0.8365 & 0.8363 & 0.8498 & 0.8267 \\ 
	%	&\(\nu = 15\)& &0.855 & 0.8541 & 0.8471 & 0.8465 & 0.8447 & 0.8685 & 0.8406 & 0.8897 & 0.8719 \\ 
	%	&\(\nu = 20\)& &0.94 & 0.9174 & 0.9524 & 0.9195 & 0.9607 & 0.9128 & 0.9069 & 0.9674 & 0.9383 \\
	%	\bottomrule
	%\end{tabular}
	%}
%\end{table}
%
%
%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Interval vector-valued time series discriminant results based on IJRP}
%\setlength{\tabcolsep}{2mm}{
	%\begin{tabular}{cccccccccccc}
	%	\toprule
	%	DGP& kernel &Acc. & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%	\midrule
	%	\multirow{3}{*}{\tabincell{c}{C1}} &\(K_1\) & & 0.6428 & 0.6604 & 0.6674 & 0.6961 & 0.6898 & 0.6966 & 0.6134 & 0.663 & 0.6681 \\ 
	%	&\(K_2\)&  &0.7124 & 0.6759 & 0.6815 & 0.7381 & 0.6846 & 0.7285 & 0.6645 & 0.6663 & 0.665 \\ 
	%	&\(K_3\)&  & 0.8272 & 0.8042 & 0.8033 & 0.8002 & 0.8181 & 0.8115 & 0.8137 & 0.8181 & 0.8357 \\ 
	%	\midrule
	%	\multirow{3}{*}{\tabincell{c}{C1}} &\(K_1\) &  & 0.603 & 0.631 & 0.6784 & 0.6649 & 0.6142 & 0.6489 & 0.6922 & 0.6244 & 0.6393 \\ 
	%	&\(K_2\) & &  0.6785 & 0.6575 & 0.6832 & 0.7435 & 0.7498 & 0.6958 & 0.7255 & 0.6761 & 0.7428 \\ 
	%	&\(K_3\)& & 0.811 & 0.8044 & 0.8429 & 0.8252 & 0.8212 & 0.8365 & 0.8363 & 0.8498 & 0.8267 \\
	%	\bottomrule
	%\end{tabular}
	%}
%\end{table}

%\begin{table}[H]
%	\footnotesize
%	\setlength{\abovecaptionskip}{0pt}%
%	\setlength{\belowcaptionskip}{3pt}%
%	\centering
%	\caption{Univariate interval-valued time series discriminant results based on RP}
%	\setlength{\tabcolsep}{2mm}{
	%		\begin{tabular}{ccccccccccc}
		%			\toprule
		%			DGP& \(\nu\) & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
		%			\midrule
		%			\multirow{5}{*}{\tabincell{c}{H-S}} &\(\nu = 1\) & 0.6428 & 0.6604 & 0.6674 & 0.6961 & 0.6898 & 0.6966 & 0.6134 & 0.663 & 0.6681 \\ 
		%			&\(\nu = 5\)& 0.7124 & 0.6759 & 0.6815 & 0.7381 & 0.6846 & 0.7285 & 0.6645 & 0.6663 & 0.665 \\ 
		%			&\(\nu = 10\)& 0.8272 & 0.8042 & 0.8033 & 0.8002 & 0.8181 & 0.8115 & 0.8137 & 0.8181 & 0.8357 \\ 
		%			&\(\nu = 15\)& 0.8481 & 0.8446 & 0.8692 & 0.8591 & 0.8441 & 0.8564 & 0.8868 & 0.8733 & 0.8605 \\ 
		%			&\(\nu = 20\)& 0.9526 & 0.9457 & 0.9436 & 0.9254 & 0.93 & 0.9663 & 0.9017 & 0.9139 & 0.9249 \\ 
		%			\midrule
		%			\multirow{5}{*}{\tabincell{c}{S-T-B}} &\(\nu = 1\) & 0.603 & 0.631 & 0.6784 & 0.6649 & 0.6142 & 0.6489 & 0.6922 & 0.6244 & 0.6393 \\ 
		%			&\(\nu = 5\) & 0.6785 & 0.6575 & 0.6832 & 0.7435 & 0.7498 & 0.6958 & 0.7255 & 0.6761 & 0.7428 \\ 
		%			&\(\nu = 10\)& 0.811 & 0.8044 & 0.8429 & 0.8252 & 0.8212 & 0.8365 & 0.8363 & 0.8498 & 0.8267 \\ 
		%			&\(\nu = 15\)& 0.855 & 0.8541 & 0.8471 & 0.8465 & 0.8447 & 0.8685 & 0.8406 & 0.8897 & 0.8719 \\ 
		%			&\(\nu = 20\)& 0.94 & 0.9174 & 0.9524 & 0.9195 & 0.9607 & 0.9128 & 0.9069 & 0.9674 & 0.9383 \\
		%			\midrule
		%			\multirow{5}{*}{\tabincell{c}{H-S-T-B}} &\(\nu = 1\) & 0.6548 & 0.6085 & 0.6964 & 0.6335 & 0.692 & 0.6255 & 0.6309 & 0.6487 & 0.6 \\ 
		%			&\(\nu = 5\) & 0.6763 & 0.7051 & 0.6824 & 0.706 & 0.7101 & 0.6766 & 0.716 & 0.6534 & 0.6768 \\ 
		%			&\(\nu = 10\)& 0.8071 & 0.8001 & 0.8265 & 0.826 & 0.832 & 0.8285 & 0.8494 & 0.8248 & 0.8312 \\ 
		%			&\(\nu = 15\)& 0.8482 & 0.8868 & 0.8699 & 0.8686 & 0.8513 & 0.8722 & 0.8648 & 0.8662 & 0.8869 \\ 
		%			&\(\nu = 20\)& 0.9619 & 0.9353 & 0.9006 & 0.93 & 0.909 & 0.9188 & 0.9649 & 0.9105 & 0.9141 \\
		%			\bottomrule
		%		\end{tabular}
	%	} 
%\end{table}


%\begin{table}[H]
%	\footnotesize
%	\setlength{\abovecaptionskip}{0pt}%
%	\setlength{\belowcaptionskip}{3pt}%
%	\centering
%	\caption{Univariate interval-valued time series discriminant results based on IRP}
%	\setlength{\tabcolsep}{2mm}{
	%		\begin{tabular}{ccccccccccc}
		%			\toprule
		%			DGP& kernel & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
		%			\midrule
		%			\multirow{3}{*}{\tabincell{c}{H-S}} &\(K_1\) & 0.6428 & 0.6604 & 0.6674 & 0.6961 & 0.6898 & 0.6966 & 0.6134 & 0.663 & 0.6681 \\ 
		%			&\(K_2\)& 0.7124 & 0.6759 & 0.6815 & 0.7381 & 0.6846 & 0.7285 & 0.6645 & 0.6663 & 0.665 \\ 
		%			&\(K_3\)& 0.8272 & 0.8042 & 0.8033 & 0.8002 & 0.8181 & 0.8115 & 0.8137 & 0.8181 & 0.8357 \\ 
		%			\midrule
		%			\multirow{3}{*}{\tabincell{c}{S-T-B}} &\(K_1\) & 0.603 & 0.631 & 0.6784 & 0.6649 & 0.6142 & 0.6489 & 0.6922 & 0.6244 & 0.6393 \\ 
		%			&\(K_2\) & 0.6785 & 0.6575 & 0.6832 & 0.7435 & 0.7498 & 0.6958 & 0.7255 & 0.6761 & 0.7428 \\ 
		%			&\(K_3\)& 0.811 & 0.8044 & 0.8429 & 0.8252 & 0.8212 & 0.8365 & 0.8363 & 0.8498 & 0.8267 \\
		%			\midrule
		%			\multirow{3}{*}{\tabincell{c}{H-S-T-B}} &\(K_1\) & 0.6548 & 0.6085 & 0.6964 & 0.6335 & 0.692 & 0.6255 & 0.6309 & 0.6487 & 0.6 \\ 
		%			&\(K_2\) & 0.6763 & 0.7051 & 0.6824 & 0.706 & 0.7101 & 0.6766 & 0.716 & 0.6534 & 0.6768 \\ 
		%			&\(K_3\)& 0.8071 & 0.8001 & 0.8265 & 0.826 & 0.832 & 0.8285 & 0.8494 & 0.8248 & 0.8312 \\
		%			\bottomrule
		%		\end{tabular}
	%	}
%\end{table}


%\begin{table}[H] 
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Interval vector-valued time series discriminant results based on JRP}
%\setlength{\tabcolsep}{2mm}{
	%\begin{tabular}{ccccccccccc}
	%\toprule
	%DGP& \(\nu\) & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{H-S}} &\(\nu = 1\) & 0.6428 & 0.6604 & 0.6674 & 0.6961 & 0.6898 & 0.6966 & 0.6134 & 0.663 & 0.6681 \\ 
	%&\(\nu = 5\)& 0.7124 & 0.6759 & 0.6815 & 0.7381 & 0.6846 & 0.7285 & 0.6645 & 0.6663 & 0.665 \\ 
	%&\(\nu = 10\)& 0.8272 & 0.8042 & 0.8033 & 0.8002 & 0.8181 & 0.8115 & 0.8137 & 0.8181 & 0.8357 \\ 
	%&\(\nu = 15\)& 0.8481 & 0.8446 & 0.8692 & 0.8591 & 0.8441 & 0.8564 & 0.8868 & 0.8733 & 0.8605 \\ 
	%&\(\nu = 20\)& 0.9526 & 0.9457 & 0.9436 & 0.9254 & 0.93 & 0.9663 & 0.9017 & 0.9139 & 0.9249 \\ 
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{S-T-B}} &\(\nu = 1\) & 0.603 & 0.631 & 0.6784 & 0.6649 & 0.6142 & 0.6489 & 0.6922 & 0.6244 & 0.6393 \\ 
	%&\(\nu = 5\) & 0.6785 & 0.6575 & 0.6832 & 0.7435 & 0.7498 & 0.6958 & 0.7255 & 0.6761 & 0.7428 \\ 
	%&\(\nu = 10\)& 0.811 & 0.8044 & 0.8429 & 0.8252 & 0.8212 & 0.8365 & 0.8363 & 0.8498 & 0.8267 \\ 
	%&\(\nu = 15\)& 0.855 & 0.8541 & 0.8471 & 0.8465 & 0.8447 & 0.8685 & 0.8406 & 0.8897 & 0.8719 \\ 
	%&\(\nu = 20\)& 0.94 & 0.9174 & 0.9524 & 0.9195 & 0.9607 & 0.9128 & 0.9069 & 0.9674 & 0.9383 \\
	%\midrule
	%\multirow{5}{*}{\tabincell{c}{H-S-T-B}} &\(\nu = 1\) & 0.6548 & 0.6085 & 0.6964 & 0.6335 & 0.692 & 0.6255 & 0.6309 & 0.6487 & 0.6 \\ 
	%&\(\nu = 5\) & 0.6763 & 0.7051 & 0.6824 & 0.706 & 0.7101 & 0.6766 & 0.716 & 0.6534 & 0.6768 \\ 
	%&\(\nu = 10\)& 0.8071 & 0.8001 & 0.8265 & 0.826 & 0.832 & 0.8285 & 0.8494 & 0.8248 & 0.8312 \\ 
	%&\(\nu = 15\)& 0.8482 & 0.8868 & 0.8699 & 0.8686 & 0.8513 & 0.8722 & 0.8648 & 0.8662 & 0.8869 \\ 
	%&\(\nu = 20\)& 0.9619 & 0.9353 & 0.9006 & 0.93 & 0.909 & 0.9188 & 0.9649 & 0.9105 & 0.9141 \\
	%\bottomrule
	%\end{tabular}
	%} 
%\end{table}
%
%
%\begin{table}[H]
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Interval vector-valued time series discriminant results based on IJRP}
%\setlength{\tabcolsep}{2mm}{
	%\begin{tabular}{ccccccccccc}
	%\toprule
	%DGP& kernel & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%\midrule
	%\multirow{3}{*}{\tabincell{c}{H-S}} &\(K_1\) & 0.6428 & 0.6604 & 0.6674 & 0.6961 & 0.6898 & 0.6966 & 0.6134 & 0.663 & 0.6681 \\ 
	%&\(K_2\)& 0.7124 & 0.6759 & 0.6815 & 0.7381 & 0.6846 & 0.7285 & 0.6645 & 0.6663 & 0.665 \\ 
	%&\(K_3\)& 0.8272 & 0.8042 & 0.8033 & 0.8002 & 0.8181 & 0.8115 & 0.8137 & 0.8181 & 0.8357 \\ 
	%\midrule
	%\multirow{3}{*}{\tabincell{c}{S-T-B}} &\(K_1\) & 0.603 & 0.631 & 0.6784 & 0.6649 & 0.6142 & 0.6489 & 0.6922 & 0.6244 & 0.6393 \\ 
	%&\(K_2\) & 0.6785 & 0.6575 & 0.6832 & 0.7435 & 0.7498 & 0.6958 & 0.7255 & 0.6761 & 0.7428 \\ 
	%&\(K_3\)& 0.811 & 0.8044 & 0.8429 & 0.8252 & 0.8212 & 0.8365 & 0.8363 & 0.8498 & 0.8267 \\
	%\midrule
	%\multirow{3}{*}{\tabincell{c}{H-S-T-B}} &\(K_1\) & 0.6548 & 0.6085 & 0.6964 & 0.6335 & 0.692 & 0.6255 & 0.6309 & 0.6487 & 0.6 \\ 
	%&\(K_2\) & 0.6763 & 0.7051 & 0.6824 & 0.706 & 0.7101 & 0.6766 & 0.716 & 0.6534 & 0.6768 \\ 
	%&\(K_3\)& 0.8071 & 0.8001 & 0.8265 & 0.826 & 0.832 & 0.8285 & 0.8494 & 0.8248 & 0.8312 \\
	%\bottomrule
	%\end{tabular}
	%}
%\end{table}


%\begin{table}[H] 
%\footnotesize
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{The discriminant results of Hongqiao-Baoan and based on JRP}
%\setlength{\tabcolsep}{2mm}{
	%\begin{tabular}{cccccccccc}
	%	\toprule
	%	\(\nu\) & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
	%	\midrule
	%	\(\nu = 1\) & 0.6428 & 0.6604 & 0.6674 & 0.6961 & 0.6898 & 0.6966 & 0.6134 & 0.663 & 0.6681 \\ 
	%	\(\nu = 5\)& 0.7124 & 0.6759 & 0.6815 & 0.7381 & 0.6846 & 0.7285 & 0.6645 & 0.6663 & 0.665 \\ 
	%	\(\nu = 10\)& 0.8272 & 0.8042 & 0.8033 & 0.8002 & 0.8181 & 0.8115 & 0.8137 & 0.8181 & 0.8357 \\ 
	%	\(\nu = 15\)& 0.8481 & 0.8446 & 0.8692 & 0.8591 & 0.8441 & 0.8564 & 0.8868 & 0.8733 & 0.8605 \\ 
	%	\(\nu = 20\)& 0.9526 & 0.9457 & 0.9436 & 0.9254 & 0.93 & 0.9663 & 0.9017 & 0.9139 & 0.9249 \\
	%	\bottomrule
	%\end{tabular}
	%} 
%\end{table}
%
%
%\begin{table}[H]
%	\footnotesize
%	\setlength{\abovecaptionskip}{0pt}%
%	\setlength{\belowcaptionskip}{3pt}%
%	\centering
%	\caption{The discriminant results of Hongqiao-Baoan and based on IJRP}
%	\setlength{\tabcolsep}{2mm}{
	%		\begin{tabular}{cccccccccc}
		%			\toprule
		%			kernel & miP & maP & weiP  & miR & maR & weiR & miF\(_1\) & maF\(_1\) & weiF\(_1\)\\
		%			\midrule
		%			\(K_1\) & 0.6428 & 0.6604 & 0.6674 & 0.6961 & 0.6898 & 0.6966 & 0.6134 & 0.663 & 0.6681 \\ 
		%			\(K_2\)& 0.7124 & 0.6759 & 0.6815 & 0.7381 & 0.6846 & 0.7285 & 0.6645 & 0.6663 & 0.665 \\ 
		%			\(K_3\)& 0.8272 & 0.8042 & 0.8033 & 0.8002 & 0.8181 & 0.8115 & 0.8137 & 0.8181 & 0.8357 \\ 
		%			\bottomrule
		%		\end{tabular}
	%	}
%\end{table}
%



















%Time series widely available in the various disciplines as well as in applications. The analysis and modelling of time series perform an essential part in a variety of fields including, but not limited to, climate modelling \cite{mudelsee2019trend}, bioscience \cite{stoffer2012special}, medicine \cite{topol2019high} and business decision making \cite{bose2017probabilistic}. Supervised learning of time series, i.e. prediction and discriminant, is considered to be the crucially essential and challenging task. Conceptually, the time series modelling methods can be divided into traditional statistical learning methods and contemporary deep learning methods.
%
%Traditional time series prediction or discriminant methods primarily includes distance-based \cite{gorecki2015multivariate, orsenigo2010combining}, feature-based \cite{schafer2016scalable}, and ensemble methods \cite{lines2015time, wang2017deep}. The distance-based methods are primarily based on certain metrics to measure the similarity between the raw time series, such as the common Euclidean norm and Dynamic Time Wrapping (DTW) \cite{keogh2005exact}. \citet{tsinaslanidis2014prediction} combined Perceptually Important Points (PIPs) and DTW to test the weak-form Efficient Market Hypothesis (EMH), where PIPs is used to identify significant points in financial time series and DTW is employed to express the similarity of time series with unequal lengths. \citet{jeong2011weighted} proposed a weighted DTW in terms of imposing a penalty to points with a high phase difference from the reference point, and proposed a relatively robust time series discriminant method. The Feature-based methods are primarily based on capturing global or local patterns in time series, either manually or by learning. \citet{schafer2016scalable} proposed Bag-Of-SFA-Symbols (BOSS) vector
%space model, which comprises two steps, firstly, a time series is transformed into its BOSS model and then the TF-IDF vector is computed for each class label, which is more computationally efficient and robust than the 1-nearest-neighbour DTW. The ensemble methods focus on boosting the performance of the model by assembling multiple weak classifiers in a specific fashion. \citet{wichard2004time} trained in several models from different model classes and combined them to build the final ensemble. See \cite{lines2015time, wang2017deep, qiu2014ensemble, zhang2007neural, wichard2004time} for more on ensemble for time series. The fundamental idea behind the supervised learning methods to time series mentioned above is to characterise the degree of similarity. It is particularly important to mention that a reasonable degree of similarity presupposes a good representation of the raw data, rather than being limited to a specific metric, and it is for this reason that the above methods are suffering from performance limitations in addressing large scale time series or complex patterns \cite{du2021adarnn}. 
%
%In recent years, deep learning techniques have enjoyed remarkable success in many disciplines as well as applications, and in some areas have even surpassed human performance. The utmost critical reason for the success of deep learning is considered to be having a sound representation of the raw data \cite{lecun2015deep}. In the context of time series modelling, the models represented by Recurrent Neural Networks (RNNs) and their variants, such as Gated Recurrent Unit (GRU) and Long Short Term Memory (LSTM), have achieved the currently optimal performance in numerous tasks concerning clustering \cite{DBLP:journals/tec/ChungFNL04, DBLP:conf/ijcai/LeiYVWD19}, prediction \cite{guen2019shape, bandara2020forecasting}, discriminant \cite{fulcher2014highly, bandara2020forecasting}, anomaly detection \cite{corizzo2020scalable}. These models mentioned above require no assumptions about the stationarity of the time series and are effective in identifying complex patterns of non-linearity, intra-dependence and distribution shift \cite{du2021adarnn}. Concretely, \citet{DBLP:conf/sigir/LaiCYL18} proposed LSTNet uses Convolution Neural Network (CNN) and RNN to extract short-term local dependency patterns among variables and long-term patterns of trend terms, and is employed for multivariate time series prediction; \citet{DBLP:conf/ijcai/QinSCCJC17} proposed the use of dual-stage attention to enhance RNN to address the issue that the Nonlinear autoregressive exogenous (NARX) model fails to capture long-term temporal dependencies. \citet{DBLP:conf/nips/SenYD19} constructed a hybrid model of two CNNs for high-dimensional time series, one of which was used to regularize the global matrix factorization. Further trends include combining deep learning with State space models to model uncertainty \cite{salinas2020deepar}, employing seq2seq for multi-step prediction \cite{10.5555/3495724.3496096, salinas2020deepar, DBLP:conf/nips/GuenT19}, and using Transformers structures \cite{DBLP:conf/nips/VaswaniSPUJGKP17} for sequence learning. The majority of the above models rely on a combination of attention mechanisms and deep models, which implies the importance of automatically extracting high quality features and handle the long term dependencies. 



%Time series analysis and modelling plays a vital role in areas including climate modelling \cite{mudelsee2019trend}, bioscience \cite{stoffer2012special}, medicine \cite{topol2019high}, and business decision making \cite{bose2017probabilistic}. Forecasting is the most sought after task in time series analysis and is also considered to be the most difficult, due to its importance in industrial, social and industrial applications. In general, methods for time series forecasting can be divided into traditional statistical methods and modern machine learning methods that incorporate deep learning 	models \cite{lim2021time}. Traditional time series forecasting methods focus on parametric models that combine domain expertise, such as autoregressive \cite{box2015time} and moving average \cite{fan2008nonlinear}, etc.  
%and , exponential smoothing \cite{winters1960forecasting, gardner1985exponential}, kernel regression \cite{nadaraya1964estimating} and structural time series models \cite{harvey1990forecasting}. 
%Meanwhile, Gaussian processes \cite{williams1996gaussian} and their recent extensions, i.e., deep Gaussian processes \cite{damianou2013deep}, are widely used in time series forecasting. 
%Naturally, in real applications, the statistical properties of time series, i.e., non-stationarity, are considered to change over time. Therefore, some more complex models are required to achieve better predictive performance. 
%In practical applications, the statistical properties of time series, such as non-stationarity, are considered to vary over time, thus requiring more sophisticated models to achieve better predictive performance. Over the years, a large number of studies, such as hidden markov models \cite{tuncel2018autoregressive}, dynamic Bayesian networks \cite{robinson2010learning}, Kalman filters \cite{de2020normalizing} and autoregressive integrated moving average model \cite{kalpakis2001distance} have provided more reliable and accurate models for modeling non-stationary time series, and important progress has been made. 

%In recent years, deep learning has achieved great success in many fields , and even outperforming humans in sub-tasks of computer vision, such as image discriminant \cite{he2016deep}.\cite{}
%However, in recent years, deep learning models represented by recurrent neural networks and their variants have achieved better performance in time series modeling \cite{salinas2020deepar, guen2019shape}, which not only makes no assumptions about the stationarity of the time series, but also recognizes the high degree of nonlinearity and complex interdependence in time series, suggesting that modern machine learning models, a data-driven approach, are more accurate and reliable than traditional time series modeling methods \cite{lim2021time}. The main reason for the great success of deep learning is believed to be the ability to learn complex data representations \cite{goodfellow2016deep}. Of course, deep learning has also made great progress in other cognitive domains \cite{krizhevsky2012imagenet, devlin2018bert, silver2016mastering}, and even outperforming humans in sub-tasks of computer vision, such as image discriminant \cite{he2016deep}.
%However, recently, recurrent neural networks, a deep learning model, has achieved better performance in time series modeling , In addition, with the rapid increase in data and computational power available for modeling, deep learning models have become a critical part of the next generation of time series prediction . 
%In more detail, recurrent neural networks and their variants gated recurrent unit and long short-term memory (LSTM) are popular in time series modeling because of the ability to automatically extract high-quality features from time series data and to tackle long-time dependence problems \cite{kuznetsov2014generalization, lai2018modeling}. Moreover, we should note that most time series tasks, such as clustering \cite{wang2006characteristic, bandara2020forecasting}, discriminant \cite{fulcher2014highly}, prediction \cite{talagala2018meta,talagala2021fformpp}, and anomaly detection \cite{corizzo2020scalable}, are essentially a matter of quantifying the similarity between the extracted features, so having a good representation of the time series is essential for modeling. 

%
%In this paper we simultaneously consider imaging-based time series prediction and discriminant tasks, and devise strategies to enhance performance accordingly. We extract features from a time series imaging perspective rather than directly as in the above studies. Certainly, there are several studies of modeling time series based on imaging methods. \citet{li2020forecasting} transform time series into images based on  (RP) and utilize fine-tuned deep neural networks to extract features from the images for M4 competition data prediction. However, the study merely considered a single imaging scheme and a single feature extraction network (FEN) construction paradigm, i.e. fine-tuned neural networks, without comparing with other imaging methods. \citet{wang2015encoding} utilizes CNNs to classify data sets obtained from different imaging methods for the purpose of classifying time series. Nevertheless, the similarity of images from different classes based on the identical imaging method was not considered in the selection of the discriminant method, and thus the imaging-based discriminant did not attain a sufficiently high accuracy. 


%We segment the time series disjointly at a specific length and then imaging the segments based on four imaging methods, namely RP, Gramian Angular Summation Field (GASF) \cite{wang2015encoding}, Gramian Angular Difference Field (GADF) \cite{wang2015encoding} and Markov Transition Field (MTF) \cite{liu2018encoding}, respectively. In addition, by treating the images obtained from each imaging methods as a class, we can logically obtain an image data set containing four classes. 


%From the perspective of feature extraction, in this paper, we propose a time series feature extraction procedure based on time series imaging and deep representation learning for time series prediction. Firstly, we segment the time series disjointly at a specific length and then imaging the segments based on four imaging modalities, namely Recurrence Plot (RP), Gramian Angular Summation Field (GASF) \cite{wang2015encoding}, Gramian Angular Difference Field (GADF) \cite{wang2015encoding} and Markov Transition Field (MTF) \cite{liu2018encoding}, respectively. In addition, by treating the images obtained from each imaging modality as a class, we can logically obtain an image data set containing four classes. We should note that the segmentation length needs to be artificially specified as a hyperparameter, but the experimental results in Section \ref{sec5} show that the prediction performance appears to be robust with respect to the segmentation length. Secondly, we selected VGG and ResNet \cite{he2016deep} with different number of layers as candidates for feature extraction networks (FENs) and trained them using image data sets. Remarkably, three different paradigms for FEN construction are considered, namely, self-training, pre-training and fine-tuning, mainly for the purpose of comparison, and the differences between these three paradigms are covered in detail in Section \ref{sec3}. Thirdly, to further improve the performance and robustness, we choose to use Adaboost \cite{zhou2012ensemble} to ensemble the prediction model, i.e., the support vector machine \cite{SmolaAlextutorialsvr2004}. In an empirical study, we apply the proposed feature extraction procedure to the daily minimum temperature dataset in Melbourne, and the experimental results show that different paradigms of FENs have a significant impact on the prediction performance, while the impact of different imaging modalities is subtle. 
%
%
%Not surprisingly, this has also been studied based on time series imaging and deep representation learning for time series extraction and use in prediction. 
%%also considers a depth representation of the time series and combines it with a prediction model for prediction, 
%The difference with our work that \citet{li2020forecasting} considers only one imaging modality, i.e., RP \cite{eckmann1995recurrence}, and there is no doubt that one imaging modality can extract only partial information of the time series. Additionally, \citet{li2020forecasting} considers only a shallow VGG19 \cite{simonyan2014very} as FEN, which may be insufficient for time series prediction. 


%The rest of the paper is organized as follows. The four imaging modalities are presented in section \ref{sec2}, and a total of three FEN construction paradigms are presented in section \ref{sec3}, section \ref{sec4} shows the prediction method based on feature extraction, the application of the method to daily minimum and maximum temperature data in Melbourne will be in section \ref{sec5}, and the corresponding conclusions and summaries as well as possible future research directions are given in section \ref{sec6}. 


%irstly, we segment the time series with a specific length, then we image the time series based on RP , . The images obtained by one imaging method are treated as one class, so naturally we can get an image dataset containing four classes and use different layers of VGG and ResNet  to train and obtain a feature extraction network (FEN). In this paper, we consider three different paradigms for FEN construction, namely, self-training FEN, where the neural network parameters are randomly initialized and trained on the imaging dataset, pre-training FEN, where the neural network is randomly initialized and trained on ImageNet \cite{deng2009imagenet}, and fine-tuning pre-training model, where the pre-trained model is trained again on the imaging data. Based on the above three paradigms of FENs, we choose the commonly used regression model Support Vector Regression (SVR)\cite{SmolaAlextutorialsvr2004} for prediction. To further improve the performance and robustness of the model, we ensemble SVR based on AdaBoost \cite{freund1997decision}, and the corresponding algorithm is given in section \ref{sec4}.




%\section{Time Series imaging} \label{sec2}
%In this section, we will profile the four imaging methods utilized in this paper. Time series imaging is the transformation of time series data into images is a way to transform information from one modality into another. The purpose of transformation into images is to benefit from the rapid development of computer vision technology at this stage, which can effectively extract the features of images and thus indirectly extract the features of time series. Furthermore, we should note that the four imaging modalities mentioned below are almost irreversible \cite{thiel2004much}, i.e., the time series and images are not equivalent, which is one of the reasons why we use four imaging modalities. Since the four imaging methods we describe below are all oriented to time series, without loss of generality, we state them in terms of time series \(\vx = \left\{x_1,x_2,\cdots,x_n\right\}\).
%
%\subsection{Recurrence Plot}
%Natural processes have distinct recursive behavior, such as periodic and irregular cyclicities. Furthermore, recurrence of states, i.e., states that are arbitrarily close after some time, is a fundamental property of both deterministic and nonlinear or chaotic systems. Usually, the phase space has dimensions that are not easily visualized, so the only way to see the recurrence of the phase space is to visualize it by projecting into a two- or three-dimensional subspace \cite{eckmann1995recurrence}. RP provides a way to visualize \(m\)-dimensional phase space trajectories in two dimensions, which is implemented as follows. RP first defines two trajectories of dimension \(m\), denoted as
%\[
%\vec{\vx}_i =\left(x_i, x_{i+\tau}, \cdots, x_{i+(m-1)\tau}\right),\ \vec{\vx}_j =\left(x_j, x_{j+\tau}, \cdots, x_{j+(m-1)\tau}\right), 
%\]
%where \(\tau\) is the time delay and \(i, j \in \left\{1,2,\cdots, n-(m-1)\tau\right\}\). Defining the RP matrix as \(\mR = \left(R_{ij}\right)\), it is natural to have
%\begin{equation}
%	R_{ij} = \mTheta(\epsilon - \Vert \vec{\vx}_i - \vec{\vx}_j \Vert), \label{rp}
%\end{equation}
%where \(\mTheta(\cdot)\) and \(\epsilon\) denote the Heaviside step function and the threshold value, respectively. From the definition of \(\mR\), there are two hyperparameters, threshold \(\epsilon\) and dimension \(m\), which determine whether \(\mR\) can present large-scale and small-scale features, i.e., typology features and texture features, where typology features are global features and can be described by homogeneous, periodic, drift and disrupted \cite{thiel2004much}. The default values of these hyperparameters are available in \textbf{pyts} \cite{JMLR:v21:19-763}, the time series analysis package for Python. 
%
%\subsection{Gramian Angular Field}
%Gramian Angular Field describes the correlation between any two terms of a time series in angular form \cite{wang2015encoding}. Given a time series \(\vx\), the Gramian Angular Field first scales each item in the time series to the interval \(\left[a, b\right]\), i.e. \(\widetilde{x}_i = a + (b-a)(x_i - \min(\vx)) / (\max(\vx) - \min(\vx))\), 
%and in general, \(\left[a, b\right]\) is \(\left[0, 1\right]\) or \(\left[-1, 1\right]\). Furthermore, by encoding \(\widetilde{x}_i\) as an angle through the \(\arccos(\cdot)\) and using the timestamp \(t_i\) as the radius, the polar coordinates of the deflated observable \(\widetilde{x}_i\) can be obtained as
%\[
%\phi_i = \arccos(\widetilde{x}_i), \ r_i = t_i / N, \ t_i\in \mathbb{N}, 
%\]
%where \(N\) is a constant used to regularize the polar coordinate system. By defining the correlation measure of any two terms \(x_i\) and \(x_j\) in the time series \(\vx\) as \(\cos(\phi_i + \phi_j)\) and \(\sin(\phi_i - \phi_j)\), the GASF and GADF \cite{wang2015imaging} can be defined as
%\begin{equation}
%	\text{GASF}= \mS = \left(s_{ij}\right) = \left(\cos(\phi_i + \phi_j)\right), \label{gasf}
%\end{equation}
%
%\begin{equation}
%	\text{GADF}= \mD = \left(s_{ij}\right) = \left(\sin(\phi_i - \phi_j)\right). \label{gadf}
%\end{equation}
%
%Since the dimension of GASF and GADF is \(n\times n\), where \(n\) is the length of time series \(\vx\), in order to reduce the size of GASF and GADF, 	\citet{wang2015encoding} suggests using piecewise aggregation approximation \cite{keogh2000scaling} to smooth \(\vx\) while preserving the time series trend. 
%
%
%\subsection{Markov Transition Field}
%Similar to GASF and GADF, MTF is also proposed by \cite{wang2015imaging}, but it is an improvement of Markov transition probabilities proposed by \cite{campanharo2011duality}, and the main aspect of its improvement is the preservation of information in the temporal dimension. Given a time series \(\vx\), MTF first determines \(Q\) bins, respectively \(q_1, q_2, \cdots, q_Q\), and satisfies \(\Phi(q_{i+1}) -\Phi(q_{i}) =1/Q\), where \(\Phi(\cdot)\) is the cumulative distribution function of the standard normal distribution. After assigning \(x_i\) to its corresponding bin \(q_j( j\in \left\{1,2,\cdots, Q\right\})\), we can construct a weight adjacency matrix \(\mW = \left(w_{ij}\right)\) of \(Q\times Q\) as follows
%\[
%\mW = \left[
%\begin{array}{cccc}
%	w_{11}|\mathbb{P}(x_t\in q_1 | x_{t-1}\in q_1) & w_{12}|\mathbb{P}(x_t\in q_1 | x_{t-1}\in q_2) & \cdots &w_{1Q}|\mathbb{P}(x_t\in q_1 | x_{t-1}\in q_Q)\\
%	w_{21}|\mathbb{P}(x_t\in q_2 | x_{t-1}\in q_1) & w_{22}|\mathbb{P}(x_t\in q_2 | x_{t-1}\in q_2) & \cdots &w_{2Q}|\mathbb{P}(x_t\in q_2 | x_{t-1}\in q_Q)\\
%	\vdots & \vdots & \ddots & \vdots\\
%	w_{Q1}|\mathbb{P}(x_t\in q_Q | x_{t-1}\in q_1) & w_{Q2}|\mathbb{P}(x_t\in q_Q | x_{t-1}\in q_2) & \cdots & w_{QQ}|\mathbb{P}(x_t\in q_Q | x_{t-1}\in q_Q)\\
%\end{array}
%\right], 
%\]
%where \(w_{ij}\) denotes the frequency of the point \(x_t\) in bin \(q_i\) and \(x_{t-1}\) in bin \(q_j\), and \(\mW\) is normalized, i.e., \(\sum_{j=1}w_{ij} = 1\). MTF solves the problem that \(\mW\) ignores the dependence of the distribution of \(\vx\) on time \(t_i\) by aligning each probability along the temporal order, which is defined as
%\begin{equation}
%	\mM=\left[
%	\begin{array}{cccc}
	%		m_{11} & m_{12} & \cdots & m_{1n}\\
	%		m_{21} & m_{22} & \cdots & m_{2n}\\
	%		\vdots & \vdots & \ddots & \vdots\\
	%		m_{n1} & m_{n2} & \cdots & m_{nn}\\
	%	\end{array}
%	\right],  \label{mtf}
%\end{equation}
%where \(m_{ij} = (w_{ij}|x_i \in q_i, x_j\in q_j)\) denotes the transition probability of \(q_i \to q_j\), and we should note that the quantile bins containing the data at time steps \(i\) and \(j\) (temporal axis) in \(\mM\) is \(q_i\) and \(q_j\). More details about MTF can be found in \cite{wang2015imaging}
%
%
%
%\section{Three paradigms for feature extraction networks construction}\label{sec3}
%Before prediction, we need to construct a FEN to extract features from the time series. Commonly, the following three paradigms are used to construct FENs: self-training, pre-training and fine-tuning. In the following, we will introduce the three paradigms in detail. 
%
%\begin{algorithm}[H]
%	\caption{The construction of self-training FENs}
%	\label{imagingcon}
%	\begin{algorithmic}
	%		\REQUIRE ~~\\
	%		Time series \(\vx = \left(x_1, x_2,\cdots,x_n\right)\),\\
	%		Segmentation length \(\left\{\Delta _1, \Delta_2, \cdots, \Delta_K\right\}\),\\
	%		Four time series imaging methods: RP (Eq.(\ref{rp})), GASF (Eq.(\ref{gasf})), GADF (Eq.(\ref{gadf})), MTF (Eq.(\ref{mtf})),\\
	%		FEN candidates: \(\text{FENs}=\left\{\right.\) VGG11, VGG13, VGG16, VGG19, ResNet18, ResNet34, ResNet50, ResNet101, ResNet152\(\left.\right\}\).\\
	%		\ENSURE ~~\\
	%		\textbf{For} \(k = 1,2,\cdots, K\)\\
	%		\quad \quad Constructing data sets for imaging \(\mathcal{I}_k\) based on Eq.(\ref{imagingd}).\\
	%		\quad \quad Constructing imaging data set
	%		\[
	%		\mathcal{B}_k = \left\{\left(\text{RP}(\mathcal{I}_k), 1\right), \left(\text{GASF}(\mathcal{I}_k), 2\right), \left(\text{GADF}(\mathcal{I}_k), 3\right), \left(\text{MTF}(\mathcal{I}_k), 4\right)\right\}.
	%		\]
	%		\quad \quad  \textbf{For} FEN \(\in\) FENs:\\
	%		\quad \quad \quad \quad Train FEN based on imaging data set \(\mathcal{B}_k\).\\
	%		\quad \quad \quad \quad Comput training loss \(\mathcal{L}_k\) and test accuracy \(\mathcal{C}_k\).\\
	%		\quad \quad \quad \quad Save the trained model FEN\(_k\).\\
	%		\quad \quad  \textbf{End}\\
	%		\textbf{End}\\
	%		\textbf{Output}: \(\left\{\left(\text{FEN}_k, \mathcal{L}_{\text{FEN}_k}, \mathcal{C}_{\text{FEN}_k}\right)\right\}, k=1,2,\cdots, K, \text{FEN} \in \text{FENs}\).
	%	\end{algorithmic}
%\end{algorithm}
%
%
%\subsection{Feature extraction based on self-training FENs}  \label{sec33}
%In this subsection, we propose a self-training FEN-based feature extraction, which consists of three main steps: (\expandafter{\romannumeral1}) time series segmentation and time series imaging, (\expandafter{\romannumeral2}) FEN training; and (\expandafter{\romannumeral3}) Extract the features of the penultimate layer as a representation of the corresponding time series. Below we will give a detailed description of these three steps. Before performing imaging, we should first construct the dataset for imaging, which is designed with a hyperparameter for the length of the time series segmentation. In addition, it should be noted that our time series segmentation is disjoint, so that any two images obtained using the same imaging method are less similar and improve the discriminant accuracy. Given a time series \(\vx = \left\{x_1, x_2, \cdots, x_n\right\}\), with \(\Delta\) denoting the segmentation length of the time series, it is natural to construct the following dataset for imaging
%\begin{equation}
%	\mathcal{I} = \left\{\vi_1, \vi_2, \cdots, \vi_{\lfloor n/\Delta \rfloor}\right\},  \label{imagingd}
%\end{equation}
%where \(\vi_j = \left(x_{1+(j-1)\times \Delta}, x_{2+(j-1)\times \Delta}, \cdots, x_{j \times \Delta}\right), j = 1,2,\cdots, \lfloor n/\Delta \rfloor\). We should note that the hyperparameter \(\Delta\) is related to some statistical properties of the time series, and in this paper we autonomously determine the set \(\left\{\Delta _1, \Delta_2, \cdots, \Delta_K\right\}\) and choose the optimal one from it. For details, please refer to Section \ref{sec5}. In addition, the candidates for the FENs are a series of VGG \cite{simonyan2014very} and ResNet \cite{he2016deep} with different layers, as VGG11, VGG13, VGG16, VGG19 and ResNet18, ResNet34, ResNet50, ResNet101, ResNet152. Algorithm \ref{imagingcon} gives the construction procedure of self-training FENs.
%
%
%In Algorithm \ref{imagingcon}, we calculate the training loss \(\mathcal{L}_k\) and test accuracy \(\mathcal{C}_k\) under each segmentation length and network structure for the purpose of determining whether it has an impact on the prediction performance. In order not to lose information due to image scaling, i.e., the same size of the image used for training the FEN and for feature extraction. For \(\text{FEN}_k, k=1,2,\cdots, K, \text{FEN} \in \text{FENs}\), we construct the following data set,
%\begin{equation}
%	\mathcal{T}_{\text{FEN}_k} = \left(\vx_j, y_j\right)^{n-\Delta_k}_{j=1}, \label{fenk}
%\end{equation}
%where  \(\vx_j = \left(x_j, x_{j+1}, \cdots, x_{\Delta_k +j-1}\right)\), and \(y_j = x_{\Delta_k +j}\) implies single-step prediction, and furthermore it is obvious that \(\vx_j, \vi_j \in \mathbb{R}^{\Delta_k}\), i.e., the images encoded have the same dimensionality. Based on the data set in Eq.(\ref{fenk}), we build the following data set after feature extraction,
%\begin{equation}
%	\mathcal{D}_{\text{FEN}_k} = \left(\text{FEN}_k(\text{Imaging}(\vx_j)), y_j\right)^{n-\Delta_k}_{j=1},  \label{dfen}
%\end{equation}
%where \(k=1,2,\cdots, K, \text{FEN} \in \text{FENs}\), \(\text{Imaging}(\cdot)\) indicates one of the four imaging methods in Section \ref{sec2} and in the following, we will fit and predict the time series based on the data set \(\mathcal{D}_{\text{FEN}_k}\). The feature extraction process based on self-training FENs is given in Figure \ref{fenconstruction}.
%\begin{figure}[H]
%	\centering
%	\includegraphics[scale=0.6]{figures/fenconstruction/fenconstructionw.pdf}
%	\caption{Feature extraction based on self-training FENs.} \label{fenconstruction}
%\end{figure}
%
%Since we selected VGG and ResNet with different layers, the representation of the original data differs between the layers of different depths, but we believe that the features input to softmax, i.e., the features in the penultimate layer of \(\text{FEN}_k\), have the best representation of the original data \cite{goodfellow2016deep}, so for different network architectures, we always select the penultimate layer as the representation of the original time series. In addition, we should note that, as shown in Eq.(\ref{dfen}), we will first image the time series before performing feature extraction on the original time series data, because it is uncertain in advance which imaging method for feature extraction is the best representation of the original data, i.e., has the best predictive performance, so all four imaging methods will be used for feature extraction and for performance comparison.
%
%
%
%
%\subsection{Feature extraction based on pre-trained FENs}
%Large-scale pre-trained models such as BERT \cite{zhang2020ternarybert} and GPT have recently achieved great success and become a milestone in artificial intelligence \cite{han2021pre}. Pre-trained models store knowledge in their large number of parameters and fine-tune them for specific tasks, which has benefited many artificial intelligence downstream tasks and has been heavily validated for both experimental and empirical analysis \cite{han2021pre}. Similarly, we used the pre-trained models of ResNet and VGG on the large-scale image data set ImageNet \cite{deng2009imagenet}. However, the difference is that we do not fine-tune the pre-training model, and the underlying reason is that this is an empirical exercise, and we cannot guarantee that fine-tuning will necessarily lead to an improvement in prediction performance. 
%
%In addition, as we will see from Section \ref{sec5}, the pre-trained model is weak in classifying the imaging data, i.e., the training loss is high and the test accuracy is low. As mentioned earlier, this does not mean that the features extracted based on the pretrained model cannot have better prediction performance.
%The feature extraction process based on the pre-training model is shown in the upper part (A) of Figure \ref{trasferlearning}.
%
%
%
%
%
%\subsection{Feature extraction based on fine-tuned FENs}
%The alternative to self-training FENs can be a fine-tuned pre-trained model. At this stage, the consensus in the artificial intelligence community is to use pre-trained models as the backbone in downstream tasks, rather than training a model from scratch \cite{han2021pre}. 
%
%As in subsection \ref{sec33}, the FENs we selected are still VGG and ResNet with different layers, but these models have been pre-trained on the large-scale data set ImageNet \cite{krizhevsky2012imagenet}. There are numerous ways to fine-tune the pre-trained model, and we choose a similar approach to \cite{li2020forecasting}, i.e., fixing all parameters from the first to the penultimate layer of the model and fine-tuning only the parameters in the penultimate layer using the imaging data set. The following operation is similar to the Subsection \ref{sec33}, based on the fine-tuned FENs to extract features from \(\vx_i\) in Eq.(\ref{fenk}), i.e., replacing the \(\text{FEN}_k\) in Eq.(\ref{dfen}) with the fine-tuned pre-trained model.
%
%The milestone that pre-trained models can be widely used for downstream tasks is due to the maturity of transfer learning \cite{thrun1998learning, pan2009survey} techniques. Transfer learning consists of two main phases, a pre-training phase for capturing knowledge from one or more source tasks, and a fine-tuning phase to apply the captured knowledge to the target task. In this paper our source task is the discriminant of ImagNet by VGG and ResNet with different layers and the target task is the feature extraction of time series imaging data set by VGG and ResNet. Figure \ref{trasferlearning} illustrates the process of feature extraction based on transfer learning. More details about the feature extraction will be given in Section \ref{sec4}.
%\begin{figure}[H]
%	\centering
%	\includegraphics[scale=0.7]{figures/trasferlearning/trasferlearning.pdf}
%	\caption{Feature extraction based on fine-tuned pre-training FENs.} \label{trasferlearning}
%\end{figure}
%
%For an arbitrary FEN \(f( \cdot| \mTheta)\), where \(\mTheta\) is the parameter to be learned and \(\mTheta_0\) denotes the parameter initialized randomly. Let \(\mathcal{L}(\text{Data}, \mTheta)\) denotes the loss, then we can summarize the parameter change process of the FEN for the three paradigms as follows:
%\begin{equation}
%	\begin{aligned} \label{paraupdate}
	%		&\text{Self-training FEN}: \mTheta_s \leftarrow  \mTheta_0 - \alpha_s \frac{\partial \mathcal{L}(\mathcal{B}, \mTheta)}{\partial \mTheta}, \\
	%		& \text{Pre-trained FEN}: \mTheta_p \leftarrow  \mTheta_0 - \alpha_p \frac{\partial \mathcal{L}(\text{ImageNet}, \mTheta)}{\partial \mTheta}, \\
	%		& \text{Fine-tuned pre-trained FEN}: \mTheta_f \leftarrow  \mTheta_p - \alpha_f \frac{\partial \mathcal{L}(\mathcal{B}, \mTheta)}{\partial \mTheta}, \\
	%	\end{aligned}
%\end{equation}
%where \(\alpha_s, \alpha_p, \alpha_f\) denote the learning rates of the self-trained, pre-trained and fine-tuned models, respectively. From Equation (\ref{paraupdate}), it is obvious that both self-training and pre-training are updated from randomly initialized parameters, the difference is that the data used is different; fine-tuning is updated from pre-trained parameters and uses its own data set. It is not difficult to obtain that fine-tuning should be the representation with the best performance.
%
%\section{Time series prediction based on extracted features} \label{sec4}
%After the feature extraction of the time series in Section \ref{sec3}, we can obtain the data set \(\mathcal{D}_{\text{FEN}_k} = \left(\text{FEN}_k(\text{Imaging}(\vx_j)), y_j\right)^{n-\Delta_k}_{j=1}, k=1,2,\cdots, K, \text{FEN} \in \text{FENs}\). In this section we will give a brief introduction to the prediction model based on the data set \(\mathcal{D}_{\text{FEN}_k}\). We believe that if the extracted features represent the raw data well, then a general model can also achieve an excellent prediction performance. In the paper, we selected a common regression model Support Vector Regression (SVR) \cite{SmolaAlextutorialsvr2004}, and to further improve the model performance and robustness, we ensemble SVR based on AdaBoost \cite{freund1997decision}.
%
%The SVR model is an extension of support vector machines to regression problems with good performance and interpretability. Support vector machine models were initially used to solve discriminant issues and are typically classified into three categories based on whether the data set is linearly separable, namely hard margins, soft margins (by introducing slack variables), and non-linearity (by using kernel techniques). There are very sophisticated optimization algorithms for solving the parameters of the support vector machine, which are conventionally transformed into dual problems for solving. In this paper, we introduce and use the soft-margin SVR model. By introducing slack variables \(\xi_i\) and \(\xi^*_i\), the soft margin SVR is equivalent to the following optimization problem
%\[
%\begin{aligned}
%	&\text{minimize } \frac{1}{2} \left\|\bm{w}\right\|^2 + C\sum_{i=1}^{n}(\xi_i + \xi_i^*), \\
%	& \text{S.t.} \left\{
%	\begin{array}{l}
	%		y_i - \bm{w}^\top \text{FEN}_k(\text{Imaging}(\vx_j)) - b \leq \nu + \xi_i, \\
	%		\bm{w}^\top \text{FEN}_k(\text{Imaging}(\vx_j)) + b - y_i\leq \nu + \xi^*_i, \\
	%		\xi_i, \xi_i^*  \geq 0, \\
	%	\end{array}
%	\right.	
%\end{aligned}
%\]
%the constant \(C > 0\) determines the trade-off between the flatness of 
%\[
%f = \bm{w}^\top \text{FEN}_k(\text{Imaging}(\vx_j)) + b
%\]
%and the amount up to which deviations larger than \(\nu\) are tolerated. The above optimization problem can be easily transformed into its dual problem and solved. Adaboost is a tandem, ensemble learning algorithm that continuously adjusts the weights of the samples and base learners during the learning process. 
%
%\begin{algorithm}[H]
%	\caption{Ensemble SVR based on Adaboost}
%	\label{svradaboost}
%	\begin{algorithmic}
	%		\REQUIRE ~~\\
	%		Training data \(\mathcal{D}_{\text{FEN}_k}\),\\
	%		Base learner \(G:\)\(\text{FEN}_k(\text{Imaging}(\vx)) \to y\),\\
	%		Number of learning rounds \(T\).\\
	%		\ENSURE ~~\\
	%		Initialize the weight distribution \(\mathbb{D}_1:\)\(p_i = \frac{1}{n-\Delta_k}, i = 1,2,\cdots, n-\Delta_k\),\\
	%		\textbf{For} \(t = 1,2,\cdots, T\)\\
	%		\quad \quad Draw \(n-\Delta_k\) samples (with replacement) \(\mathcal{D}^t_{\text{FEN}_k}\) from \(\mathcal{D}_{\text{FEN}_k}\) based on distribution \(\mathbb{D}_t\);\\
	%		\quad \quad Training the base learner \(G_t\) based on data \(\mathcal{D}^t_{\text{FEN}_k}\);\\
	%		\quad \quad Compute \(D_t = \max \abs{G^i_t(\text{FEN}_k(\text{Imaging}(\vx_i)))- y_i}\);\\
	%		\quad \quad Calculate the loss for each sample based on any one of the following three candidate losses:\\
	%		\[
	%		\begin{aligned}
		%			&\text{linear} \qquad	L_i = \frac{\abs{G^i_t(\text{FEN}_k(\text{Imaging}(\vx_i)))- y_i}}{D_t},\\
		%			&\text{square} \qquad	L_i = \frac{\abs{G^i_t(\text{FEN}_k(\text{Imaging}(\vx_i)))- y_i}^2}{D^2_t},\\
		%			&\text{exponential} \qquad	L_i =1-\exp\left\{-\frac{\abs{G^i_t(\text{FEN}_k(\text{Imaging}(\vx_i)))- y_i}}{D_t}\right\};
		%		\end{aligned}
	%		\]
	%		\quad \quad Calculate an average loss \(L_t = \sum\limits_{i=1}^{n-\Delta_k}L_i p_i\);\\
	%		\quad \quad Let 
	%		\begin{equation}\label{betaadaboost}
		%			\beta_t = \frac{L_t}{1-L_t}
		%		\end{equation}
	%		and update the weights
	%		\begin{equation}\label{weightsupdate}
		%			w_i \longleftarrow w_i \beta_t^{1-L_i}.
		%		\end{equation}
	%		\quad \quad Update weight distribution \(\mathbb{D}_t\).\\
	%		\textbf{End}\\
	%		\textbf{Output}:
	%		\[
	%		\mathcal{G}(\text{FEN}_k(\text{Imaging}(\vx))) = \inf \left\{y:\sum\limits_{t:G_t(\text{FEN}_k(\text{Imaging}(\vx))) \leq y }\log(1/\beta_t) \geq \frac{1}{2}\sum\limits_{t=1}^{T}\log(1/\beta_t)\right\}.
	%		\]
	%	\end{algorithmic}
%\end{algorithm}
%
%Let SVR be the base learner, Algorithm \ref{svradaboost} gives the SVR ensemble based on Adaboost \cite{zhou2012ensemble}. There are three common losses in Algorithm \ref{svradaboost}, namely linear, square and exponential losses; different losses yield different \(L_t\) in each learning round, and the update of the weight distribution behind them is also different, so a suitable loss function selection is necessary to achieve a faster convergence. The \(\beta_t\) in Eq.(\ref{betaadaboost}) is the confidence measure of \(G_t\), with smaller indicating better learning. We use Eq.(\ref{weightsupdate}) to update the weight distribution. It is clear that the greater the loss of \(G_t\) to sample \(\left(\text{FEN}_k(\text{Imaging}(\vx_j)), y_j\right)\), the greater the increase in its weight, then the greater the probability of being sampled in the next round of learning, resulting in a better performance of the final model.  Furthermore, we should note that for an arbitrary sample \(\text{FEN}_k(\text{Imaging}(\vx))\), we use the weighted median  \(\mathcal{G}(\text{FEN}_k(\text{Imaging}(\vx)))\) for prediction, which is more robust \cite{drucker1997improving}. 
%
%
%
%
%
%
%%Gradient boosting \cite{friedman2001greedy} trains a series of base classifiers in a sequential manner. Given data set \(\mathcal{D}_{\text{FEN}_k}\) (other data sets are similar), \(\mR(\vz) \in \mathbb{R}^k\) is the input space, \(y \in\mathcal{Y}\) is the output space, and there is mapping \(F:\mathbb{R}^k\to \mathcal{Y}\). Given a predefined loss function \(\mathcal{L}\), the goal of learning from data \(\mathcal{D}_{\text{FEN}_k}\) is to find a function \(F^*\) that minimizes the following expectations
%%\begin{equation}
%%	F^*(\mR(\vz)) = \argmin_{F(\mR(\vz))} \mathbb{E}_{\mR(\vz), y}\mathcal{L}(F(\mR(\vz)), y).
%%\end{equation}
%%In order to approximate \(F^*\), the gradient boosting approximation \(F\) has the following additive form
%%\[
%%F(\mR(\vz)) = \sum_{j=0}^{T_r} \beta_j h(\mR(\vz);\va_j),
%%\]
%%where \(h(\mR(\vz);\va)\) is the base classifier with parameters \(\va = \left\{a_1, a_2, \cdots\right\}\), and the base regression model \(\mathscr{L}\) is SVR. 
%%In each iteration, a base regression model is used to fit the gradient of the loss function that currently needs to be minimized. Finally, all base regression model will be weighted for prediction. Algorithm \ref{gradientboosting} gives the emsemble of SVR based on gradient boosting.
%%\begin{breakablealgorithm}
%%	\caption{Ensemble of SVR based on gradient boosting}
%%	\label{gradientboosting}
%%	\begin{algorithmic}
	%	%		\REQUIRE ~~\\
	%	%		Imaging data sets: \(\mathcal{D}_{\text{FEN}_k}, k=1,2,\cdots, K, \text{FEN} \in \text{FENs}\);\\
	%	%		Base learners: SVR \(\longrightarrow \mathscr{L}\);\\
	%	%		Number of base learners: \(T_{\text{FEN}_k}, k=1,2,\cdots, K, \text{FEN} \in \text{FENs}\);
	%	%		\ENSURE ~~\\
	%	%		 Initial guess \(F_0^{\text{FEN}_k}(\mJ(\mZ))\)\\
	%	%		\textbf{for} \(i= 1,2, \cdots, T_{\text{FEN}_k}\)\\
	%	%		\begin{equation}
		%		%			(\beta_{i}, \va_{i}) = \argmin_{\beta, \va} \sum_{k=1}^{\#\mathcal{D}_{\text{FEN}_k}} \mathcal{L}(F^{\text{FEN}_k}_{i-1}(\mJ(\mZ_k)) + \beta \mathscr{L}(\mJ(\mZ_k);\va), y_k); \label{grade1}
		%		%		\end{equation}
	%	%		\qquad and \\
	%	%		\begin{equation}
		%		%			F^{\text{FEN}_k}_{i}(\mJ(\mZ)) =F^{\text{FEN}_k}_{i-1}(\mJ(\mZ)) +  \beta_{i} \mathscr{L}(\mJ(\mZ);\va_{i}),\label{gradient21}
		%		%		\end{equation}
	%	%		\qquad solving (\ref{grade1}) with a two step procedure, the first step is\\
	%	%		\begin{equation}
		%		%			\va_{i} = \argmin_{\va,\rho} \sum_{k=1}^{\#\mathcal{D}_{\text{FEN}_k}}\left(\tilde{y}_{k,i} - \rho\mathscr{L}(\mJ(\mZ_k);\va)\right)^2,\label{gradient31}
		%		%		\end{equation}
	%	%		\qquad  where \\
	%	%		\begin{equation}
		%		%			\tilde{y}_{k,i} = - \left[\frac{\partial \mathcal{L}(F^{\text{FEN}_k}_{i-1}(\mJ(\mZ_k), y_k))}{\partial F^{\text{FEN}_k}_{i-1}(\mJ(\mZ_k))}\right].\label{gradient4}
		%		%		\end{equation}
	%	%		\qquad \qquad The \(\beta_{i}\) is determined \\
	%	%		\begin{equation}
		%		%			\beta_{i} = \argmax_{\beta} \sum_{k=1}^{\#\mathcal{D}_{\text{FEN}_k}}\mathcal{L}(F^{\text{FEN}_k}_{i-1}(\mJ(\mZ_k)) + \beta \mathscr{L}(\mJ(\mZ_k);\va_{i_1}), y_k),\label{gradient51}
		%		%		\end{equation}
	%	%		%\begin{equation}
	%	%		%	\beta_{i_2} = \argmax_{\beta} \sum_{i=1}^{\#\mathcal{B}^j_M}\mathcal{L}(F_{i_2-1}(\mJ(\mZ_i)) + \beta \mathscr{L}_{\text{Den}}(\mJ(\mZ_i);\va_{i_2}), y_i).\label{gradient52}
	%	%		%\end{equation}
	%	%		\textbf{end}\\
	%	%		\textbf{Output:} \(F_{T_{\text{FEN}_k}}(\mJ(\mZ)), k=1,2,\cdots, K, \text{FEN} \in \text{FENs}\).
	%	%	\end{algorithmic}
%%\end{breakablealgorithm}
%
%
%
%
%\section{Experiments} \label{sec5}
%In this section we apply the proposed method to real dataset, the daily minimum temperature data in Melbourne from 1981 to 1990\footnote{\url{https://www.kaggle.com/paulbrabban/daily-minimum-temperatures-in-melbourne}}.  
%In this paper, we have 9 alternative FENs and five different segmentation length \(\left\{20, 25, 30, 35, 40\right\}\), and our choice of segmentation lengths is also based on experience and can be found in \cite{tian2021drought}, for details. Since we need not only to train the FENs first, but also to extract features, the computational effort to determine which combination of segmentation length and FEN has the best time series prediction performance is huge. Therefore, we believe that the combination with the best discriminant accuracy of the imaging dataset has the best representation of the time series and thus the best predictive performance. However, we need to note that these discussions are in the context of the three paradigms of FEN construction in section \ref{sec3}, i.e., the FENs of different paradigms cannot be compared with each other. 
%
%
%Firstly, we segment the time series according to different segmentation lengths and image the segmented series according to the four imaging methods introduced in section \ref{sec2} to construct the imaging dataset. Secondly, we construct the FEN and classify the imaging dataset according to the three paradigms in section \ref{sec3}. We plot the training loss and discriminant accuracy for the three paradigms as shown in Figure \ref{dailyminlossa}.
%
%\begin{figure}[H]
%	\centering 
%	\begin{minipage}[t]{0.32\textwidth}
	%		\centering
	%		\includegraphics[scale=0.49]{figures/fen_selection/daily-min-temperatures_self-training.pdf}
	%	\end{minipage}
%	\begin{minipage}[t]{0.32\textwidth}
	%		\centering
	%		\includegraphics[scale=0.49]{figures/fen_selection/daily-min-temperatures_pre-trained.pdf}
	%	\end{minipage}
%	\begin{minipage}[t]{0.32\textwidth}
	%		\centering
	%		\includegraphics[scale=0.49]{figures/fen_selection/daily-min-temperatures_fine-tuned.pdf}
	%	\end{minipage}
%	\caption{Training losses and test accuracies corresponding to nine different FENs under different segmentation lengths for three different FEN construction paradigms. Each column represents a FEN construction paradigm and each figure has the same legend, i.e. the same colour represents the same network structure.}\label{dailyminlossa}
%\end{figure}
%
%It is clear from Figure \ref{dailyminlossa} that the fine-tuned FENs show a significant improvement in each network structure compared to the self-training and pre-trained FENs, and similarly, the self-training shows a significant improvement over the pre-trained FENs. The FENs under the three different paradigms are selected as follows,
%\begin{itemize}
%	\item For the self-training FEN, it can be found from the first column of Figure \ref{dailyminlossa} that the segmentation length of 20 has the smallest training loss (upper panel) and the largest test accuracy (bottom panel) overall. Specifically, at a segmentation length of 20, VGG13 (with training loss = 0.229, test accuracy = 1.000) can be identified as the best FEN. 
%	\item For the pre-trained FEN, it can be found from the second column of Figure \ref{dailyminlossa} that the model has the best overall performance at a segmentation length of 25, specifically, ResNet34 (with training loss = 1.341, test accuracy = 0.449) may be the best FEN. We should note that the pre-trained model is not trained on the imaging dataset, the training loss is essentially the loss of the pre-trained model on the training data, and the test accuracy is the accuracy of the pre-trained model on the test dataset. This is the reason for its larger training loss and lower test accuracy. 
%	\item Similarly, for the fine-tuned FEN, it can be observed from the third column of Figure \ref{dailyminlossa} that the segmentation length of 25 has the best performance, and specifically, VGG13 (with training loss = 0.028, test accuracy = 1.000) might be used as the best FEN.
%\end{itemize}
%
%
%In the following, we extract features from the time series based on the selected FENs and segmentation lengths under three different paradigms, and use these features for prediction. Our selected model evaluation metrics are mean square error (MSE), mean absolute error (MAE) and symmetric mean absolute percentage error (SMAPE), which are common evaluation metrics in forecasting tasks. Table \ref{raw} shows the prediction results based on the original data, while Tables \ref{resultsRP}, \ref{resultsgasf}, \ref{resultsgadf} and \ref{resultsMTF} show the prediction results after feature extraction based on imaging methods RP, GASF, GADF and MTF respectively. In addition, to demonstrate the effectiveness of the proposed feature extraction method and to compare it with the SVR (AdaBoost) in the section \ref{sec4}, several common and effective models were selected for comparison, namely Random Forest (RF) \cite{CutlerAdele2011} and Wavelet Neural Networks (WNN) \cite{AlexandridisAntonios2011}.
%\begin{table}[H]
%	\footnotesize
%	\setlength{\abovecaptionskip}{0pt}%
%	\setlength{\belowcaptionskip}{3pt}%
%	\centering
%	\caption{Prediction results without feature extraction}\label{raw}
%	\setlength{\tabcolsep}{1mm}{  
	%		\begin{tabular}{ccccccc}
		%			\toprule
		%			\multirow{2}{*}{\tabincell{c}{model}} & \multirow{2}{*}{\tabincell{c}{metrics}} & \multicolumn{5}{c}{Order of time series prediction}\\
		%			\cline{3-7}
		%			& & 20 & 25 &  30& 35 & 40  \\
		%			\midrule
		%			%		\multirow{3}{*}{\tabincell{c}{LSTM}}& MSE &5.6743/6.1606& 5.5778/6.0427& 5.8030/5.5945& 5.7935/5.0815& 6.5523/6.2263\\
		%			%		&MAE &1.8912/1.9093& 1.8375/1.9223&1.8854/1.8189& 1.8778 /1.7542& 2.0012/1.9227\\
		%			%		&SMAPE &0.1946/0.1802& 0.1866/0.1989&0.1910/0.1825& 0.1902/0.1838& 0.1991/0.1887\\
		%			%		\midrule
		%			
		%			\multirow{3}{*}{\tabincell{c}{RF}}& MSE &\textbf{0.8745}/5.8610&\textbf{0.8716}/5.9601&\textbf{0.8802}/6.1787&\textbf{0.8736}/6.0940&\textbf{0.9368}/5.8041\\
		%			&MAE &\textbf{0.7174}/1.9220&\textbf{0.7265}/1.8848&\textbf{0.7230}/1.9429&\textbf{0.7185}/1.9499&\textbf{0.7149}/1.9705\\
		%			&SMAPE &\textbf{0.0788}/0.1985 &\textbf{0.0783}/0.2067&\textbf{0.0790}/0.2010&\textbf{0.0797}/0.1866&\textbf{0.0774}/0.2016\\
		%			\midrule
		%			
		%			\multirow{3}{*}{\tabincell{c}{SVR}}& MSE &5.4839/\textbf{5.4114}&5.4499/\textbf{5.5265}& 5.4003/\textbf{5.6060}&5.3236/\textbf{5.6296}&5.2603/\textbf{5.6350}\\
		%			&MAE &1.7596/\textbf{1.8184}&1.7468/\textbf{1.8420}& 1.7245/\textbf{1.8565}&1.7062/\textbf{1.8517}&1.6963/\textbf{1.8472}\\
		%			&SMAPE &0.1823/\textbf{0.1796}& 0.1813/\textbf{0.1825}& 0.1794/\textbf{0.1839}& 0.1780/\textbf{0.1831}&0.1773/\textbf{0.1823}\\
		%			\midrule
		%			
		%			\multirow{3}{*}{\tabincell{c}{SVR\\(Adaboost)}}& MSE &5.2736/5.5167&5.1781/5.6416&5.0937/\textbf{5.6066}&5.0439/5.7002&4.9605/5.6708\\
		%			&MAE &1.7897/1.8479&1.7744/1.8692&1.7564/1.8730&1.7468/1.8814&1.7312/1.8636\\
		%			&SMAPE &0.3932/0.3872& 0.3945/0.3890&0.3934/0.3896&0.3920/0.3882&0.3904/0.3875\\
		%			\midrule
		%			
		%			\multirow{3}{*}{\tabincell{c}{WNN}}& MSE &16.387/16.112&16.368/16.133&16.313/16.171&16.235/16.179&16.149/16.194\\
		%			&MAE &3.2475/3.2844&3.2445/3.2868&3.2374/3.2918&3.2301/3.2910&3.2228/3.2911\\
		%			&SMAPE &0.3123/0.3034&0.3122/0.3037&0.3118/0.3041&0.3115/0.3040&0.3113/0.3040\\
		%			\bottomrule
		%		\end{tabular}
	%	}
%	\begin{tablenotes}
	%		\item The left and right sides of ``/'' represent the results of the training and testing phases, respectively, as do Tables \ref{resultsRP}, \ref{resultsgasf}, \ref{resultsgadf} and \ref{resultsMTF}.
	%	\end{tablenotes}
%\end{table}
%From Table \ref{raw}, we can see that the models RF, SVR and SVR (Adaboost) perform similarly and much better than WNN. In addition, it is noticeable that different segmentation lengths do not have a significant impact on the performance of the model, e.g. for RF, the magnitude of the metrics is almost the same for different segmentation lengths.
%
%\begin{table}[H]
%	\small
%	\centering
%	\caption{Prediction results under different FEN paradigms with imaging scheme as \textbf{RP}} \label{resultsRP}
%	\begin{tabular}{ccccc}
	%		\toprule
	%		model & metrics & Self-training & Pre-trained & \textbf{Fine-tuned}\\
	%		\midrule
	%		%		\multirow{3}{*}{\tabincell{c}{LSTM}}& MSE &&&\\
	%		%		&MAE &&&\\
	%		%		&SMAPE &&&\\
	%		%		\midrule
	%		
	%		\multirow{3}{*}{\tabincell{c}{RF}}& MSE &0.2478/1.6026&0.2462/1.6148&0.2514/1.5846\\
	%		&MAE &0.1236/0.3398&0.1236/0.3227&0.1236/0.3311\\
	%		&SMAPE &0.0135/0.0319&0.0136/0.0313&0.0135/0.3120\\
	%		\midrule
	%		
	%		\multirow{3}{*}{\tabincell{c}{SVR}}& MSE &9.1782/20.042&0.2776/22.4269&1.8876/2.3458\\
	%		&MAE &2.0744/3.6420&0.4909/3.7760&0.8087/1.8705\\
	%		&SMAPE &0.2050/0.3447&0.0547/0.3654&0.0854/0.3648\\
	%		\midrule
	%		
	%		\multirow{3}{*}{\tabincell{c}{SVR\\(Adaboost)}}& MSE &15.1576/16.964&12.7513/17.09&1.3650/1.6970\\
	%		&MAE &3.1076/3.3516&2.8245/3.3676&0.9321/1.3630\\
	%		&SMAPE &0.3176/0.3081&0.3200/0.3084&0.1207/0.1511\\
	%		\midrule
	%		
	%		\multirow{3}{*}{\tabincell{c}{WNN}}& MSE &16.1097/16.9177&16.1017/16.9065&16.1382/16.8027\\
	%		&MAE &3.2406/3.3136&3.2363/3.3150&3.2340/3.3302\\
	%		&SMAPE &0.3070/0.3193&0.3081/0.3159&0.3054/0.3240\\
	%		\bottomrule
	%	\end{tabular}
%\end{table}
%
%\begin{table}[H]
%	\small
%	\centering
%	\caption{Prediction results under different FEN paradigms with imaging scheme as \textbf{GASF}} \label{resultsgasf}
%	\begin{tabular}{ccccc}
	%		\toprule
	%		models & metrics & Self-training & Pre-trained & \textbf{Fine-tuned}\\
	%		\midrule
	%		%		\multirow{3}{*}{\tabincell{c}{LSTM}}& MSE &&&\\
	%		%		&MAE &&&\\
	%		%		&SMAPE &&&\\
	%		%		\midrule
	%		
	%		\multirow{3}{*}{\tabincell{c}{RF}}& MSE &0.2462/1.6148&0.2469/1.5304&0.2480/1.5682\\
	%		&MAE &0.1231/0.3345&0.1236/0.3227&0.1226/0.3277\\
	%		&SMAPE &0.0135/0.0315&0.0135/0.0304&0.0135/0.0309\\
	%		\midrule
	%		
	%		\multirow{3}{*}{\tabincell{c}{SVR}}& MSE &9.0464/16.8628&0.2600/21.9285&0.8321/1.8860\\
	%		&MAE &2.0315/3.3410&0.4846/3.7789&0.1912/0.3478\\
	%		&SMAPE &0.2004/0.3148&0.0543/0.3509&0.1884/0.3338\\
	%		\midrule
	%		
	%		\multirow{3}{*}{\tabincell{c}{SVR\\(Adaboost)}}& MSE &15.0842/16.8569&13.1500/16.6203&1.4647/1.6974\\
	%		&MAE &3.0975/3.3518&2.8767/3.3446&0.4970/1.0335\\
	%		&SMAPE &0.3168/0.3071&0.3193/0.308&0.3176/0.3067\\
	%		\midrule
	%		
	%		\multirow{3}{*}{\tabincell{c}{WNN}}& MSE &16.2855/16.3987&16.2945/16.3397&16.2328/16.5225\\
	%		&MAE &3.2542/3.2657 &3.2550/3.2691&3.2458/3.2845\\
	%		&SMAPE &0.3115/0.3055&0.3081/0.3160&0.3094/0.3119\\
	%		\bottomrule
	%	\end{tabular}
%\end{table}
%
%\begin{table}[H]
%	\small
%	\centering
%	\caption{Prediction results under different FEN paradigms with imaging scheme as \textbf{GADF}} \label{resultsgadf}
%	\begin{tabular}{ccccc}
	%		\toprule
	%		models & metrics & Self-training & Pre-trained & \textbf{Fine-tuned}\\
	%		\midrule
	%		%		\multirow{3}{*}{\tabincell{c}{LSTM}}& MSE &&&\\
	%		%		&MAE &&&\\
	%		%		&SMAPE &&&\\
	%		%		\midrule
	%		
	%		\multirow{3}{*}{\tabincell{c}{RF}}& MSE &0.2525/1.7540&0.2746/1.6359&0.2577/1.7672\\
	%		&MAE &0.1239/0.3318&0.1282/0.3265&0.1256/0.3382\\
	%		&SMAPE &0.0133/0.0313&0.0139/0.0308&0.0137/0.0315\\
	%		\midrule
	%		
	%		\multirow{3}{*}{\tabincell{c}{SVR}}& MSE &6.5503/20.6106&0.2452/23.2767&0.8972/2.1280\\
	%		&MAE &1.6588/3.5855&0.4816/3.7762&0.6106/1.6968\\
	%		&SMAPE &0.1642/0.3443&0.0533/0.3642&0.0664/0.3565\\
	%		\midrule
	%		\multirow{3}{*}{\tabincell{c}{SVR\\(Adaboost)}}& MSE &14.2156/16.4264&13.0922/16.2227&1.3123/1.6557\\
	%		&MAE &2.9919/3.2815&2.8588/3.2733&0.8421/1.2657\\
	%		&SMAPE &0.3220/0.3116&0.3193/0.3085&0.3229/0.3108\\
	%		\midrule
	%		
	%		\multirow{3}{*}{\tabincell{c}{WNN}}& MSE &16.5826/15.508&16.4302/15.9396&15.9782/17.2787\\
	%		&MAE &3.2804/3.1873&3.2590/3.2586&3.2173/3.3706\\
	%		&SMAPE &0.3141/0.2977&0.3082/0.3159&0.3063/0.3210\\
	%		\bottomrule
	%	\end{tabular}
%\end{table}
%
%
%
%
%\begin{table}[H]
%	\small
%	\centering
%	\caption{Prediction results under different FEN paradigms with imaging scheme as \textbf{MTF}} \label{resultsMTF}
%	\begin{tabular}{ccccc}
	%		\toprule
	%		model & metrics & Self-training & Pre-trained & \textbf{Fine-tuned}\\
	%		\midrule
	%		%		\multirow{3}{*}{\tabincell{c}{LSTM}}& MSE &&&\\
	%		%		&MAE &&&\\
	%		%		&SMAPE &&&\\
	%		%		\midrule
	%		
	%		\multirow{3}{*}{\tabincell{c}{RF}}& MSE &0.2801/1.6449&0.2672/1.8602&0.2824/1.6420\\
	%		&MAE &0.1298/0.3280&0.1270/0.3470&0.1292/0.3260\\
	%		&SMAPE &0.0132/0.0312&0.0135/0.03310&0.0139/0.0306\\
	%		\midrule
	%		
	%		\multirow{3}{*}{\tabincell{c}{SVR}}& MSE &13.300/16.3801&0.2588/23.5088&0.6983/2.2067\\
	%		&MAE &2.7508/3.2121&0.4839/3.8791&0.1686/0.3692\\
	%		&SMAPE &0.2651/0.3019&0.0543/0.3651&0.1665/0.3490\\
	%		\midrule
	%		
	%		\multirow{3}{*}{\tabincell{c}{SVR\\(Adaboost)}}& MSE &15.9704/16.4199&12.9034/16.8592&1.4776/1.6421\\
	%		&MAE &3.1937/3.3104&2.8474/3.3537&0.3951/1.3247\\
	%		&SMAPE &0.3145/0.3048&0.3193/0.3079&0.3173/0.3072\\
	%		\midrule
	%		
	%		\multirow{3}{*}{\tabincell{c}{WNN}}& MSE &15.9581/17.3777&15.9241/17.4366&16.1259/16.854\\
	%		&MAE &3.2216/3.3734&3.2209/3.3643&3.2513/3.2670\\
	%		&SMAPE &0.3033/0.3305&0.3054/0.3238&0.3102/0.3094\\
	%		\bottomrule
	%	\end{tabular}
%\end{table}
%
%Comparing Tables \ref{resultsRP} to \ref{resultsMTF}, we can obtain the following results: (1) predictions based on extracted features are more likely to be overfitted, which can be easily observed from the tables, i.e. the difference between training and testing metrics is large; (2) predictions based on features extracted by different imaging methods are similar, which means that different imaging methods do not have a significant impact on the final extracted features; (3) fine-tuned FENs have a better performance than pre-trained and self-trained ones. Comparing Table \ref{raw} with Tables \ref{resultsRP}, \ref{resultsgasf}, \ref{resultsgadf} and \ref{resultsMTF}, we can obtain the following results: (1) among the three different paradigms for the construction of FENs, only the fine-tuned FEN has improved the prediction performance; (2) the prediction performance of WNN has hardly changed compared to the prediction results on the original data, which may mean that this feature extraction method fails for WNN.
%
%The reasons for the poor prediction performance of pre-trained and self-trained FENs are analysed as follows. For pre-training, the parameters are not trained on the imaging dataset and therefore the depth representation of the image cannot be extracted well for prediction. For self-training, the parameters are randomly initialised and then trained on the imaging dataset, which may not be able to learn enough due to the limited size of the imaging dataset, and therefore cannot extract the image features well. To confirm our analysis, we compare the variability of the 512-dimensional features obtained with three different paradigms of FENs and four different imaging modalities. In this paper, we use principal component analysis and plot the cumulative distribution function of the kernel density estimates (using the Gaussian kernel) of the principal component contributions, as shown in Figure \ref{pcakernel} .
%
%\begin{figure}[H]
%	\centering 
%	\begin{minipage}[t]{0.24\textwidth}
	%		\centering
	%		\includegraphics[scale=0.31]{figures/density_analysis/daily-min-temperatures_RP_density.pdf}
	%	\end{minipage}
%	\begin{minipage}[t]{0.24\textwidth}
	%		\centering
	%		\includegraphics[scale=0.31]{figures/density_analysis/daily-min-temperatures_GASF_density.pdf}
	%	\end{minipage}
%	\begin{minipage}[t]{0.24\textwidth}
	%		\centering
	%		\includegraphics[scale=0.31]{figures/density_analysis/daily-min-temperatures_GADF_density.pdf}
	%	\end{minipage}
%	\begin{minipage}[t]{0.24\textwidth}
	%		\centering
	%		\includegraphics[scale=0.31]{figures/density_analysis/daily-min-temperatures_MTF_density.pdf}
	%	\end{minipage}
%	\caption{Cumulative distribution function of the kernel density estimates of the contribution of the corresponding principal components of the extracted features. From the left to the right panel are based on imaging modality RP, GASF, GADF and MTF, respectively.} \label{pcakernel}
%\end{figure}
%
%It is clear from Figure \ref{pcakernel} that the fine-tuned FEN is always in between self-training and pre-training for the different imaging modalities, which explains the better predictive performance of the fine-tuned network. For the features extracted by the pre-training network, it can be found that the cumulative distribution function is almost concentrated around one point, which means that the contribution is almost concentrated on one principal component, indicating that there is no diversity in the extracted features, which also leads to poor prediction performance. For self-training models with a wide range of cumulative distribution functions, which means that the contribution of the principal components is more similar, i.e. there is a high degree of similarity between individual features and a large amount of redundancy, thus leading to poor predictive performance. The fine-tuned FEN sits between self-training and pre-training, taking into account the diversity and similarity between features and therefore offering better predictive performance in comparison.
%
%
%\section{Concluding remarks} \label{sec6}
%In this paper, we propose a time series prediction method based on deep representation learning. Specifically, we first image time series based on different methods and construct imaging datasets for training FENs. Secondly, we use the FEN to extract features of the time series and use them for prediction. Also, we consider three different paradigms for the construction of FENs for comparison. Finally, to improve the robustness of the model, we ensemble SVR based on AdaBoost. 
%
%
%We applied the proposed method to the Melbourne daily minimum temperature data and the experimental results showed that the fine-tuned FEN achieves optimal performance, slightly outperforming the prediction on the raw data. Moreover, the self-training and pre-training based prediction performance is worse than the raw data prediction for the same model settings. This also suggests that we need not only pre-traine	d models on large-scale datasets when representing time series based on deep learning models, but also fine-tuning on task-relevant datasets.  





%
%
%% 16种方法
%\begin{table}[H]
%\tiny
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Discrimination accuracy based on univariate point-value time series methods.}
%\setlength{\tabcolsep}{1mm}{ 
	%\begin{tabular}{cccccccccc|cccccc}
	%\hline
	%\multirow{2}{*}{DGPs}  & \multirow{2}{*}{Point}  & \multicolumn{8}{c|}{Non-deep learning methods} & \multicolumn{6}{c}{Deep learning-based approachs} \\
	%\cline{3-16}
	%&  & KN & SD & IB & ITDE & MrSQM  & Bagging & CFT & WE & FCN & FCNPlus & Inception & XCoord & MLP & RNN\\
	%\hline
	%\multirow{4}{*}{\tabincell{c}{DGP1}} & \(c\) &19.60 & 19.00 & 23.60 & 19.00 & 22.00 & 22.40 & 21.60& 20.20 &&&&&&\\
	%& \(r\) &21.40 & 19.20 & 17.60 & 20.80 & 18.20 & 16.80 & 19.00 & 20.60 &&&&&&\\ 
	%& \(l\) &18.40 & 18.34 & 21.00 & 19.60 & 21.60 & 21.40 & 82.00 & 19.80 &&&&&&\\ 
	%& \(u\) &20.40 & 20.40 & 30.80 & 23.80 & 21.20 & 18.60 & 86.20 & 17.20 &&&&&&\\
	%\hline
	%
	%\multirow{4}{*}{\tabincell{c}{DGP2}} & \(c\) &20.60 & 19.80 & 20.00 & 19.60 & 21.20 & 34.00 & 30.80 & 26.40 &&&&&&\\
	%& \(r\) &24.40 & 25.60 & 23.60 & 33.20 & 50.80 & 42.80 & 45.00 & 38.80 &&&&&&\\ 
	%& \(l\) &18.20 & 19.20 & 18.80 & 21.80 & 19.80 & 20.60 & 54.00 & 19.80 &&&&&&\\ 
	%& \(u\) &22.60 & 23.60 & 24.20 & 27.60 & 44.40 & 41.80 & 45.20 & 42.40 & &&&&&\\ 
	%\hline
	%
	%\multirow{4}{*}{\tabincell{c}{DGP3}} & \(c\) &18.20 & 21.80 & 19.60 & 19.00 & 25.80 & 27.40 & 31.40 & 25.40 &&&&&&\\
	%& \(r\) &22.00 & 21.20 & 26.00 & 32.80 & 62.40 & 38.80 & 60.60 & 35.60 &&&&&&\\ 
	%& \(l\) &19.60 & 19.00 & 16.00 & 21.80 & 18.80 & 19.60 & 49.40 & 15.80 &&&&&&\\ 
	%& \(u\) &21.00 & 21.20 & 24.40& 24.80 & 48.40 & 43.60 & 65.80 & 43.60 &&&&&&\\
	%\hline	
	%\end{tabular}
	%
	%}
%
%\end{table}
%
%\begin{table}[H]
%\tiny 
%\setlength{\abovecaptionskip}{0pt}%
%\setlength{\belowcaptionskip}{3pt}%
%\centering
%\caption{Discrimination accuracy based on univariate point-value time series methods.}
%\setlength{\tabcolsep}{1mm}{ 
	%	\begin{tabular}{ccccccccccccccc}
		%		\hline
		%		\multirow{2}{*}{DGPs}  & \multirow{2}{*}{Point}  & \multicolumn{13}{c}{Deep learning-based approachs} \\
		%		\cline{3-15}
		%		&  & LSTM & GRU & RNN\_FCN & LSTM\_FCN & GRU\_FCN  & MRNN\_FCN & MLSTM\_FCN & MGRU\_FCN & ResCNN & ResNet & TCN & TST & Transformer\\
		%		\hline
		%		\multirow{4}{*}{\tabincell{c}{DGP1}} & \(c\) &19.60 & 19.00 & 23.60 & 19.00 & 22.00 & 22.40 & 21.60& 20.20 &&&&&\\
		%		& \(r\) &21.40 & 19.20 & 17.60 & 20.80 & 18.20 & 16.80 & 19.00 & 20.60 &&&&&\\ 
		%		& \(l\) &18.40 & 18.34 & 21.00 & 19.60 & 21.60 & 21.40 & 82.00 & 19.80 &&&&&\\ 
		%		& \(u\) &20.40 & 20.40 & 30.80 & 23.80 & 21.20 & 18.60 & 86.20 & 17.20 &&&&&\\
		%		\hline
		%		
		%		\multirow{4}{*}{\tabincell{c}{DGP2}} & \(c\) &20.60 & 19.80 & 20.00 & 19.60 & 21.20 & 34.00 & 30.80 & 26.40 &&&&&\\
		%		& \(r\) &24.40 & 25.60 & 23.60 & 33.20 & 50.80 & 42.80 & 45.00 & 38.80 &&&&&\\ 
		%		& \(l\) &18.20 & 19.20 & 18.80 & 21.80 & 19.80 & 20.60 & 54.00 & 19.80 &&&&&\\ 
		%		& \(u\) &22.60 & 23.60 & 24.20 & 27.60 & 44.40 & 41.80 & 45.20 & 42.40 & &&&&\\ 
		%		\hline
		%		
		%		\multirow{4}{*}{\tabincell{c}{DGP3}} & \(c\) &18.20 & 21.80 & 19.60 & 19.00 & 25.80 & 27.40 & 31.40 & 25.40 &&&&&\\
		%		& \(r\) &22.00 & 21.20 & 26.00 & 32.80 & 62.40 & 38.80 & 60.60 & 35.60 &&&&&\\ 
		%		& \(l\) &19.60 & 19.00 & 16.00 & 21.80 & 18.80 & 19.60 & 49.40 & 15.80 &&&&&\\ 
		%		& \(u\) &21.00 & 21.20 & 24.40& 24.80 & 48.40 & 43.60 & 65.80 & 43.60 &&&&&\\
		%		\hline	
		%	\end{tabular}
	%	
	%}
%
%\end{table}




%\begin{table}[H] 
%	\setlength{\abovecaptionskip}{0pt}%
%	\setlength{\belowcaptionskip}{3pt}%
%	\centering
%	\caption{Discrimination accuracy based on multivariate point-value time series methods.}
%	\setlength{\tabcolsep}{2mm}{ 
%		\begin{tabular}{cccccc|cccccc}
%			\hline
%			\multirow{2}{*}{DGPs}  & \multirow{2}{*}{Point}  & \multicolumn{4}{c|}{Non-deep learning methods} & \multicolumn{6}{c}{Deep learning-based approachs} \\
%			\cline{3-12}
%			&  & KN  & ITDE & Bagging & WE & TapNet & MLP & FCN & Inception & LF  & CNN\\
%			\hline
%			\multirow{4}{*}{\tabincell{c}{C1}} & \(c\) &37.33&71.00&82.33&77.00&&&&&&\\
%			& \(r\) &38.67 & 70.33&75.67 & 69.33&&&&&&\\
%			& \(l\) &37.33 & 65.67 & 76.67 & 73.67 & &&&&&\\ 
%			& \(u\) &37.33&73.00&68.67 & 71.33 &&&&&&\\
%			\hline
%			\multirow{4}{*}{\tabincell{c}{C2}} & \(c\) & 17.00 & 18.60 & 23.20 & 21.00 &&&&&&\\
%			& \(r\) &20.80 & 38.20 & 37.40 & 34.80 &&&&&&\\ 
%			& \(l\) &18.20 & 18.60 & 21.60 & 19.60 &&&&&&\\ 
%			& \(u\) &20.40 & 30.20 & 35.80 & 41.60 &&&&&&\\
%			\hline	
%		\end{tabular}
%	}
%\end{table}








%\begin{table}[H]
%	\scriptsize 
%	\setlength{\abovecaptionskip}{0pt}%
%	\setlength{\belowcaptionskip}{3pt}%
%	\centering
%	\caption{Discrimination accuracy based on univariate point-value time series methods.}
%	\setlength{\tabcolsep}{1.2mm}{ 
%		\begin{tabular}{cccccccccc|cccccc}
%			\hline
%			\multirow{2}{*}{DGPs}  & \multirow{2}{*}{Point}  & \multicolumn{8}{c|}{Non-deep learning methods} & \multicolumn{6}{c}{Deep learning-based approachs} \\
%			\cline{3-16}
%			&  & KN & SD & IB & ITDE & MrSQM  & Bagging & CFT & WE & TapNet & MLP & FCN & LF & Inception & CNN\\
%			\hline
%			\multirow{4}{*}{\tabincell{c}{H-S}} & \(c\) &46.03 & 55.56 & 61.90 & 65.08 & 82.54 & 76.19 & 76.19 & 79.37 &&&&&&\\
%			& \(r\) &55.56 & 58.73 & 66.67 & 69.84 & 65.08 & 80.95 & 87.30 & 74.60 &&&&&&\\ 
%			& \(l\) &61.9 & 60.32 & 65.08 & 61.90 & 74.60 & 74.60 & 84.13 & 88.89 &&&&&&\\ 
%			& \(u\) &53.97 & 69.84 & 68.25 & 63.49 & 76.19 & 80.95 & 80.95 & 74.6 &&&&&&\\
%			\hline
%			
%			\multirow{4}{*}{\tabincell{c}{S-T-B}} & \(c\) &25.56 & 33.83 & 38.35 & 37.59 & 38.35 & 39.10 & 41.35 & 45.11 &&&&&\\
%			& \(r\) &35.34 & 48.12 & 35.34 & 33.08 & 43.61 & 45.86 & 54.14 & 40.6 &&&&&\\ 
%			& \(l\) &32.33 & 38.35 & 39.85 & 36.84 & 50.38 & 51.88 & 57.14 & 45.11 &&&&&&\\ 
%			& \(u\) &27.82 & 24.81 & 38.35 & 36.84 & 48.87 & 50.38 & 46.62 & 50.38 &&&&&\\
%			\hline
%			
%			\multirow{4}{*}{\tabincell{c}{H-S-T-B}} & \(c\) &20.53 & 23.84 & 26.49 & 25.83 & 43.71 & 36.42 & 39.07 & 35.76 & &&&&& \\
%			& \(r\) &27.15 & 34.43 & 33.11 & 33.11 & 31.13 & 39.74 & 49.01 & 39.07 &&&&&\\ 
%			& \(l\) &22.52 & 25.82& 29.14 & 28.48 & 39.07 & 42.38 & 50.99 & 44.37 &&&&&\\ 
%			& \(u\) &19.87 & 21.19 & 34.44 & 29.14 & 36.42 & 42.38 & 39.07 & 38.41 & &&&&&\\
%			\hline
%		\end{tabular}
%		
%	}
%	
%\end{table}



%
%\begin{table}[H] 
%	\setlength{\abovecaptionskip}{0pt}%
%	\setlength{\belowcaptionskip}{3pt}%
%	\centering
%	\caption{Discrimination accuracy based on multivariate point-value time series methods.}
%	\setlength{\tabcolsep}{2mm}{ 
%		\begin{tabular}{cccccc|cccccc}
%			\hline
%			\multirow{2}{*}{DGPs}  & \multirow{2}{*}{Point}  & \multicolumn{4}{c|}{Non-deep learning methods} & \multicolumn{6}{c}{Deep learning-based approachs} \\
%			\cline{3-12}
%			&  & KN  & ITDE & Bagging & WE & TapNet & MLP & FCN & Inception & LF  & CNN\\
%			\hline
%			\multirow{4}{*}{\tabincell{c}{H-S}} & \(c\) &92.06 & 76.19 & 73.02 & 93.65&&&&&&\\
%			& \(r\) &90.48 & 69.84 & 79.37 & 74.60&&&&&&\\ 
%			& \(l\) &88.89 & 80.95 & 71.43 & 87.30 &&&&&&\\ 
%			& \(u\) &92.06 & 82.54 & 73.02 & 90.48 &&&&&&\\
%			\hline
%			\multirow{4}{*}{\tabincell{c}{S-T-B}} & \(c\) &100.0 & 64.66 & 31.58 & 58.65 &&&&&&\\
%			& \(r\) &66.17 & 42.86 & 36.84 & 48.12 &&&&&&\\ 
%			& \(l\) &100.0 & 59.40 & 36.097 & 58.65 &&&&&&\\ 
%			& \(u\) &98.50 & 72.18 & 33.83 & 56.39 &&&&&&\\
%			\hline
%			\multirow{4}{*}{\tabincell{c}{H-S-T-B}} & \(c\) &96.03 & 52.98 & 29.80 & 61.59 &&&&&&\\
%			& \(r\) &67.55 & 46.36 & 37.75 & 45.70 &&&&&&\\ 
%			& \(l\) &96.69 & 56.29 & 36.42 & 58.28 &&&&&&\\ 
%			& \(u\) &93.38 & 58.28 & 47.68 & 54.97 &&&&&&\\
%			\hline	
%		\end{tabular}
%	}
%\end{table}


%
%\begin{table}[H]
%	\small 
%	\setlength{\abovecaptionskip}{0pt}%
%	\setlength{\belowcaptionskip}{3pt}%
%	\centering
%	\caption{Discrimination accuracy based on multivariate point-value time series methods.}
%	\setlength{\tabcolsep}{2mm}{ 
%		\begin{tabular}{ccccc|cccccc}
%			\hline
%			\multirow{2}{*}{Point}  & \multicolumn{4}{c|}{Non-deep learning methods} & \multicolumn{6}{c}{Deep learning-based approachs} \\
%			\cline{2-11}
%			& KN  & ITDE & Bagging & WE & TapNet & MLP & FCN & Inception & LF  & CNN\\
%			\hline
%			\(c\) &77.78 & 51.85 & 83.33 & 83.33 &&&&&&\\
%			\(r\) &94.44 & 66.67 & 83.33 & 83.33 &&&&&&\\
%			\(l\) &77.78 & 59.26 & 83.33 & 83.33 &&&&&&\\
%			\(u\) &90.74 & 50.00 & 83.33 & 83.33 &&&&&&\\	
%			\hline	
%		\end{tabular}
%	}
%\end{table}

